SEEDS: Exponential SDE Solvers for Fast High-Quality Sampling from Diffusion Models

A potent class of generative models known as Diffusion Probabilistic Models (DPMs) has become prominent. A forward diffusion process adds gradually noise to data, while a model learns to gradually denoise. Sampling from pre-trained DPMs is obtained by solving differential equations (DE) defined by the learnt model, a process which has shown to be prohibitively slow. Numerous efforts on speeding-up this process have consisted on crafting powerful ODE solvers. Despite being quick, such solvers do not usually reach the optimal quality achieved by available slow SDE solvers. Our goal is to propose SDE solvers that reach optimal quality without requiring several hundreds or thousands of NFEs to achieve that goal. We propose Stochastic Explicit Exponential Derivative-free Solvers (SEEDS), improving and generalizing Exponential Integrator approaches to the stochastic case on several frameworks. After carefully analyzing the formulation of exact solutions of diffusion SDEs, we craft SEEDS to analytically compute the linear part of such solutions. Inspired by the Exponential Time-Differencing method, SEEDS use a novel treatment of the stochastic components of solutions, enabling the analytical computation of their variance, and contains high-order terms allowing to reach optimal quality sampling $\sim3$-$5\times$ faster than previous SDE methods. We validate our approach on several image generation benchmarks, showing that SEEDS outperform or are competitive with previous SDE solvers. Contrary to the latter, SEEDS are derivative and training free, and we fully prove strong convergence guarantees for them.

==> data/drawPixel1.tex <==
\newcommand{\drawPixelOne}{%
(1, -0.8726907120940317)
(2, -0.8382374066818454)
(3, -0.6504518648520856)
(4, -1.0701605191767383)
(5, -1.313866005255552)
(6, -0.6764591504926698)
(7, -1.2047764120862434)
(8, -0.7371782928137791)
(9, -0.5526959210872799)
(10, 0.19521661622140574)
(11, 0.18774072297868483)
(12, 1.0986511359773161)
(13, 1.0433517133405554)
(14, 0.10705237548656599)
(15, 0.18383440963741077)
(16, -0.38680859732005646)
(17, -0.20342148157217785)
(18, 0.7377817996227326)
(19, 1.050972902884963)
(20, 0.8259486622567886)
(21, 0.599921260877087)
(22, 0.16274371384680913)
(23, 0.28192928572961107)
(24, 0.1606923765612971)
(25, 0.2897897210111483)
(26, 0.03338176618479649)
(27, 0.42433653718964254)
(28, 0.2816526939935101)
(29, -0.02224563530563442)
(30, -0.5547396032741013)
(31, -0.8013945796589704)
(32, -0.9416479065112446)
(33, -0.8598739682299843)
(34, -0.7164793224174381)
(35, -1.1146365992233043)
(36, -1.356882451806366)
(37, -1.658007087661554)
(38, -1.321617744576581)
(39, -0.9305724145830679)
(40, -1.2665140028945268)
(41, -1.3787848619771181)
(42, -1.4586929573826828)
(43, -1.420500621013794)
(44, -1.1624312481203236)
(45, -1.3480467289335427)
(46, -1.3663801033988403)
(47, -1.1059164049376373)
(48, -0.9203062549484845)
(49, -0.7421568253199278)
(50, -0.7421568253199278)
}


\newcommand{\drawPixelTwo}{%
(1, 0.1657364210939875)
(2, -1.3500793093311927)
(3, -1.2222730672245157)
(4, -0.4292601521936965)
(5, -0.250735378203858)
(6, 1.0567805476817775)
(7, 0.11331225497836961)
(8, 0.2552710406615663)
(9, -0.4595604917977836)
(10, -0.0721828399085453)
(11, 0.3502644080443672)
(12, 1.161786992752859)
(13, 2.076314986356116)
(14, 2.139924191186037)
(15, 2.342672515077124)
(16, 1.801003512575599)
(17, 0.502873427388816)
(18, 0.5455184697444752)
(19, 0.48914323083195377)
(20, -0.21069307554696648)
(21, -0.10475018397176791)
(22, -0.37100925498109516)
(23, 0.025209754529168515)
(24, 0.10417046774493231)
(25, 0.40490592927850283)
(26, 0.3983639713749668)
(27, 0.4503193480673243)
(28, 0.6866824946487932)
(29, 0.12829197117714541)
(30, 0.42684339810514643)
(31, 0.6599617006109495)
(32, 0.5963787604750931)
(33, -0.01885565263953959)
(34, -0.0741391032099191)
(35, 0.0879860821545992)
(36, 0.48944338998289694)
(37, 0.4657475408704406)
(38, 0.5459390581426523)
(39, 0.9568799987104945)
(40, 1.2322003609238559)
(41, 1.2325287283338249)
(42, 1.5266616235925272)
(43, 1.494710788421198)
(44, 1.4175957244203967)
(45, 1.234398578373442)
(46, 1.051260542142192)
(47, 0.9049956054248841)
(48, 0.8384686515416594)
(49, 0.9036727261791023)
(50, 0.9036727261791023)
}


\newcommand{\drawPixelThree}{%
(1, 1.8761629693121673)
(2, 1.520682323637531)
(3, 1.6074733996369135)
(4, 1.578773585367248)
(5, 2.826231519740435)
(6, 1.8465157503215266)
(7, 2.786379999776895)
(8, 1.5698659086989832)
(9, 0.5108576504399127)
(10, 1.185368587219068)
(11, 0.9983261983635834)
(12, 1.1033469464515804)
(13, 0.8775364683070498)
(14, -0.36984540005499367)
(15, -0.2573070411450459)
(16, 0.005633401155328593)
(17, -0.32993953828677525)
(18, -0.9375173597917197)
(19, -0.31247362715644833)
(20, -0.22370988729618288)
(21, -0.5994215977422479)
(22, -0.8357576527532997)
(23, -0.8887194822915494)
(24, -1.3011623349880184)
(25, -0.8923489622865994)
(26, -0.4192633458064019)
(27, -0.6938071293580017)
(28, -0.616599306927895)
(29, -0.9634069878589571)
(30, -0.8696201813220452)
(31, -0.7979686875143148)
(32, -0.4573445425477865)
(33, -0.9436483808067269)
(34, -0.8263481260143131)
(35, -0.1659187180263051)
(36, -0.2101406219526212)
(37, 0.08264293835402678)
(38, 0.24512965829245964)
(39, 0.23624757517278705)
(40, -0.1911995553063133)
(41, -0.3868368156950517)
(42, -0.8795241688006347)
(43, -0.923096812898104)
(44, -0.8559967242017774)
(45, -0.8871263274488377)
(46, -0.8327211548011907)
(47, -0.6603893518551576)
(48, -0.4768467313120509)
(49, -0.5087472475133888)
(50, -0.5087472475133888)
}


\newcommand{\drawPixelFour}{%
(1, 1.0431414556564125)
(2, 1.4430673989956773)
(3, 1.2136781152339675)
(4, 1.1275040113792727)
(5, 0.8114072716382417)
(6, 1.004571549654105)
(7, 0.69212754966406)
(8, 0.36929868377332536)
(9, 1.3666533322142669)
(10, 0.4465112902874022)
(11, 0.6104826720291017)
(12, 0.3469134150180439)
(13, -0.35834452058044663)
(14, 0.43582519101379846)
(15, -0.5458711496534564)
(16, -0.7429962317638087)
(17, -1.3694813865654893)
(18, -1.674227464366055)
(19, -1.0637730961678753)
(20, -0.9782434147562948)
(21, -0.721739781078777)
(22, -0.3807233731979748)
(23, -0.601586373625388)
(24, -0.6216493356854208)
(25, -0.41170894056764096)
(26, -0.9288336337984584)
(27, -0.9431520530009081)
(28, -0.965337810152896)
(29, 0.0315994883643399)
(30, 0.9026936433947427)
(31, 0.8734334868802824)
(32, 1.3177441092305853)
(33, 1.7302795969778137)
(34, 1.617458472971499)
(35, 1.492509186424102)
(36, 1.4254044929702945)
(37, 1.4302049258848997)
(38, 0.6853935890962011)
(39, 0.3723011634038793)
(40, 0.32589047623857614)
(41, 0.617076281829942)
(42, 0.8837497259319266)
(43, 0.8574834213732436)
(44, 0.780007976091401)
(45, 0.6372456575948333)
(46, 0.6307371968456967)
(47, 0.8577646400083363)
(48, 0.7184902109886048)
(49, 0.7748642418574786)
(50, 0.7748642418574786)
}


\newcommand{\drawPixelFive}{%
(1, -1.5684069905924498)
(2, -1.2760044185092596)
(3, -1.2181766329047434)
(4, -0.8608491118966531)
(5, -0.08795525111140035)
(6, 0.5471864461227441)
(7, 1.045020884382823)
(8, 0.5867219623550883)
(9, 0.397902814247124)
(10, 0.4947371909782287)
(11, 0.014559807849222173)
(12, 0.24714373327900296)
(13, 0.8269799029535521)
(14, 0.3266791211410584)
(15, 0.7030146099602271)
(16, 0.2239604127236205)
(17, -0.02642448648170531)
(18, 0.5448871506369353)
(19, 0.4886858149345387)
(20, 0.18936456800804816)
(21, -0.3869257572042811)
(22, -0.4301112724927767)
(23, -1.0995752123077134)
(24, -0.6450260850034925)
(25, -0.917833734429923)
(26, -1.0188746293870339)
(27, -0.6617092307325311)
(28, -0.29371506210547466)
(29, -0.29833875272285015)
(30, -1.1386812353529323)
(31, -0.8350661304808109)
(32, -0.43759581655437496)
(33, 0.3105549755190526)
(34, 0.13871407893465101)
(35, 0.4889384893786951)
(36, 0.8228520480860635)
(37, 0.5037712055341101)
(38, 0.29866803108560913)
(39, 0.5738044909752947)
(40, 0.2090496418472026)
(41, -0.18092277308590943)
(42, 0.057914040521183735)
(43, 0.07548408120621548)
(44, -0.0046222900505444075)
(45, -0.17918075263435135)
(46, -0.4049481042388899)
(47, -0.49456803840099967)
(48, -0.39375532681670394)
(49, -0.33715445376404435)
(50, -0.33715445376404435)
}


\newcommand{\drawPixelSix}{%
(1, 0.9102963643888693)
(2, 1.7895768510317687)
(3, 1.7828690152285072)
(4, 1.201047709170033)
(5, 0.8627074045901464)
(6, 0.7390731891728495)
(7, 0.6816695345306056)
(8, 0.7253492899502997)
(9, 0.29204813750417674)
(10, 0.29737699968526726)
(11, 0.044783187549083)
(12, 0.033991286476368676)
(13, -0.18473670931850347)
(14, -0.9836963397116952)
(15, -1.0258262419199697)
(16, -0.08594236184854642)
(17, -0.23879287461569826)
(18, 0.4272285547404132)
(19, 0.9090290697544228)
(20, 1.237223955669902)
(21, 1.1045609538955568)
(22, 1.5374112562990754)
(23, 1.6400952537429578)
(24, 1.6235572175662787)
(25, 1.7602130874842843)
(26, 1.9647320161170543)
(27, 1.2224537533906061)
(28, 0.7177246957785206)
(29, 0.5879390811420769)
(30, 0.8363762649438404)
(31, 1.087782857835112)
(32, 0.7680995402845976)
(33, 1.2793133142808886)
(34, 1.4477605437176295)
(35, 0.8958189542049757)
(36, 1.0312239737936557)
(37, 1.248524783829236)
(38, 1.3102867477835514)
(39, 1.227458564368302)
(40, 1.066822599614494)
(41, 1.0236100827100691)
(42, 1.277394966127994)
(43, 1.2842735851637634)
(44, 1.438772893158582)
(45, 1.2862496192200463)
(46, 1.2051708535538663)
(47, 1.0485082485704085)
(48, 1.064742904360559)
(49, 1.0000141779054954)
(50, 1.0000141779054954)
}


\newcommand{\drawPixelSeven}{%
(1, 0.5183381888281092)
(2, -0.04389985253058448)
(3, -0.10763909560983119)
(4, 0.4101765067823522)
(5, 0.14787539751074652)
(6, 1.077619047898462)
(7, 1.084561581376383)
(8, 1.3456350340931795)
(9, 1.3002067342329036)
(10, 1.0105196778836745)
(11, 0.5540623368586053)
(12, 0.8093168330902123)
(13, 1.1587855983432616)
(14, 1.2924388750966205)
(15, 1.3759082707771166)
(16, 1.8190887804241502)
(17, 0.9912993888008395)
(18, 2.0813779921749473)
(19, 1.5626092553103441)
(20, 1.0637662235113057)
(21, 0.9696044640203396)
(22, 1.481876139829899)
(23, 0.7930327755153461)
(24, 1.1775817650199878)
(25, 2.1599003206477665)
(26, 1.530331726213348)
(27, 1.5178675487614277)
(28, 1.1711262582952253)
(29, 1.0501304388862867)
(30, 1.177777375022963)
(31, 0.6621510416562822)
(32, 0.33393460393484264)
(33, 0.4060282470493838)
(34, 0.3465817971165205)
(35, 0.2416945721975216)
(36, 0.11889420047370375)
(37, 0.4313376261655601)
(38, 0.7109983566365774)
(39, 0.6809104342627368)
(40, 1.0762308895871573)
(41, 1.454073066790802)
(42, 1.13229794974235)
(43, 1.0297781964450996)
(44, 1.3105848251296104)
(45, 1.3037522499589698)
(46, 1.261277128171235)
(47, 1.42396294360649)
(48, 0.9720607289556564)
(49, 1.0595241787289287)
(50, 1.0595241787289287)
}


\newcommand{\drawPixelEight}{%
(1, 0.7022906119242012)
(2, 0.38904708973203894)
(3, 0.4226952632187583)
(4, 0.24579109646186004)
(5, 0.9228379095311509)
(6, 1.2094343691925713)
(7, 1.3018675824544788)
(8, 0.9068051615275855)
(9, 0.7701693185465281)
(10, 1.1207815548522135)
(11, 1.243259606222311)
(12, 0.8405526629291109)
(13, 0.6887592817527499)
(14, 0.03751079103071275)
(15, -0.07086184841534399)
(16, -0.7767448163496474)
(17, -0.7223284510141706)
(18, -0.4112507620390341)
(19, -0.06411672333780055)
(20, -0.881998900706256)
(21, -0.4045517467273587)
(22, -0.14291667187392165)
(23, -0.06376356599356817)
(24, -0.4739320570899487)
(25, -0.049359631958515615)
(26, -0.16464122191972635)
(27, -0.7797581908571185)
(28, -0.8970220246812806)
(29, -1.478388677761924)
(30, -1.3444430148988624)
(31, -1.0875443919371703)
(32, -0.6480286962842062)
(33, -0.6567026652604884)
(34, 0.011919001144548358)
(35, -0.24187665538617947)
(36, -0.3303601966042994)
(37, -0.36804108804426505)
(38, -0.30604945885472795)
(39, 0.08104777711884092)
(40, -0.23199002333931537)
(41, -0.19079676132589887)
(42, -0.19733454980037077)
(43, -0.2889628959211758)
(44, 0.19682208345466784)
(45, 0.07748017929842722)
(46, -0.012106807552224166)
(47, -0.020066061602237298)
(48, -0.03403809796796649)
(49, -0.204990177647829)
(50, -0.204990177647829)
}


\newcommand{\drawPixelNine}{%
(1, -0.9604801009757633)
(2, -1.1725958743783802)
(3, -0.8899582664136757)
(4, 0.4937536039769026)
(5, 1.3336954613889713)
(6, 0.7742416470211513)
(7, 1.1629478518037808)
(8, 1.8338074568660736)
(9, 1.4128008828155028)
(10, 1.3664687882523747)
(11, 0.02396204295829296)
(12, 0.5583708512227066)
(13, 0.24635178538856922)
(14, 0.6293852236834392)
(15, 0.16893646929565154)
(16, -0.27025784604460856)
(17, 0.5971295317899987)
(18, 0.11428411502007002)
(19, 0.6262952894177977)
(20, 0.7043409027088925)
(21, 0.36627189469033544)
(22, -0.1495810708839525)
(23, -0.43079229323373514)
(24, -0.33791082859862503)
(25, -0.31111832426617003)
(26, -0.36286211267349333)
(27, -0.20733927338313973)
(28, -0.8212298810031258)
(29, -0.519648783186669)
(30, -0.09495904970630409)
(31, -0.3078184614462851)
(32, -0.30560791961005185)
(33, -0.33339947875853543)
(34, -0.37335459924729786)
(35, -0.2256737693151153)
(36, -0.4534253965463832)
(37, -0.14149655046446513)
(38, 0.16790362961037525)
(39, -0.17086375192212058)
(40, -0.0546111639712798)
(41, -0.33095461850594715)
(42, -0.10085842549723306)
(43, -0.04176852064067495)
(44, -0.06670468306941302)
(45, -0.010693790026815059)
(46, -0.08462154990145584)
(47, -0.016046638686281145)
(48, -0.06401840692545048)
(49, -0.0822845713394004)
(50, -0.0822845713394004)
}


\newcommand{\drawPixelTen}{%
(1, -0.40691059299187016)
(2, 0.6268950740043087)
(3, -0.5195184732084881)
(4, -0.2951194480446336)
(5, 0.36684088686564265)
(6, 0.750126571198056)
(7, 0.40267663533522247)
(8, -0.16764673023453724)
(9, -0.1704610074733351)
(10, -0.7993064683171489)
(11, -0.6084261337078429)
(12, -1.46340958929729)
(13, -1.0768221722104663)
(14, -1.0406129960360568)
(15, -1.522911410028204)
(16, -1.8483748104342723)
(17, -0.36525123034605333)
(18, -0.701070140048871)
(19, -0.43926830079258344)
(20, -0.6501742620878537)
(21, -0.6783694675932903)
(22, -0.9973521848463422)
(23, -1.6366443182452293)
(24, -1.7562513749117024)
(25, -1.6525247433707366)
(26, -1.7153584435790445)
(27, -1.7273977152969509)
(28, -1.5822616312296935)
(29, -1.2968940180991473)
(30, -1.2551272530769058)
(31, -0.8513597134745602)
(32, -1.3478473488751428)
(33, -0.9804746826663242)
(34, -0.4351700100406496)
(35, -0.047492596961549005)
(36, -0.1923823012528404)
(37, -0.28413439384443734)
(38, -0.3687936976414111)
(39, -0.10672210316617112)
(40, -0.39500027720008746)
(41, 0.45725689781015993)
(42, 0.5351079655505855)
(43, 0.2859034684524346)
(44, 0.7080678343276792)
(45, 0.9881662630363468)
(46, 1.0381591472434994)
(47, 0.907766503073683)
(48, 0.8421659807164164)
(49, 1.0485759281094285)
(50, 1.0485759281094285)
}

==> data/drawPixel1_cifar.tex <==
\newcommand{\drawPixelOne}{%
(1, 0.17392996661055038)
(2, 1.3829620872892905)
(3, 1.0901463185889553)
(4, 0.7411301728584286)
(5, 0.106124825395284)
(6, -0.22428202882054243)
(7, 0.18910683680945356)
(8, 0.5781259861655199)
(9, 0.9973314591649534)
(10, 0.4421233010880232)
(11, -0.3135775140157352)
(12, 0.011985779116439277)
(13, -0.4833798198126148)
(14, 0.031403669763862)
(15, -0.06628118553420612)
(16, -0.6477513583211977)
(17, -0.4463003130992287)
(18, -0.2299705352249239)
(19, -0.42237103487688205)
(20, 0.11628666749547156)
(21, 0.9403522951360006)
(22, 0.22495693885957024)
(23, -0.2291223861780638)
(24, -0.31158928285859505)
(25, 0.5889282020211705)
(26, 0.5341405030595181)
(27, 0.5683943680463107)
(28, 0.3915930997881868)
(29, -0.48931155685695504)
(30, 0.3028955792749146)
(31, -0.08009057268088504)
(32, -0.17493987796773713)
(33, -0.3181364023420889)
(34, 0.01673640410397348)
(35, -0.4075820294306886)
(36, -0.2917978956321548)
(37, -0.15120880995012173)
(38, 0.5411302942591965)
(39, 0.7888837025809214)
(40, 0.597305442574043)
(41, 0.32232664716733517)
(42, 0.19637393320537527)
(43, 0.20422604362011673)
(44, -0.030830669754596765)
(45, -0.16441686107866604)
(46, -0.327746216624922)
(47, -0.12969990378673868)
(48, -0.24413299667623153)
(49, -0.28118219983712206)
(50, -0.28118219983712206)
}

\newcommand{\drawPixelTwo}{%
(1, -0.1019826063293881)
(2, 0.53578352081292)
(3, 0.1723098627387153)
(4, 0.43427801105606156)
(5, 1.2458812086253594)
(6, 0.4560375708342743)
(7, 1.5140381377210432)
(8, 0.9198975431423504)
(9, -0.35805654787637897)
(10, 0.16419428831811983)
(11, -0.006878579791059158)
(12, 0.6815521187256874)
(13, 0.42684745288873693)
(14, 0.3006005749783302)
(15, 0.13705980515762028)
(16, 0.5523255007121703)
(17, 0.37962990231977795)
(18, 0.857004957717012)
(19, 0.7476911786824644)
(20, 0.4774766377206955)
(21, 0.9236997902899924)
(22, 0.8117168139467128)
(23, 0.876084817204658)
(24, 0.9467885483246254)
(25, 1.3207031901992823)
(26, 0.11267813428176532)
(27, -0.32631647669805136)
(28, 0.3469142087669016)
(29, -0.022180314755993136)
(30, 0.20135483004609223)
(31, -0.20080223602650485)
(32, 0.02131266904023224)
(33, -0.014172882459475677)
(34, -0.34038553098172114)
(35, -0.2528702440362305)
(36, -0.28278025362734405)
(37, -0.28617526926133785)
(38, 0.30269254218186337)
(39, 0.24498689850292338)
(40, 0.40903372037664404)
(41, 0.39622713806693377)
(42, 0.15280637356815682)
(43, -0.06147407010850783)
(44, 0.09642295535718892)
(45, 0.49192142634436875)
(46, 0.4739137780625331)
(47, 0.45886810291850505)
(48, 0.3824814277784585)
(49, 0.35195662818558265)
(50, 0.35195662818558265)
}

\newcommand{\drawPixelThree}{%
(1, -0.22751267376776613)
(2, -0.6499609429353113)
(3, -0.7690260127260253)
(4, 0.09591141491828103)
(5, 0.20520698206506371)
(6, 1.0705430874337762)
(7, 0.46281463786182153)
(8, 0.8872985840593604)
(9, 1.123699903728526)
(10, 0.9736387394274526)
(11, 0.1482095508653296)
(12, -0.7813024472813719)
(13, -1.4459166390579195)
(14, -0.720891229073595)
(15, -0.7429468850976564)
(16, -0.9800632754641341)
(17, -0.4544756498616065)
(18, -0.6935859349205682)
(19, -0.7843389853352783)
(20, -0.5935290475024123)
(21, -0.4123258780840561)
(22, -0.018537265886554077)
(23, -0.2598368693637707)
(24, -0.5582522159380598)
(25, -0.11038007988330328)
(26, 0.19578565634771256)
(27, -0.8376739921432503)
(28, -1.2298306763868943)
(29, -1.1132600601903322)
(30, -1.4064918268895306)
(31, -0.8548305154091823)
(32, -0.9148942072510219)
(33, -1.0944772487941992)
(34, -0.9118648996743932)
(35, -1.2939242453547048)
(36, -0.697095282886329)
(37, -0.7066066138462967)
(38, -0.6233859499868896)
(39, -0.7293798698479295)
(40, -0.8765689140309556)
(41, -0.5906266139564764)
(42, -0.9263605460814452)
(43, -1.0706779514673097)
(44, -1.1025606550438194)
(45, -0.6396495335997189)
(46, -0.4493511801139645)
(47, -0.24177500420939624)
(48, -0.15307631055867155)
(49, -0.2752028135860503)
(50, -0.2752028135860503)
}

\newcommand{\drawPixelFour}{%
(1, -0.921362634402772)
(2, -1.3064811703061547)
(3, -0.33342100489756277)
(4, -1.2626519055588887)
(5, -0.435450112334139)
(6, -0.27843778596056257)
(7, 0.06736040475478053)
(8, 0.23193409525258574)
(9, 0.5946949155071637)
(10, 0.6269845719021504)
(11, 0.11208989826632754)
(12, 0.5071585432178273)
(13, -0.252361045634691)
(14, -0.1324121201043968)
(15, -0.43050274139627287)
(16, -1.0713020580546457)
(17, -0.6889350210391818)
(18, -1.5439326736577257)
(19, -0.9465460946626936)
(20, -1.0641987845574485)
(21, -1.0232905485996118)
(22, -1.238789758251906)
(23, -0.886036321324983)
(24, -0.01327163810431331)
(25, -0.125683718377692)
(26, -0.7062227628032801)
(27, -1.1862245416583568)
(28, -0.6677855647468134)
(29, -0.7886827575315273)
(30, -1.5294518750824786)
(31, -2.122525848708565)
(32, -1.7691571031490276)
(33, -1.354139265014726)
(34, -1.1420353799975915)
(35, -0.7670225061242145)
(36, -0.21237424618438683)
(37, -0.2298560988011555)
(38, 0.2570584951938814)
(39, 0.10421540253431347)
(40, 0.29251368804145483)
(41, 0.10146155619753378)
(42, 0.03806162028684042)
(43, -0.06920224410474513)
(44, 0.2400438457791983)
(45, 0.20986499174933998)
(46, 0.23987828005956519)
(47, 0.40591797748024094)
(48, 0.2253490142675389)
(49, 0.4505625561067439)
(50, 0.4505625561067439)
}

\newcommand{\drawPixelFive}{%
(1, -0.08458804815403875)
(2, 0.3690136480036238)
(3, 0.4487765549857911)
(4, 0.17778604794335384)
(5, -0.221694359208611)
(6, -0.8635476488691685)
(7, -1.0732577851674676)
(8, 0.02606173535050238)
(9, 0.5247824066381637)
(10, 1.3123157140716557)
(11, 1.4813262483877074)
(12, 0.9331017460458209)
(13, 0.3420984351807351)
(14, 0.7539615165216064)
(15, 0.16610929760509774)
(16, 0.8984941621050673)
(17, 1.0023408450890257)
(18, 1.342946104204471)
(19, 2.2650965937023537)
(20, 1.5212135584520907)
(21, 0.8644424259637373)
(22, 0.8071589838754736)
(23, 1.0739750935710255)
(24, -0.12736660557775203)
(25, -0.6765829389082804)
(26, -1.191716321481715)
(27, -1.3801818874711702)
(28, -1.0628963012047412)
(29, -0.7956235283086927)
(30, -1.183950491504068)
(31, -0.8748425751468994)
(32, -1.0248867885247894)
(33, -1.142782220025465)
(34, -1.1706377581175076)
(35, -1.3758747574976453)
(36, -1.4268656673400681)
(37, -1.1505590197607607)
(38, -1.3929657763837495)
(39, -1.3983523518170666)
(40, -0.955292559802234)
(41, -0.27147729379145413)
(42, -0.4656972680770931)
(43, -0.7702357475872407)
(44, -0.8140021521023306)
(45, -0.23157034879046234)
(46, 0.11514479173613434)
(47, -0.13746593043335797)
(48, -0.1056067881092051)
(49, -0.20213538082737673)
(50, -0.20213538082737673)
}

\newcommand{\drawPixelSix}{%
(1, -0.2666697442121657)
(2, -0.12058092943689225)
(3, 0.21825278710918544)
(4, 1.1594643129862447)
(5, 0.5787034981838592)
(6, -0.1877940730981445)
(7, 0.7733766219059683)
(8, 0.8448622099472511)
(9, 1.251807868671357)
(10, 1.0486469552702222)
(11, 1.1607063473211796)
(12, 1.2171429513684504)
(13, 2.1249818059130803)
(14, 1.7149444726632157)
(15, 1.3311289404694926)
(16, 1.0814916102090844)
(17, 0.7587122050279046)
(18, 1.2783538478104501)
(19, 1.3248572725599992)
(20, 1.3507794217291345)
(21, 1.0038589415737469)
(22, 0.5799496027996351)
(23, 0.9747249984523412)
(24, 1.6064827037183291)
(25, 1.7939951009381223)
(26, 1.3096351094291627)
(27, 0.7413131411739771)
(28, 0.7608911439769929)
(29, 0.29033836965019044)
(30, 0.2972973189720602)
(31, 0.4903799888254132)
(32, 0.7741407391337833)
(33, 0.4144648744233033)
(34, -0.4651867337087606)
(35, -0.2934102950376526)
(36, -0.006502145512565699)
(37, 0.030549715734633404)
(38, -0.22323365046165372)
(39, 0.12662685148874805)
(40, -0.031123509476033984)
(41, 0.13329244624928907)
(42, 0.23767447153317203)
(43, 0.26190747395766023)
(44, 0.35538399498343054)
(45, 0.20846643559393807)
(46, 0.32535598024999296)
(47, 0.08141518268143111)
(48, 0.3834456826452428)
(49, 0.2657229502893318)
(50, 0.2657229502893318)
}

\newcommand{\drawPixelSeven}{%
(1, 0.5789881321868938)
(2, 0.38994299503840824)
(3, -0.5472864806079617)
(4, 0.5671480416665774)
(5, 0.7879236606907561)
(6, 0.6501653837614141)
(7, 0.9584829473902623)
(8, 0.9633977588196099)
(9, 0.8330732882562065)
(10, 0.7498656154594753)
(11, 0.34078587523011783)
(12, 0.6549794560834603)
(13, 0.28307818505734844)
(14, 0.5152946523488091)
(15, -0.4395134333748124)
(16, -0.7560873964791552)
(17, 0.03896174294825239)
(18, -0.12552408960224692)
(19, 0.3191535388095159)
(20, 0.8847538608824198)
(21, 0.5767814061800086)
(22, 0.6445997422684682)
(23, 0.7455419034806139)
(24, 0.3717456480879358)
(25, 0.6909893160093661)
(26, 0.21737542154829387)
(27, 0.06611684155194919)
(28, 0.5276763009608569)
(29, 0.5760945347762298)
(30, 0.46956320952431074)
(31, 0.8655058671610297)
(32, 1.3035806775210244)
(33, 0.8092481110873875)
(34, 0.6322252817832807)
(35, 0.5873826537557831)
(36, 0.31571113073442036)
(37, 0.04787684190306868)
(38, -0.015071687322063154)
(39, 0.30624360342341717)
(40, 0.07448752959911364)
(41, 0.6562610155620751)
(42, 0.5117620550935006)
(43, 0.41594202327219737)
(44, -0.10665093235088685)
(45, 0.16606635283087046)
(46, 0.3566941136954189)
(47, 0.1458201099646958)
(48, 0.265262100012098)
(49, 0.3278268715460201)
(50, 0.3278268715460201)
}

\newcommand{\drawPixelEight}{%
(1, -0.9023073044997127)
(2, -1.1922825668007773)
(3, -0.319478698107325)
(4, -0.9632349329595528)
(5, -0.6274416669459615)
(6, -1.0235550579262105)
(7, -0.4098744636955584)
(8, 0.044438244750380385)
(9, 0.4532494213522277)
(10, -0.2920795814586996)
(11, 0.026059039267529893)
(12, 0.5169630409780692)
(13, 0.1452696920676233)
(14, 0.30526793908466265)
(15, 0.3638349128192686)
(16, 0.1410599675788261)
(17, 0.07955886049473603)
(18, -0.2822213238029559)
(19, 0.11367051362876926)
(20, 0.21784936622166295)
(21, 0.5267370702802019)
(22, -0.04251917634067148)
(23, 0.4885643626954987)
(24, 0.6701447698905738)
(25, 0.7263666341606153)
(26, 0.41820734361512485)
(27, 0.5663049447437066)
(28, 0.4589607937577661)
(29, 0.23909260548721534)
(30, 0.8975554610030875)
(31, 1.037065052658587)
(32, 0.561970625026069)
(33, 0.5275129580542148)
(34, 0.35610910768476667)
(35, 0.06839613249392612)
(36, 0.22768886357149892)
(37, -0.026457543406996242)
(38, -0.3617819099924031)
(39, -0.18321849693788375)
(40, -0.1655905098107561)
(41, -0.20578600353878837)
(42, -0.27288500378485353)
(43, -0.0032162284187129686)
(44, -0.05560906161275175)
(45, 0.35621861298055296)
(46, 0.20474913296474184)
(47, 0.20312961445151198)
(48, 0.2995389533253857)
(49, 0.26821986863421377)
(50, 0.26821986863421377)
}

\newcommand{\drawPixelNine}{%
(1, 1.3477174341532936)
(2, 1.7045621772950756)
(3, 0.5742986402944532)
(4, 0.00043362757179499223)
(5, 0.2563489678761257)
(6, 0.7599214451431564)
(7, 0.4011041345900965)
(8, 0.45136835057630487)
(9, 0.8816951254264873)
(10, 0.8119743491262728)
(11, 0.43094078613501907)
(12, 0.7970104064995428)
(13, 0.2056696310756181)
(14, 0.8147105148919027)
(15, 0.34702215535195546)
(16, 0.8883463029766995)
(17, 1.1526872007431714)
(18, 1.2658953316095523)
(19, 1.0745693365294817)
(20, 0.5468602185871232)
(21, 0.8526851525358304)
(22, 0.15804930959862684)
(23, 0.1329013778902215)
(24, 0.4895578303436239)
(25, 0.4779856232422792)
(26, 0.1285632469461278)
(27, 0.18377702545684016)
(28, 0.11018099733463277)
(29, -0.10752553036089565)
(30, 0.3855338371782936)
(31, 0.3199095313817024)
(32, 0.9385560944839337)
(33, 1.7055664146119731)
(34, 1.5888436440910043)
(35, 1.956084486183382)
(36, 2.3274139735280768)
(37, 2.1869701729500637)
(38, 1.7799679521906722)
(39, 1.2628736434944083)
(40, 1.4756065727742067)
(41, 1.030051788190371)
(42, 0.9525436025663065)
(43, 0.9648606143107599)
(44, 0.9995958068621902)
(45, 0.9835824767252982)
(46, 0.770034850907075)
(47, 0.6871262377441385)
(48, 0.35573160550917504)
(49, 0.4889637747155925)
(50, 0.4889637747155925)
}

\newcommand{\drawPixelTen}{%
(1, 0.3780769052378369)
(2, 1.2656045503772682)
(3, 1.0862376319485623)
(4, -0.3673930658699871)
(5, 0.6406018646353451)
(6, 0.5013662816595577)
(7, 0.07965548312665843)
(8, 0.5629475899212915)
(9, 0.4037056486868226)
(10, 0.4279023152357654)
(11, 1.0904605872585924)
(12, 0.4123275080197195)
(13, 0.53609238582394)
(14, 0.261584600096772)
(15, 0.8005938296494411)
(16, 1.2687673562567374)
(17, 1.4001693038726697)
(18, 1.5179157157959686)
(19, 1.8635521832525308)
(20, 2.4310534668305386)
(21, 1.8242470149016397)
(22, 1.5822781538661466)
(23, 2.0190129057058366)
(24, 2.3928002831739814)
(25, 2.6190354746308797)
(26, 1.9748187237797115)
(27, 1.2769849679322143)
(28, 1.5470325942499839)
(29, 1.2866954553111474)
(30, 0.6478056481967567)
(31, 1.1445277233640614)
(32, 1.5645447358976305)
(33, 1.4801429517045208)
(34, 1.2055054301245607)
(35, 0.3934757949701623)
(36, 0.3100689351695053)
(37, 0.2993455878418668)
(38, 0.3812685993344404)
(39, 0.717532450822092)
(40, 0.8005309958673101)
(41, 0.8262406861718226)
(42, 0.8068803526648762)
(43, 0.44362035704709024)
(44, 0.230441529494156)
(45, 0.28397060244491223)
(46, 0.5610741353305909)
(47, 0.37233000686496737)
(48, 0.330277565318163)
(49, 0.3712421463657944)
(50, 0.3712421463657944)
}

==> data/drawPixel2.tex <==
\newcommand{\drawPixelOne}{%
(1, -0.7115084427956856)
(2, -0.7287448082676735)
(3, -0.6214345868747159)
(4, -0.9924715052412099)
(5, -1.2444825040692538)
(6, -0.7443677777399779)
(7, -1.2351794547024586)
(8, -0.8383512090495794)
(9, -0.6610799588165728)
(10, 0.03326101353098687)
(11, 0.044455573430982054)
(12, 0.9354470815058619)
(13, 0.9093711705235112)
(14, -0.005303390996401647)
(15, 0.08873943169791862)
(16, -0.4918205630433792)
(17, -0.2710376903540525)
(18, 0.7553466336979201)
(19, 1.0812869386347272)
(20, 0.8044954448972573)
(21, 0.5439941891994677)
(22, 0.04212314582627186)
(23, 0.21376325634301072)
(24, 0.06680078982436735)
(25, 0.23454325866812564)
(26, -0.09981311071001231)
(27, 0.34715598500290057)
(28, 0.08375025403906675)
(29, -0.3345827971268508)
(30, -0.883282588617994)
(31, -1.0099701454340715)
(32, -1.0190694145328518)
(33, -0.8503575009466542)
(34, -0.6961178578049105)
(35, -0.8915642934124449)
(36, -0.933152829340242)
(37, -0.9686455701639212)
(38, -0.7850103689831401)
(39, -0.6467042491722143)
(40, -0.708648234674637)
(41, -0.7108230292140268)
(42, -0.7114276705337313)
(43, -0.6957800608469078)
(44, -0.6711032775885203)
(45, -0.6822830282170906)
(46, -0.684170034690237)
(47, -0.6811041998741056)
(48, -0.6779795600219058)
(49, -0.6746284069394977)
(50, -0.6746284069394977)
}


\newcommand{\drawPixelTwo}{%
(1, 0.2395344200868873)
(2, -0.9632128552497927)
(3, -0.924329350730266)
(4, -0.3405574680738289)
(5, -0.23362063628045093)
(6, 0.8656294925174175)
(7, 0.09386215855054802)
(8, 0.23508818829532102)
(9, -0.40083934689293577)
(10, -0.05050332902348442)
(11, 0.34682466725215794)
(12, 1.1261233067729606)
(13, 2.027606257461723)
(14, 2.09766951156392)
(15, 2.3059382186301316)
(16, 1.7351348008062417)
(17, 0.3380487846711071)
(18, 0.39968961254393987)
(19, 0.35859219038462264)
(20, -0.4236695378873719)
(21, -0.26041275456143315)
(22, -0.5388008587512273)
(23, 0.008245065314652855)
(24, 0.14324996345695437)
(25, 0.5416167568654027)
(26, 0.5785641029901676)
(27, 0.637447397961554)
(28, 0.8815722765787498)
(29, 0.24677303943151452)
(30, 0.6432566585232565)
(31, 0.9076396498782239)
(32, 0.8518454527836749)
(33, 0.4304514216704387)
(34, 0.5077479078656657)
(35, 0.6718880772381505)
(36, 0.9105484846095921)
(37, 0.8985630557927328)
(38, 0.9279926881659865)
(39, 1.0160797436447342)
(40, 1.0370696605665042)
(41, 1.0064509530771963)
(42, 1.0182084607073854)
(43, 0.9890155344270946)
(44, 0.9670563519743285)
(45, 0.9494851983384679)
(46, 0.9389759533131514)
(47, 0.9352203537805865)
(48, 0.9327964321206981)
(49, 0.9346896134148641)
(50, 0.9346896134148641)
}

\newcommand{\drawPixelThree}{%
(1, 1.8826929065315647)
(2, 1.6418914086081924)
(3, 1.7228137288454715)
(4, 1.7115792234184748)
(5, 2.7759042182197535)
(6, 1.9954576255233714)
(7, 2.8232698746183313)
(8, 1.787488823243998)
(9, 0.8285649625081091)
(10, 1.4148879872637323)
(11, 1.2226141053012796)
(12, 1.2990669290697037)
(13, 1.0557205191054622)
(14, -0.2103029742901208)
(15, -0.11563260005756446)
(16, 0.14491624949434687)
(17, -0.22795896856048536)
(18, -0.8986214350582098)
(19, -0.18229785056339842)
(20, -0.09524069943282146)
(21, -0.5557339856878838)
(22, -0.8268017736191391)
(23, -0.8851734350718914)
(24, -1.3062988676491418)
(25, -0.7618205518764314)
(26, -0.16328029547053546)
(27, -0.5379562008462346)
(28, -0.4371146543483765)
(29, -0.828521903443957)
(30, -0.6992718656644554)
(31, -0.6016606677123758)
(32, -0.30875152868675104)
(33, -0.7117751061910413)
(34, -0.5706328018861611)
(35, -0.17736340754903968)
(36, -0.24473555423561272)
(37, -0.1470387259575453)
(38, -0.13510876616624834)
(39, -0.1450693123435675)
(40, -0.21273370219883622)
(41, -0.21881912312380317)
(42, -0.26622146625721177)
(43, -0.26240576042058217)
(44, -0.24948053817128182)
(45, -0.25148983744215264)
(46, -0.251776967804229)
(47, -0.2484291567098393)
(48, -0.24505809260153466)
(49, -0.24586502896462736)
(50, -0.24586502896462736)
}


\newcommand{\drawPixelFour}{%
(1, 0.9216292194485687)
(2, 1.3013279342687842)
(3, 1.1856287932247036)
(4, 1.1650420435153108)
(5, 0.914207664635465)
(6, 1.10596198999531)
(7, 0.8355039598791294)
(8, 0.5327115405515408)
(9, 1.417264930396843)
(10, 0.5673598017397966)
(11, 0.7116533980954896)
(12, 0.4489946746695675)
(13, -0.25517877256153565)
(14, 0.5220214723420528)
(15, -0.4926333037261318)
(16, -0.7010499782267583)
(17, -1.3702444591531246)
(18, -1.6839480060187002)
(19, -0.9773366253108062)
(20, -0.876331376788059)
(21, -0.5680282587137329)
(22, -0.16295515209863115)
(23, -0.43607411164774357)
(24, -0.47237225662202675)
(25, -0.1965225319878918)
(26, -0.7890337224392158)
(27, -0.7235822565575182)
(28, -0.6042465675023928)
(29, 0.6615544310860708)
(30, 1.530556715506075)
(31, 1.3457376532292906)
(32, 1.60988366528265)
(33, 1.7179670994029714)
(34, 1.4294280188295152)
(35, 1.2030643341068452)
(36, 1.0942226081581734)
(37, 1.0419777226520675)
(38, 0.774538019212295)
(39, 0.725382524676914)
(40, 0.753787913847426)
(41, 0.8208235513199477)
(42, 0.8568760484916753)
(43, 0.8481864659105978)
(44, 0.8413338006124773)
(45, 0.8303458834811311)
(46, 0.8271899250658563)
(47, 0.8382238327676106)
(48, 0.835323610773884)
(49, 0.8355380935318523)
(50, 0.8355380935318523)
}


\newcommand{\drawPixelFive}{%
(1, -1.4795184932147383)
(2, -1.2849095239852466)
(3, -1.2704980023719463)
(4, -1.0085219328748427)
(5, -0.3739528890020901)
(6, 0.19415125943729034)
(7, 0.6694359233475728)
(8, 0.32436868528705254)
(9, 0.1948220373859894)
(10, 0.312925266369315)
(11, -0.11193834061321395)
(12, 0.12284103304859631)
(13, 0.7113086467254355)
(14, 0.22845326572552388)
(15, 0.6265612132538437)
(16, 0.13505187543259112)
(17, -0.11335248150747157)
(18, 0.5107474796588758)
(19, 0.44314920616003195)
(20, 0.10743809132162452)
(21, -0.562236685216877)
(22, -0.5741365717470972)
(23, -1.3314585030233081)
(24, -0.7021715935415831)
(25, -1.0089785778097267)
(26, -1.0834669891862425)
(27, -0.6249416769912834)
(28, -0.22206346954234513)
(29, -0.2628375053626744)
(30, -1.178077622294694)
(31, -0.7415960056781992)
(32, -0.3668372999412394)
(33, 0.14024860906962533)
(34, -0.12743854204756744)
(35, -0.043201437159347766)
(36, -0.010350349504703815)
(37, -0.23329984787774352)
(38, -0.32936635267280984)
(39, -0.2696180401626882)
(40, -0.35467917096255624)
(41, -0.4186574236121107)
(42, -0.38609970079950473)
(43, -0.385792319123691)
(44, -0.3914122271952821)
(45, -0.4009923429679798)
(46, -0.41397934304261724)
(47, -0.4236229868624575)
(48, -0.42373087160573075)
(49, -0.42447011815405733)
(50, -0.42447011815405733)
}


\newcommand{\drawPixelSix}{%
(1, 0.9479092206803386)
(2, 1.6969892002714388)
(3, 1.7580153879487157)
(4, 1.337827597402097)
(5, 1.0489380279332163)
(6, 0.9340347277150135)
(7, 0.8833484218757474)
(8, 0.8865292794069558)
(9, 0.47687971407770224)
(10, 0.46510299540589706)
(11, 0.20268441152544425)
(12, 0.16813529472339458)
(13, -0.06504787978973275)
(14, -0.8807020327060822)
(15, -0.9366537925284614)
(16, 0.03334770410962884)
(17, -0.14470540526623538)
(18, 0.568943516843133)
(19, 1.0744199059176223)
(20, 1.3977283568993975)
(21, 1.1678148110646918)
(22, 1.6627589722167477)
(23, 1.762512133232051)
(24, 1.652094789455153)
(25, 1.772116032546236)
(26, 1.9391611723971551)
(27, 0.9676690208816936)
(28, 0.4766151730974262)
(29, 0.42767784245543394)
(30, 0.803649275363312)
(31, 1.0876164899785177)
(32, 0.8104904934975901)
(33, 1.2367279092057246)
(34, 1.2830798779886257)
(35, 0.920147888552797)
(36, 1.001579905414223)
(37, 1.0800277955655668)
(38, 1.0703741383364567)
(39, 1.0256555757075665)
(40, 0.9899505761453162)
(41, 0.9849205016079595)
(42, 1.0204561277651223)
(43, 1.0149749704144788)
(44, 1.0258701459065322)
(45, 1.0120581746418946)
(46, 1.0069942707042165)
(47, 1.0014279542677438)
(48, 1.0031475465834274)
(49, 1.0022779062367402)
(50, 1.0022779062367402)
}


\newcommand{\drawPixelSeven}{%
(1, 0.6076150993401166)
(2, 0.16559275204173818)
(3, 0.10808401853002834)
(4, 0.5047595176970874)
(5, 0.2670418153875297)
(6, 1.0317189008032377)
(7, 1.0478581388954131)
(8, 1.2951802018140275)
(9, 1.2977984177217345)
(10, 1.053686130888478)
(11, 0.633205083090461)
(12, 0.8716533180205189)
(13, 1.2064037760094735)
(14, 1.332133536192943)
(15, 1.407725928350368)
(16, 1.8555158955796462)
(17, 0.9612914045921722)
(18, 2.140093787253944)
(19, 1.5184305718638489)
(20, 0.9521316735392011)
(21, 0.8161871135626798)
(22, 1.4232630988774102)
(23, 0.5914144398949621)
(24, 1.079537197212674)
(25, 2.247143752030146)
(26, 1.4302917793211645)
(27, 1.4141364084797374)
(28, 0.9873872005853925)
(29, 0.8889847702265026)
(30, 1.0934593947039688)
(31, 0.5855635650475923)
(32, 0.4248314930260753)
(33, 0.62430256191447)
(34, 0.7024786118019564)
(35, 0.7311367547994942)
(36, 0.7453090774031832)
(37, 0.9118227919991405)
(38, 1.0161641096202365)
(39, 0.9848949528941728)
(40, 1.0561779306240502)
(41, 1.086493523167291)
(42, 1.0178237800181547)
(43, 1.000687026688268)
(44, 1.021596823489354)
(45, 1.0146773592949996)
(46, 1.0101183301148424)
(47, 1.0165211867395747)
(48, 1.0020570072722137)
(49, 1.0022148856456108)
(50, 1.0022148856456108)
}


\newcommand{\drawPixelEight}{%
(1, 0.4274817685777844)
(2, 0.2381835493216821)
(3, 0.28694373866470474)
(4, 0.18219704453537836)
(5, 0.7692078470705142)
(6, 1.0434382641320665)
(7, 1.1596074968616854)
(8, 0.8430630577301668)
(9, 0.7519697484357426)
(10, 1.0812088786598535)
(11, 1.2217399386088577)
(12, 0.8450741610776278)
(13, 0.6998766424596197)
(14, 0.04857130870382398)
(15, -0.06381737605944757)
(16, -0.8001747066485282)
(17, -0.7396772896828716)
(18, -0.38570183046157597)
(19, -0.0014782957123581353)
(20, -0.9579475133770876)
(21, -0.372301784190163)
(22, -0.07339806915921732)
(23, 0.011462806226112718)
(24, -0.5020863828904398)
(25, 0.020170088164803368)
(26, -0.17615312309279685)
(27, -0.9510403082998411)
(28, -1.0112709809126124)
(29, -1.5899435556934294)
(30, -1.2722238328464874)
(31, -0.8733026018296368)
(32, -0.39117990130634284)
(33, -0.39359000864076166)
(34, 0.0219743542038231)
(35, -0.2150815399494026)
(36, -0.29389519651204077)
(37, -0.3236620673532692)
(38, -0.3179020027981914)
(39, -0.22237569633164672)
(40, -0.30158141498482527)
(41, -0.29168259832288573)
(42, -0.2908232487040038)
(43, -0.30250460017756803)
(44, -0.26554669538617004)
(45, -0.27309247212890647)
(46, -0.2770892735465932)
(47, -0.2759158932686962)
(48, -0.27462020639523865)
(49, -0.27795976718907023)
(50, -0.27795976718907023)
}


\newcommand{\drawPixelNine}{%
(1, -1.0027354095535794)
(2, -1.1953485341691654)
(3, -1.0040731415864792)
(4, 0.14215635810950333)
(5, 0.8951216791100122)
(6, 0.50705652546296)
(7, 0.9009253040411311)
(8, 1.5538330951719335)
(9, 1.2364297853197894)
(10, 1.2310442243828228)
(11, -0.002899332530666321)
(12, 0.5074237171760339)
(13, 0.20900300489588863)
(14, 0.596079850737872)
(15, 0.12831469177724264)
(16, -0.3293896073206312)
(17, 0.6012400764525136)
(18, 0.06685670866715887)
(19, 0.6275166082396867)
(20, 0.7123147325300844)
(21, 0.30283353454006245)
(22, -0.3404634891437247)
(23, -0.6353678091642785)
(24, -0.49132300059221706)
(25, -0.4206489731033974)
(26, -0.4889920910444969)
(27, -0.2827456024405483)
(28, -0.9978508925293884)
(29, -0.5917925917576392)
(30, -0.10775995721229226)
(31, -0.3521605802550609)
(32, -0.3868007120734834)
(33, -0.43779944727238745)
(34, -0.4674515943233647)
(35, -0.39854650905394423)
(36, -0.5087988961490453)
(37, -0.3913360293044926)
(38, -0.3182040825341875)
(39, -0.415399840749745)
(40, -0.38825875633890183)
(41, -0.43934865882326196)
(42, -0.40898246506386426)
(43, -0.39783571250035504)
(44, -0.40124667525395874)
(45, -0.3929005873159272)
(46, -0.3945322024994708)
(47, -0.38917273694682897)
(48, -0.3896513406465962)
(49, -0.3902643040472015)
(50, -0.3902643040472015)
}


\newcommand{\drawPixelTen}{%
(1, -0.443516520409119)
(2, 0.37331821161268886)
(3, -0.5203045057566111)
(4, -0.3451108232954702)
(5, 0.20504150501120427)
(6, 0.561519766293544)
(7, 0.2932792762667903)
(8, -0.18172065933859116)
(9, -0.1868574122579294)
(10, -0.7735318315267329)
(11, -0.6070156498530014)
(12, -1.4339192058376113)
(13, -1.0686334093383207)
(14, -1.037052679848398)
(15, -1.5312145619632798)
(16, -1.8627028123035536)
(17, -0.2738802398247717)
(18, -0.6554816338746141)
(19, -0.3594332717632144)
(20, -0.5863412237093392)
(21, -0.5864198832130649)
(22, -0.9356850498052321)
(23, -1.639050481624829)
(24, -1.661710969442513)
(25, -1.4143013751904463)
(26, -1.353489868155287)
(27, -1.2175697287299587)
(28, -0.8748092819393446)
(29, -0.36315545767068563)
(30, -0.1875328398556874)
(31, 0.3501085883088153)
(32, -0.02385478264603713)
(33, 0.37305427660982005)
(34, 0.7721668685908841)
(35, 0.9709299549712871)
(36, 0.8653994383558903)
(37, 0.8125091165238226)
(38, 0.8117114114100334)
(39, 0.8978234426234781)
(40, 0.8466057721486371)
(41, 0.991604260366736)
(42, 0.9806169215858402)
(43, 0.9394595753195837)
(44, 0.9648546983923315)
(45, 0.9741231516475896)
(46, 0.9711298397834968)
(47, 0.962791230164047)
(48, 0.9569663676067475)
(49, 0.9595703256568239)
(50, 0.9595703256568239)
}

==> data/drawPixel2_cifar.tex <==
\renewcommand{\drawPixelOne}{%
(1, 0.14842306009351108)
(2, 1.117868914305072)
(3, 0.9680576536923721)
(4, 0.7153156247872583)
(5, 0.18878692799166574)
(6, -0.11067275717068309)
(7, 0.23848015919756166)
(8, 0.5795651347066416)
(9, 0.9639463287182441)
(10, 0.4592557440156242)
(11, -0.24136547667951963)
(12, 0.061372185715973415)
(13, -0.4293163666410197)
(14, 0.07628835976398135)
(15, -0.029711952300368744)
(16, -0.6360724562983051)
(17, -0.4222838333031313)
(18, -0.19335023676469248)
(19, -0.39987725005302666)
(20, 0.21853524781927852)
(21, 1.1510831840974507)
(22, 0.26052277761358655)
(23, -0.2886938654002502)
(24, -0.3535932791637761)
(25, 0.7793131699899741)
(26, 0.6205534557378358)
(27, 0.6419395162207813)
(28, 0.36594195077086994)
(29, -0.6865429994130187)
(30, 0.20388309215999867)
(31, -0.27659916558064007)
(32, -0.3676160221720419)
(33, -0.45458657109110656)
(34, -0.18951386491289046)
(35, -0.4287507714291432)
(36, -0.34670335317966533)
(37, -0.29821685913595203)
(38, -0.10958012626574043)
(39, -0.09081155031051723)
(40, -0.15838276346554492)
(41, -0.19972244864172947)
(42, -0.217635439135102)
(43, -0.22469568314243918)
(44, -0.2496654261803868)
(45, -0.25876013438730716)
(46, -0.2664403665419171)
(47, -0.26058837801564644)
(48, -0.2643335630428869)
(49, -0.2663977868353678)
(50, -0.2663977868353678)
}

\renewcommand{\drawPixelTwo}{%
(1, -0.00281187435261393)
(2, 0.5081154849018441)
(3, 0.24079158295085104)
(4, 0.44981527183248754)
(5, 1.1519330548734221)
(6, 0.5258375213775583)
(7, 1.4442383972640682)
(8, 0.9397977377714768)
(9, -0.20295754182444203)
(10, 0.24607068077261793)
(11, 0.0864143721399029)
(12, 0.7423997797505041)
(13, 0.48908473407520325)
(14, 0.35380663054406364)
(15, 0.17788486956232683)
(16, 0.6042435621454312)
(17, 0.4042532680251694)
(18, 0.9190278550559445)
(19, 0.7750043709417858)
(20, 0.4396010737859427)
(21, 0.9538267569312749)
(22, 0.7928567639987305)
(23, 0.852198906547476)
(24, 0.8958040770137498)
(25, 1.3103076451883808)
(26, -0.2713865169164291)
(27, -0.7060778027947111)
(28, 0.14145785148933543)
(29, -0.24759223601346056)
(30, 0.087889344412544)
(31, -0.2740927860653765)
(32, 0.008489395735228195)
(33, -0.00589869320981775)
(34, -0.17785017639697376)
(35, -0.05659153009371592)
(36, -0.024244649579153524)
(37, 0.03158028590885969)
(38, 0.27525515001985823)
(39, 0.2660461441702816)
(40, 0.29695746318514604)
(41, 0.2817492517347453)
(42, 0.24202360699120315)
(43, 0.22218422960369907)
(44, 0.23626673125063705)
(45, 0.26714746490759006)
(46, 0.26709265293589246)
(47, 0.26826846568894025)
(48, 0.2662542413996765)
(49, 0.26975937066339223)
(50, 0.26975937066339223)
}

\renewcommand{\drawPixelThree}{%
(1, -0.2805874127782111)
(2, -0.6442803656848134)
(3, -0.7788063074904767)
(4, -0.09099409365155564)
(5, 0.01885696595771466)
(6, 0.8025368143553411)
(7, 0.32603972431780015)
(8, 0.718717751511559)
(9, 0.9747033176420934)
(10, 0.8502343039276741)
(11, 0.10370736374636125)
(12, -0.780897012747447)
(13, -1.4327190065826771)
(14, -0.7127421575616503)
(15, -0.7374533094951492)
(16, -0.9801530735794178)
(17, -0.4188999611800591)
(18, -0.6648533359007325)
(19, -0.7570225418733337)
(20, -0.5253796964796571)
(21, -0.3339448697631684)
(22, 0.1084409675397982)
(23, -0.20462485926076654)
(24, -0.5697051308818948)
(25, -0.013253170014771554)
(26, 0.29843577247392944)
(27, -1.0013630888827985)
(28, -1.3021007477566373)
(29, -1.0802567183583174)
(30, -1.2579289040658055)
(31, -0.5964389114299034)
(32, -0.6318191677881699)
(33, -0.730825445207311)
(34, -0.524064668555444)
(35, -0.6960778837455874)
(36, -0.3356300055383813)
(37, -0.34032238599039927)
(38, -0.3062572072533381)
(39, -0.32537728458384574)
(40, -0.33537103496645015)
(41, -0.2694021899621832)
(42, -0.3056129088960715)
(43, -0.3160345019050782)
(44, -0.32177317421071405)
(45, -0.29200847654272283)
(46, -0.28396461644820775)
(47, -0.273432939180269)
(48, -0.26830820990836707)
(49, -0.26869993428260835)
(50, -0.26869993428260835)
}

\renewcommand{\drawPixelFour}{%
(1, -0.7377871521604006)
(2, -1.1250206544717885)
(3, -0.3998819788634601)
(4, -1.1950153574801798)
(5, -0.5486010886640609)
(6, -0.4267649162261374)
(7, -0.13191934041211045)
(8, 0.024328434597660674)
(9, 0.3624064145248836)
(10, 0.42872968188904137)
(11, -0.03271702358944406)
(12, 0.3576805598959859)
(13, -0.36430272393838586)
(14, -0.2309399204610826)
(15, -0.5233655583180714)
(16, -1.178881311731299)
(17, -0.7548554764952561)
(18, -1.65911205586702)
(19, -0.9573738667110069)
(20, -1.0630544883110666)
(21, -1.0003644785206867)
(22, -1.2132441191905632)
(23, -0.748858984569442)
(24, 0.3028399851832235)
(25, 0.10508841705391941)
(26, -0.6374866760972385)
(27, -1.157785833262131)
(28, -0.4852060902186337)
(29, -0.5886963698255318)
(30, -1.3434082981517677)
(31, -1.7879208175756887)
(32, -1.2813636218422864)
(33, -0.8661396019520633)
(34, -0.6989503471665185)
(35, -0.49898093517885567)
(36, -0.2967871189643902)
(37, -0.36434078396930303)
(38, -0.23813374978175333)
(39, -0.302704791644895)
(40, -0.275807906945036)
(41, -0.3285980286794034)
(42, -0.34723176182364546)
(43, -0.36680425697396807)
(44, -0.34427645206409047)
(45, -0.35047246937350635)
(46, -0.3481442567883172)
(47, -0.34049436431361707)
(48, -0.34580438390318)
(49, -0.3398819304702267)
(50, -0.3398819304702267)
}

\renewcommand{\drawPixelFive}{%
(1, -0.1384314243001296)
(2, 0.2550811371772255)
(3, 0.3194773542592515)
(4, 0.13641715676617833)
(5, -0.15727784940694872)
(6, -0.7030869679158964)
(7, -0.9009243720855518)
(8, 0.038258754651344096)
(9, 0.5022428316086114)
(10, 1.2391923234290232)
(11, 1.4217319117660216)
(12, 0.9090692779394453)
(13, 0.3386683673039692)
(14, 0.7476003463498299)
(15, 0.1454904861445453)
(16, 0.9109206685340853)
(17, 1.0162421406784947)
(18, 1.3786863881812748)
(19, 2.3653011905070684)
(20, 1.476069884569002)
(21, 0.6797674121664941)
(22, 0.6029774739118259)
(23, 0.9419970207510274)
(24, -0.5397760551473296)
(25, -1.1461999861677419)
(26, -1.651001013157945)
(27, -1.690366324116944)
(28, -1.1401372107002878)
(29, -0.7184896109766308)
(30, -1.0684302490119566)
(31, -0.662392359732931)
(32, -0.733177871294217)
(33, -0.7535330378320921)
(34, -0.7031814666388465)
(35, -0.7373967638895873)
(36, -0.6806137853297863)
(37, -0.5300937683249747)
(38, -0.5852373338800226)
(39, -0.5531372750219937)
(40, -0.43729070570132333)
(41, -0.32438966532393243)
(42, -0.35651314255980915)
(43, -0.39197340841475625)
(44, -0.39705722072089616)
(45, -0.3617125483694894)
(46, -0.345932480567623)
(47, -0.35433171699611166)
(48, -0.35259180801352674)
(49, -0.3538730723721946)
(50, -0.3538730723721946)
}

\renewcommand{\drawPixelSix}{%
(1, -0.24996419971542613)
(2, -0.1616868623762063)
(3, 0.12071376796802791)
(4, 0.9099617439032626)
(5, 0.47999598240568986)
(6, -0.13058011591661045)
(7, 0.7078339533443194)
(8, 0.7838617787164694)
(9, 1.1571463761102019)
(10, 0.9840685598312818)
(11, 1.1104848271396082)
(12, 1.1749141130303309)
(13, 2.0707258878340062)
(14, 1.670215267245334)
(15, 1.280989275869565)
(16, 1.0175151568839809)
(17, 0.6797762895823336)
(18, 1.2488233003166471)
(19, 1.283225347859459)
(20, 1.2811301151573964)
(21, 0.8689147711478118)
(22, 0.3630886598207469)
(23, 0.8681476126549574)
(24, 1.633157888590485)
(25, 1.7825467798335242)
(26, 1.0888106282099366)
(27, 0.37908757986439345)
(28, 0.43222627242217976)
(29, -0.045246453225527894)
(30, 0.0319903518703654)
(31, 0.25026368826763434)
(32, 0.5085504275507802)
(33, 0.2241562387281505)
(34, -0.30239762198695763)
(35, -0.06918370595979323)
(36, 0.12795292473711753)
(37, 0.1562922047263031)
(38, 0.10081230018121884)
(39, 0.22391137936670746)
(40, 0.20000111766748202)
(41, 0.23165232398482213)
(42, 0.23988922928184456)
(43, 0.23397410621573086)
(44, 0.23787531099998926)
(45, 0.2247661931413959)
(46, 0.2281785239009836)
(47, 0.21874053408560357)
(48, 0.2280033963652002)
(49, 0.2282500857008032)
(50, 0.2282500857008032)
}

\renewcommand{\drawPixelSeven}{%
(1, 0.5711387357529485)
(2, 0.4312708886799774)
(3, -0.3173556679097801)
(4, 0.5655371972418319)
(5, 0.7450593268854473)
(6, 0.6611858339581235)
(7, 0.9538648849040419)
(8, 0.9834894412418184)
(9, 0.8759069466833164)
(10, 0.8083530042341007)
(11, 0.4160567608581013)
(12, 0.7091729381913863)
(13, 0.3356797356257258)
(14, 0.5595742867982348)
(15, -0.4202749754065347)
(16, -0.751490577600122)
(17, 0.097182609671846)
(18, -0.0986443009944771)
(19, 0.3885826147912241)
(20, 0.9946888122634563)
(21, 0.6067979516655678)
(22, 0.6707954078438483)
(23, 0.7382679386122066)
(24, 0.22293411615009495)
(25, 0.5760333867212584)
(26, -0.02356204105864057)
(27, -0.13184213234909004)
(28, 0.5014838730257772)
(29, 0.5029990889211324)
(30, 0.4007644965373942)
(31, 0.7711068682246023)
(32, 1.0736570354521437)
(33, 0.5625773681809505)
(34, 0.46760164975587554)
(35, 0.4900263350456375)
(36, 0.3855133109465242)
(37, 0.3135146161192561)
(38, 0.3440336694521438)
(39, 0.4594009147080185)
(40, 0.4246515684523558)
(41, 0.5276476812848196)
(42, 0.5050788278072252)
(43, 0.4931721804524339)
(44, 0.4530017116660484)
(45, 0.4744793708447109)
(46, 0.4883168517095013)
(47, 0.482920046920351)
(48, 0.4846271221941868)
(49, 0.4873516921388272)
(50, 0.4873516921388272)
}

\renewcommand{\drawPixelEight}{%
(1, -0.9075653738664943)
(2, -1.1810815833567885)
(3, -0.512774503388024)
(4, -1.024095851750803)
(5, -0.7500995064982334)
(6, -1.100186547399492)
(7, -0.588772763616074)
(8, -0.1643838607673408)
(9, 0.23642508761137032)
(10, -0.4127967420494749)
(11, -0.10174499189066333)
(12, 0.38247188620352196)
(13, 0.03703114616952874)
(14, 0.20859806714302537)
(15, 0.27859419888812753)
(16, 0.05019100978830343)
(17, -0.011139576949115847)
(18, -0.3957249989114217)
(19, 0.07349074627642543)
(20, 0.19685517507089972)
(21, 0.5411787017996607)
(22, -0.14343118194597393)
(23, 0.49898666444652906)
(24, 0.698139078785255)
(25, 0.7341430246987297)
(26, 0.314038297028046)
(27, 0.5060357581472625)
(28, 0.3839683826865772)
(29, 0.20903922140678532)
(30, 0.9377207744149955)
(31, 1.0076941254289402)
(32, 0.5637264994621857)
(33, 0.5512819264189823)
(34, 0.49286939367616234)
(35, 0.4192590612453457)
(36, 0.5559752418919393)
(37, 0.4956014774730922)
(38, 0.4338182240979257)
(39, 0.525831029224981)
(40, 0.5352847893605732)
(41, 0.5398164634005137)
(42, 0.5411697029900167)
(43, 0.5689966125612934)
(44, 0.5610531782033752)
(45, 0.5895786853203928)
(46, 0.5846233266720733)
(47, 0.5859584786648808)
(48, 0.5871833040792428)
(49, 0.584771636915146)
(50, 0.584771636915146)
}

\renewcommand{\drawPixelNine}{%
(1, 1.207086252091896)
(2, 1.533368417742385)
(3, 0.6887055015505598)
(4, 0.18527503954507685)
(5, 0.37481139929567964)
(6, 0.8054754519036016)
(7, 0.5181668297260718)
(8, 0.5476154873180332)
(9, 0.9330311531430164)
(10, 0.878363835202886)
(11, 0.5159082999917611)
(12, 0.8614816031880626)
(13, 0.27571259300169004)
(14, 0.872661593286336)
(15, 0.3853215957247954)
(16, 0.9344941066883614)
(17, 1.1916747310069538)
(18, 1.2923811058745514)
(19, 1.0460410980512618)
(20, 0.44423754983436314)
(21, 0.8072331009499932)
(22, -0.027947700872862247)
(23, -0.034770430711267904)
(24, 0.39756281239580293)
(25, 0.3699428442896803)
(26, -0.03633799240395952)
(27, 0.09626008515657695)
(28, 0.014682124391237991)
(29, -0.1950864807574515)
(30, 0.4214602491711964)
(31, 0.32752191267914443)
(32, 0.8147665544161273)
(33, 1.1943928365579848)
(34, 0.8442749374688707)
(35, 0.8539460190246957)
(36, 0.8378929322214365)
(37, 0.605826515524137)
(38, 0.3754834610139078)
(39, 0.19618989447977211)
(40, 0.21985827202290145)
(41, 0.12281178477141666)
(42, 0.09933751426029094)
(43, 0.09874534777561945)
(44, 0.10077937212750858)
(45, 0.10183583181427532)
(46, 0.09446748780546557)
(47, 0.09397140128386498)
(48, 0.08311261717521025)
(49, 0.08379114997515624)
(50, 0.08379114997515624)
}

\renewcommand{\drawPixelTen}{%
(1, 0.29013297407719707)
(2, 1.0267252059819585)
(3, 0.9135120420520122)
(4, -0.23872606789690431)
(5, 0.5712132340939888)
(6, 0.4953390416384232)
(7, 0.14105949253290606)
(8, 0.5830353980652331)
(9, 0.4290857780309263)
(10, 0.4492162784448587)
(11, 1.0704484586972005)
(12, 0.429619630024506)
(13, 0.5483495187105596)
(14, 0.272545061347172)
(15, 0.8190856491690559)
(16, 1.2979153338874738)
(17, 1.421629407626438)
(18, 1.536718512238612)
(19, 1.906481953340041)
(20, 2.523546990501069)
(21, 1.7585524092328852)
(22, 1.4404536377385173)
(23, 1.9548764248878627)
(24, 2.3686399482267664)
(25, 2.5590027427812734)
(26, 1.6255486730701307)
(27, 0.7533994154058699)
(28, 1.108780685309262)
(29, 0.7927350652235994)
(30, 0.1420172153817424)
(31, 0.7250083658733669)
(32, 1.0364757137125105)
(33, 0.8918131216278439)
(34, 0.6679904993990841)
(35, 0.21315234059400312)
(36, 0.2594867757382215)
(37, 0.31871244543485244)
(38, 0.3651742280452326)
(39, 0.43309672417408646)
(40, 0.42305973622460996)
(41, 0.40991981301240255)
(42, 0.40105771851070593)
(43, 0.3616586336338008)
(44, 0.3430648371762945)
(45, 0.3449028796303824)
(46, 0.3590437914880254)
(47, 0.35449157232907597)
(48, 0.35473419676551177)
(49, 0.3558629256423308)
(50, 0.3558629256423308)
}

==> data/drawPixel3.tex <==
\newcommand{\drawPixelOne}{%
(1, -49.57467428538022)
(2, -45.29835818380813)
(3, -34.696410066403544)
(4, -49.72664671856651)
(5, -56.10609520847051)
(6, -30.24772995000192)
(7, -44.97539264197901)
(8, -27.309380133624845)
(9, -18.603530659256393)
(10, 0.01954590663227762)
(11, -0.0030095800264791847)
(12, 16.19076915477668)
(13, 14.087361252866408)
(14, -0.17093478198499312)
(15, 1.1157041136466068)
(16, -4.771448479137353)
(17, -2.350080382832805)
(18, 5.9839237269072685)
(19, 7.391888805333171)
(20, 4.820087813356897)
(21, 2.6678076301109375)
(22, -0.009656871406624079)
(23, 0.43476473051588516)
(24, -0.04535752710842758)
(25, 0.3391880171400127)
(26, -0.4326072057441162)
(27, 0.4495944916339093)
(28, -0.00846003503899398)
(29, -0.5941836385854824)
(30, -1.2587671417454902)
(31, -1.3283426701848466)
(32, -1.2627454003345278)
(33, -1.035961485762104)
(34, -0.8481885493888868)
(35, -1.000871017319579)
(36, -1.0213494266556427)
(37, -1.0293371073649558)
(38, -0.8565268277609435)
(39, -0.7364145587221279)
(40, -0.7993172789618882)
(41, -0.8016227625424499)
(42, -0.7936238381921267)
(43, -0.7825947789662104)
(44, -0.760098172175774)
(45, -0.7681845072115794)
(46, -0.7669665935701662)
(47, -0.759735552339102)
(48, -0.7574188345802612)
(49, -0.7552836981496804)
(50, -0.7552836981496804)
}


\newcommand{\drawPixelTwo}{%
(1, 17.156573156561123)
(2, -60.591305116897374)
(3, -51.07725483145515)
(4, -16.592283736411023)
(5, -11.126113557264828)
(6, 33.167707748737534)
(7, 2.83569482362223)
(8, 7.398412029538431)
(9, -10.504927882573224)
(10, -0.5160096985718043)
(11, 8.097653384317935)
(12, 21.025888514886493)
(13, 32.48804827567395)
(14, 28.411924924719564)
(15, 26.588466479465055)
(16, 16.998166937132133)
(17, 2.822040280159717)
(18, 2.9515880637680496)
(19, 2.101246484989369)
(20, -2.465569761390885)
(21, -1.338830736793902)
(22, -2.2488519516892524)
(23, -0.07542554709825056)
(24, 0.26880585344302976)
(25, 1.1745737975545176)
(26, 0.9618045357669025)
(27, 0.9252977077127976)
(28, 1.2933446781780424)
(29, 0.22769501400821635)
(30, 0.7128382792797898)
(31, 0.9443255301003624)
(32, 0.7790157352444939)
(33, 0.25208347184341073)
(34, 0.2510644141909909)
(35, 0.38615055038246265)
(36, 0.5661705097309229)
(37, 0.5357154828723576)
(38, 0.5027647895642007)
(39, 0.5385779216410201)
(40, 0.5566085692029015)
(41, 0.5376771752858222)
(42, 0.5506007021291134)
(43, 0.5352441181698379)
(44, 0.5283157731793415)
(45, 0.5170706973996598)
(46, 0.5075684927333908)
(47, 0.5043619545761402)
(48, 0.501328841289778)
(49, 0.5023214683347719)
(50, 0.5023214683347719)
}


\newcommand{\drawPixelThree}{%
(1, 135.21940462544134)
(2, 104.71982637325695)
(3, 96.91021542820536)
(4, 84.84230333493048)
(5, 122.61515707042334)
(6, 77.3882280887993)
(7, 96.83252303117074)
(8, 53.76644949009422)
(9, 21.56225853904853)
(10, 32.75327600276974)
(11, 24.886429366410074)
(12, 22.95853823142371)
(13, 15.933369162147352)
(14, -3.0841101902662533)
(15, -1.3692599995832353)
(16, 1.2378681250417602)
(17, -2.25354037262219)
(18, -6.929085943941185)
(19, -1.3669272442245841)
(20, -0.5491915314910284)
(21, -2.6261687705602936)
(22, -3.4022732100082385)
(23, -3.0644691150388246)
(24, -4.025168739707263)
(25, -2.0157854089736813)
(26, -0.4793669924298365)
(27, -1.1388878275259127)
(28, -0.8426490701386635)
(29, -1.323118127619117)
(30, -1.001257825713176)
(31, -0.8027349081424417)
(32, -0.4105174377355541)
(33, -0.787461622343608)
(34, -0.6145753239735997)
(35, -0.20255633861588007)
(36, -0.26280182631917154)
(37, -0.17869609147871873)
(38, -0.17667546810977436)
(39, -0.21394967695924202)
(40, -0.3136190050018197)
(41, -0.3274062200580071)
(42, -0.3745391957797204)
(43, -0.36719640553034877)
(44, -0.35511063908632623)
(45, -0.35104923751951267)
(46, -0.3437487342392504)
(47, -0.33491211309260543)
(48, -0.32946377850778863)
(49, -0.32919012720754043)
(50, -0.32919012720754043)
}


\newcommand{\drawPixelFour}{%
(1, 66.25921559693269)
(2, 83.88587853330435)
(3, 68.69357173380277)
(4, 60.57384139817216)
(5, 41.866811780127264)
(6, 45.692825534000065)
(7, 30.42410196784493)
(8, 16.747270772996856)
(9, 38.463085729650935)
(10, 12.983449277261759)
(11, 14.605526239563648)
(12, 7.961218548198822)
(13, -4.261803844863201)
(14, 7.008158397364716)
(15, -5.966904123014891)
(16, -7.563923377296286)
(17, -12.261324690176142)
(18, -12.987432252737598)
(19, -6.607817208285392)
(20, -4.978948210334542)
(21, -2.752999940219412)
(22, -0.743826669395536)
(23, -1.6337290073635744)
(24, -1.5125989400273234)
(25, -0.6406111347164604)
(26, -2.010735750169441)
(27, -1.6280182276554422)
(28, -1.3973822958649127)
(29, 0.5451144868821055)
(30, 1.5276872694549617)
(31, 1.08718425367633)
(32, 1.2408153139588667)
(33, 1.2578344099173961)
(34, 0.9102731303522233)
(35, 0.6772704689838809)
(36, 0.5424882242070617)
(37, 0.44938936586291545)
(38, 0.20305003588385104)
(39, 0.1470083583384901)
(40, 0.16269334128750315)
(41, 0.2155191175949483)
(42, 0.24251673870106577)
(43, 0.22992361519696033)
(44, 0.22686881651813195)
(45, 0.21945696487875124)
(46, 0.21764304566476206)
(47, 0.2296827443259734)
(48, 0.2291572989044548)
(49, 0.22966671401897062)
(50, 0.22966671401897062)
}


\newcommand{\drawPixelFive}{%
(1, -105.98648899353329)
(2, -81.21434947732651)
(3, -71.35365685254915)
(4, -50.61838299700669)
(5, -17.092804078683987)
(6, 7.001770208305119)
(7, 22.30058058308328)
(8, 9.102995426825983)
(9, 4.64945980340287)
(10, 6.725858784052024)
(11, -3.0705664840949156)
(12, 1.2158534010553317)
(13, 11.150820329463322)
(14, 3.0912102089221865)
(15, 7.3352064898557625)
(16, 1.4303335941834732)
(17, -1.1960944527095991)
(18, 3.9070075971806375)
(19, 2.9417001869714605)
(20, 0.6503926181057285)
(21, -2.542076621381147)
(22, -2.300173172589681)
(23, -4.655578163518569)
(24, -2.1777040461934085)
(25, -2.6114162173422413)
(26, -2.39940360321966)
(27, -1.165707018161967)
(28, -0.34852283112626037)
(29, -0.396758337462389)
(30, -1.5422630438963467)
(31, -0.9207236433300658)
(32, -0.45568058573222686)
(33, 0.1077096339167476)
(34, -0.16676012706532925)
(35, -0.07302647614053198)
(36, -0.04212366984357868)
(37, -0.2515935610990305)
(38, -0.34491203955945565)
(39, -0.29579925803426566)
(40, -0.3681473843703629)
(41, -0.43060260970331665)
(42, -0.3967961897951155)
(43, -0.3947375983221984)
(44, -0.4033853858321873)
(45, -0.41389017727325295)
(46, -0.42701399276119606)
(47, -0.4334989897168367)
(48, -0.42986378772640704)
(49, -0.4290710074240919)
(50, -0.4290710074240919)
}


\newcommand{\drawPixelSix}{%
(1, 68.10323219044224)
(2, 109.45541625570652)
(3, 100.98889356284585)
(4, 68.90219210755461)
(5, 47.351337567801295)
(6, 36.96821319248387)
(7, 31.388064871609124)
(8, 26.620266411062666)
(9, 12.142815517516631)
(10, 10.786644361974131)
(11, 3.5871399400055415)
(12, 2.342745099209349)
(13, -1.592955244340418)
(14, -12.49882013789734)
(15, -11.68246328299642)
(16, -0.24975300963999914)
(17, -1.7941284989549746)
(18, 3.8145423449610467)
(19, 6.614027424114456)
(20, 7.584391150020178)
(21, 5.587566969154693)
(22, 6.662555728185037)
(23, 5.88100731306479)
(24, 4.864278921988698)
(25, 4.461864161236712)
(26, 4.2573303027559914)
(27, 1.8800404020039132)
(28, 0.7423225286753643)
(29, 0.6393419140884795)
(30, 1.075709038911324)
(31, 1.320510716261184)
(32, 0.9361905622941071)
(33, 1.3550921406518794)
(34, 1.3695017391437962)
(35, 0.9750918610476593)
(36, 1.0357742267313563)
(37, 1.0982742723169927)
(38, 1.0826074266246042)
(39, 1.0381015853144604)
(40, 1.0019100088926711)
(41, 0.992975037033244)
(42, 1.021284894474953)
(43, 1.0134328072011185)
(44, 1.0187845818213364)
(45, 1.0052239737042017)
(46, 1.0004320178235462)
(47, 0.9957594472842408)
(48, 0.9975248393138029)
(49, 0.9960653771154964)
(50, 0.9960653771154964)
}


\newcommand{\drawPixelSeven}{%
(1, 44.324141753463095)
(2, 11.164097719078754)
(3, 7.2909422362339615)
(4, 26.174166861500126)
(5, 11.773078870338832)
(6, 39.72051953749909)
(7, 34.94108355542807)
(8, 38.27641709490342)
(9, 34.95216539573215)
(10, 25.36426546880132)
(11, 13.842261212339375)
(12, 16.64258642389009)
(13, 19.795228721155745)
(14, 19.22336193361641)
(15, 17.265645154295576)
(16, 19.322644063593554)
(17, 8.409511362269106)
(18, 16.031115877315372)
(19, 9.738644749568426)
(20, 4.953579024560135)
(21, 3.804089952909626)
(22, 5.7164975322526494)
(23, 1.9350081430772876)
(24, 3.129459357125134)
(25, 5.656486526653595)
(26, 2.978786490101195)
(27, 2.5339736901088696)
(28, 1.560152744874146)
(29, 1.2701106619047673)
(30, 1.4037825691465802)
(31, 0.7379596014098181)
(32, 0.5077855119773897)
(33, 0.7020215171662205)
(34, 0.7405684721150727)
(35, 0.7455595758669975)
(36, 0.7487432647732448)
(37, 0.9138832428650572)
(38, 1.0010750943546896)
(39, 0.9815094404759808)
(40, 1.0512148299171888)
(41, 1.0815024320586908)
(42, 1.0168774281437416)
(43, 0.9995760606936294)
(44, 1.0166836226632316)
(45, 1.0098931561354376)
(46, 1.0047140048020196)
(47, 1.0092029888107246)
(48, 0.9970404777592192)
(49, 0.9976266935747691)
(50, 0.9976266935747691)
}


\newcommand{\drawPixelEight}{%
(1, 30.9506336447757)
(2, 16.13317459623454)
(3, 16.83468523425193)
(4, 10.225415056926245)
(5, 35.383092847972804)
(6, 41.47779224725952)
(7, 40.243400837956)
(8, 25.299844646482526)
(9, 20.400359567559413)
(10, 25.316424962372242)
(11, 25.878560871733022)
(12, 15.608542119633693)
(13, 11.466600127457994)
(14, 0.4423760294766854)
(15, -0.954308166225169)
(16, -8.370758891252018)
(17, -6.433185442439714)
(18, -3.030558422770849)
(19, -0.14096122741065065)
(20, -5.221626803345235)
(21, -1.7618069499850066)
(22, -0.22761101472969014)
(23, 0.03380633816895812)
(24, -1.5286924182755084)
(25, -0.012229358524390443)
(26, -0.3874274459778928)
(27, -1.6749026273999787)
(28, -1.6208977958555173)
(29, -2.223099985442546)
(30, -1.5875236588712418)
(31, -0.9792958337418065)
(32, -0.39731371295492257)
(33, -0.3577170380222044)
(34, 0.07940173850506066)
(35, -0.14687263995620484)
(36, -0.22050600426474037)
(37, -0.2361888923886814)
(38, -0.23295370749905098)
(39, -0.14027790881667748)
(40, -0.22284863969294613)
(41, -0.20154875580750217)
(42, -0.20159590411088157)
(43, -0.2155507218627131)
(44, -0.18627548091424692)
(45, -0.19631428314715546)
(46, -0.2028762635195291)
(47, -0.20640488992567804)
(48, -0.20855421390834006)
(49, -0.2113924504510372)
(50, -0.2113924504510372)
}


\newcommand{\drawPixelNine}{%
(1, -71.60923312530174)
(2, -76.08122535677717)
(3, -57.20891706736312)
(4, 7.439683618363617)
(5, 40.014268109825736)
(6, 20.553394049326453)
(7, 32.53036467190776)
(8, 49.06374035978297)
(9, 34.612791285952206)
(10, 30.08204526756567)
(11, 0.46823981025426065)
(12, 9.1500421380479)
(13, 3.0445229269616707)
(14, 7.985354766962915)
(15, 1.5577671740798715)
(16, -3.104323664998554)
(17, 5.53312801179833)
(18, 0.7149088300741759)
(19, 4.3610151848337395)
(20, 3.9829091318803904)
(21, 1.3938554130222616)
(22, -1.182471458320797)
(23, -2.146644890141321)
(24, -1.4131949587350823)
(25, -1.1016373289548527)
(26, -1.003230715867494)
(27, -0.5089897169252513)
(28, -1.6140936259808003)
(29, -0.8213676022802526)
(30, -0.17163400704533804)
(31, -0.4700907225394033)
(32, -0.44715185231191845)
(33, -0.45409371729750464)
(34, -0.46702486175547825)
(35, -0.38883948754083625)
(36, -0.5019523097712557)
(37, -0.3744868401132686)
(38, -0.31342157818778305)
(39, -0.42515781475810577)
(40, -0.4015811779608046)
(41, -0.44457556710250146)
(42, -0.42018598786013794)
(43, -0.4177482901537749)
(44, -0.4271427234643343)
(45, -0.41897648221575245)
(46, -0.4181793688472491)
(47, -0.4137630061954828)
(48, -0.41497221036560156)
(49, -0.4169541432611085)
(50, -0.4169541432611085)
}


\newcommand{\drawPixelTen}{%
(1, -30.440225195686633)
(2, 24.611264218341855)
(3, -29.14718591138659)
(4, -17.076380533078442)
(5, 9.087734312458455)
(6, 22.273443397155155)
(7, 10.186942143457571)
(8, -4.929340531133631)
(9, -4.525590512734002)
(10, -18.22694753525175)
(11, -12.518177779338584)
(12, -26.160200365817218)
(13, -17.197262829538065)
(14, -14.4747298284571)
(15, -18.086037397088003)
(16, -19.01978038597305)
(17, -2.319015407656968)
(18, -4.75037881377186)
(19, -2.2000490286688485)
(20, -3.3214803163305233)
(21, -3.019423935062027)
(22, -4.026003943829254)
(23, -5.8428368765375795)
(24, -5.058357280339562)
(25, -3.6493117404462976)
(26, -3.0247375795672293)
(27, -2.352258538798522)
(28, -1.503206286191136)
(29, -0.6246111304569762)
(30, -0.3273226444767372)
(31, 0.3191422952898181)
(32, -0.07514293258303528)
(33, 0.3962876613984969)
(34, 0.8208819476467508)
(35, 0.9989260710779913)
(36, 0.8770255602339331)
(37, 0.8319537273285423)
(38, 0.8230642725639642)
(39, 0.9063339674571408)
(40, 0.8555445857034425)
(41, 0.9959947672136623)
(42, 0.9863808900969473)
(43, 0.9550235167468407)
(44, 0.9874067676805044)
(45, 0.9977695599648128)
(46, 0.9949659392008292)
(47, 0.9866857138442899)
(48, 0.9818031427278667)
(49, 0.9839265129494074)
(50, 0.9839265129494074)
}

==> data/drawPixel3_cifar.tex <==
\renewcommand{\drawPixelOne}{%
(1, 8.563700567039149)
(2, 69.1155387893669)
(3, 54.28961027503663)
(4, 35.19482877611635)
(5, 7.196767279672194)
(6, -5.777663416773188)
(7, 7.636196118029578)
(8, 17.192038751084688)
(9, 25.51482714613892)
(10, 9.941324382900714)
(11, -5.2592665431317185)
(12, 1.1545117925143558)
(13, -6.584010619464791)
(14, 1.0487084150843033)
(15, -0.3460655466196668)
(16, -6.668013949406452)
(17, -3.799641947918592)
(18, -1.3366433440580814)
(19, -2.65334031805678)
(20, 1.094546593332632)
(21, 5.349231209687304)
(22, 0.8843858097198805)
(23, -1.1776284190647004)
(24, -1.246959835059997)
(25, 1.715540287551081)
(26, 1.1416141631606598)
(27, 0.8953581479638262)
(28, 0.3157050674808403)
(29, -1.0869038810055804)
(30, 0.1886161689646373)
(31, -0.34956334601682837)
(32, -0.4014765324768714)
(33, -0.5035572411181207)
(34, -0.2570185878102942)
(35, -0.5037097228539235)
(36, -0.41744814217103704)
(37, -0.3756387395185822)
(38, -0.19305103832646453)
(39, -0.19805947832230603)
(40, -0.2700961640851322)
(41, -0.3301368924593826)
(42, -0.3554489026542149)
(43, -0.3633936393770101)
(44, -0.38776683649072685)
(45, -0.3973462640819832)
(46, -0.4026611252598839)
(47, -0.3989746890874101)
(48, -0.4024955714123016)
(49, -0.4035632710314496)
(50, -0.4035632710314496)
}

\renewcommand{\drawPixelTwo}{%
(1, -0.2707725792596207)
(2, 32.995908840033614)
(3, 14.569703188184247)
(4, 23.133334307898505)
(5, 52.311543493640926)
(6, 22.02137888973899)
(7, 51.23625518224728)
(8, 29.162234506581918)
(9, -5.149030683066837)
(10, 5.600280528318537)
(11, 2.3877500218038596)
(12, 14.765345358371773)
(13, 9.03759337337533)
(14, 5.862355845956826)
(15, 2.796658546142941)
(16, 6.429986184789499)
(17, 3.828739231211632)
(18, 7.015758744967304)
(19, 5.113107712851956)
(20, 2.6002292664096203)
(21, 4.573121035867127)
(22, 3.1543755107597455)
(23, 2.7446654465324944)
(24, 2.5278167603083705)
(25, 3.241489926879768)
(26, -0.557273502333854)
(27, -1.3253277821292349)
(28, 0.30993371429542227)
(29, -0.3566893888757172)
(30, 0.14938141422241596)
(31, -0.33071015866003034)
(32, 0.08015375400759689)
(33, 0.12104990023982108)
(34, -0.07844327634670914)
(35, 0.006836090633286633)
(36, 0.00870677716367451)
(37, 0.014525709904286213)
(38, 0.18788850345669195)
(39, 0.187795642257616)
(40, 0.21844211422411636)
(41, 0.20646338185427277)
(42, 0.1759046007658229)
(43, 0.1445706506009489)
(44, 0.15254717256104844)
(45, 0.18034305962010244)
(46, 0.1845729242511984)
(47, 0.18852619575662735)
(48, 0.1878276291949193)
(49, 0.19134954353008898)
(50, 0.19134954353008898)
}

\renewcommand{\drawPixelThree}{%
(1, -20.51112875035772)
(2, -42.6570350752596)
(3, -46.13731118910505)
(4, -6.739790577436459)
(5, -1.03965704729106)
(6, 30.93290833905194)
(7, 10.750423445854576)
(8, 21.314729170185263)
(9, 26.181359723954095)
(10, 18.976422838030302)
(11, 1.5174312896175586)
(12, -14.662582499960187)
(13, -22.79723101216042)
(14, -9.536967997303918)
(15, -8.35147659975102)
(16, -9.871428660191862)
(17, -3.351266690669296)
(18, -5.0392522054701745)
(19, -4.954332883010264)
(20, -3.022803686208663)
(21, -1.5359760944578162)
(22, 0.5124957377188255)
(23, -0.6503374122458451)
(24, -1.6363292974419659)
(25, -0.06481199047256436)
(26, 0.6182144772812355)
(27, -1.925547456495732)
(28, -2.3408651868454418)
(29, -1.719914156818616)
(30, -1.8482246193174894)
(31, -0.9249090314048956)
(32, -0.88311753085368)
(33, -0.9717115122520388)
(34, -0.7398554214448523)
(35, -0.8624023563093746)
(36, -0.47835036985937146)
(37, -0.4703790226545655)
(38, -0.4373307490996268)
(39, -0.45931716667421246)
(40, -0.4723806919455315)
(41, -0.41038291335764904)
(42, -0.4415130509984229)
(43, -0.44082421110155534)
(44, -0.43829130155723117)
(45, -0.4115868986488112)
(46, -0.40682046671866645)
(47, -0.3969895601538856)
(48, -0.39346900202661583)
(49, -0.3944629713064807)
(50, -0.3944629713064807)
}

\renewcommand{\drawPixelFour}{%
(1, -51.40822903694278)
(2, -72.0725068375487)
(3, -23.39057811292374)
(4, -61.92716579022966)
(5, -26.49209358725742)
(6, -19.18566112884757)
(7, -7.279098201452463)
(8, -2.035702423512272)
(9, 6.587503142578039)
(10, 7.709161739415595)
(11, -2.9893587731793385)
(12, 4.325305373652055)
(13, -7.379255872879488)
(14, -4.5906488641360195)
(15, -6.984020013406774)
(16, -12.486553528799012)
(17, -6.79769928887356)
(18, -12.832099880954267)
(19, -6.424464350621836)
(20, -6.105102965654342)
(21, -4.8192804590799785)
(22, -5.127542573773818)
(23, -2.8281010631773826)
(24, 0.6719606939396217)
(25, 0.10338782119534778)
(26, -1.5287116348129512)
(27, -2.318297363490732)
(28, -0.9261360798758362)
(29, -1.0130446942599414)
(30, -1.8952103498565274)
(31, -2.2815507411547675)
(32, -1.5768444064446505)
(33, -1.0606050504119906)
(34, -0.8252390229038225)
(35, -0.592003721504432)
(36, -0.3806002954126335)
(37, -0.446299070071147)
(38, -0.3187667075375271)
(39, -0.39673843960877825)
(40, -0.37309634081879317)
(41, -0.42194747434576263)
(42, -0.4368223942105748)
(43, -0.4527834183964392)
(44, -0.4325752775436977)
(45, -0.43914049073569933)
(46, -0.4345723809566142)
(47, -0.430065108448323)
(48, -0.4336754784422015)
(49, -0.43000121949982023)
(50, -0.43000121949982023)
}

\renewcommand{\drawPixelFive}{%
(1, -8.751935607612005)
(2, 18.237752499808078)
(3, 18.661945455272487)
(4, 8.199123665498782)
(5, -4.308295938693551)
(6, -24.81289435174397)
(7, -27.968579683143922)
(8, 4.0142509102423425)
(9, 16.521816029038703)
(10, 31.93249016057578)
(11, 31.66372522676799)
(12, 17.787330059182054)
(13, 6.814339472348965)
(14, 11.318855839574399)
(15, 2.483057102094893)
(16, 9.530937905996907)
(17, 8.877472366844641)
(18, 10.172320126572137)
(19, 15.29720550920899)
(20, 8.003493495214745)
(21, 3.062571341948267)
(22, 2.3200518641796126)
(23, 3.0484256426335676)
(24, -1.7305146701176186)
(25, -2.956468372639611)
(26, -3.5764542124213294)
(27, -3.2691846509854656)
(28, -1.9810452936838787)
(29, -1.127609578162141)
(30, -1.4596979224831346)
(31, -0.8360488716024213)
(32, -0.8776908898615084)
(33, -0.8229510738881719)
(34, -0.7173705918721597)
(35, -0.74209341726584)
(36, -0.6594662306480074)
(37, -0.48193096956493875)
(38, -0.5205054572412088)
(39, -0.4922601855567812)
(40, -0.38108421878366056)
(41, -0.27197717796936105)
(42, -0.2962374131587937)
(43, -0.32074717561664773)
(44, -0.3267944105091852)
(45, -0.29411899557787125)
(46, -0.2773242443258062)
(47, -0.28206887146240295)
(48, -0.28112585158625375)
(49, -0.2820215979207857)
(50, -0.2820215979207857)
}

\renewcommand{\drawPixelSix}{%
(1, -17.8157631859508)
(2, -11.008678019564572)
(3, 6.680058332901426)
(4, 45.364126175446216)
(5, 21.280812640259235)
(6, -4.21145827763366)
(7, 25.972901428985267)
(8, 24.67226155866245)
(9, 30.958192329922678)
(10, 22.48061749599247)
(11, 22.707462044940478)
(12, 20.82358881044105)
(13, 32.260452317708896)
(14, 22.694401549955096)
(15, 15.098305760418006)
(16, 10.561708699742328)
(17, 5.814299113171531)
(18, 9.194374501320624)
(19, 8.139119841958692)
(20, 7.086363107327263)
(21, 3.9960633101931413)
(22, 1.3913228586908315)
(23, 2.7407617712391668)
(24, 4.563797358668587)
(25, 4.285495251109072)
(26, 2.2461936799378686)
(27, 0.6207178115614744)
(28, 0.667122039907817)
(29, -0.13165432231353558)
(30, 0.0012700987703588885)
(31, 0.29970554374207814)
(32, 0.5022654889136029)
(33, 0.10873900511710935)
(34, -0.45816724358383537)
(35, -0.2003985204349044)
(36, 0.001886130551649684)
(37, 0.03238203754985771)
(38, -0.012001022924175625)
(39, 0.09924123555702112)
(40, 0.08961886550608551)
(41, 0.12368968715302553)
(42, 0.1378210458672754)
(43, 0.128638024816861)
(44, 0.1291781582512304)
(45, 0.11942921858350145)
(46, 0.12177578341673738)
(47, 0.11497008737160944)
(48, 0.11916171240557467)
(49, 0.11933319838320043)
(50, 0.11933319838320043)
}

\renewcommand{\drawPixelSeven}{%
(1, 41.89354911440237)
(2, 27.882755508049346)
(3, -17.236309451959848)
(4, 29.2138144176748)
(5, 33.03530258269159)
(6, 26.61462522554941)
(7, 34.28149772321811)
(8, 31.46488271304134)
(9, 24.51019042033546)
(10, 20.19674830258972)
(11, 8.957342431078883)
(12, 13.33199065129054)
(13, 4.931290314098935)
(14, 7.0366156046843)
(15, -5.497990710885767)
(16, -8.090916854671278)
(17, 0.572502376034655)
(18, -0.7920904815518492)
(19, 2.440944440542716)
(20, 5.579711416456445)
(21, 2.8231446945769383)
(22, 2.5634982035962355)
(23, 2.515917656870293)
(24, 0.7402259980398349)
(25, 1.5850257153362743)
(26, 0.00719630325530507)
(27, -0.2669987482758547)
(28, 0.7268765508188963)
(29, 0.6602551650206288)
(30, 0.4788601182445257)
(31, 0.8672581859276591)
(32, 1.126838249463232)
(33, 0.5121767676310653)
(34, 0.3224371897424981)
(35, 0.31932213072248106)
(36, 0.20843261803523855)
(37, 0.11352310383793317)
(38, 0.12257995579845904)
(39, 0.21383729855266698)
(40, 0.17483393220300664)
(41, 0.27630933843329175)
(42, 0.2610416828362415)
(43, 0.2492357868099086)
(44, 0.2140082588449867)
(45, 0.2257918806838875)
(46, 0.23386895679334424)
(47, 0.2276637125570293)
(48, 0.23037620972636053)
(49, 0.2310226745689458)
(50, 0.2310226745689458)
}

\renewcommand{\drawPixelEight}{%
(1, -65.45133273257937)
(2, -76.63029932426039)
(3, -30.677665021964316)
(4, -52.425714467779784)
(5, -33.9487066911866)
(6, -44.35046326316417)
(7, -21.670865240394214)
(8, -5.779877162690521)
(9, 6.303618156324119)
(10, -9.454863778938915)
(11, -1.8464624363498503)
(12, 7.044399410401671)
(13, 0.7009294975575271)
(14, 2.349946940487159)
(15, 2.7953244014107184)
(16, 0.36629907887603186)
(17, -0.046655731374092846)
(18, -2.8978595625589723)
(19, 0.3913977972888718)
(20, 0.9726319270799078)
(21, 2.513791779795856)
(22, -0.6144057376636738)
(23, 1.7052145075510325)
(24, 2.0563790397128074)
(25, 1.8674573707334088)
(26, 0.7376905643918781)
(27, 1.0283945675451935)
(28, 0.7200558886686016)
(29, 0.36420876599943713)
(30, 1.297028380520683)
(31, 1.2688490556819148)
(32, 0.6877150848845748)
(33, 0.6373722626997286)
(34, 0.49597533881163025)
(35, 0.3821461951132902)
(36, 0.49149909421407645)
(37, 0.4371222428336804)
(38, 0.39323362677025064)
(39, 0.4812080482834498)
(40, 0.4872143164870799)
(41, 0.49180017451714)
(42, 0.49137029904945184)
(43, 0.514480790912756)
(44, 0.5103040815846316)
(45, 0.5323684251102759)
(46, 0.529417700964864)
(47, 0.5292318153277711)
(48, 0.5318003576965457)
(49, 0.5310567460043115)
(50, 0.5310567460043115)
}

\renewcommand{\drawPixelNine}{%
(1, 87.68201827908818)
(2, 97.98963271287394)
(3, 39.701099911869846)
(4, 8.529614162105208)
(5, 15.91888967914318)
(6, 31.62174922281354)
(7, 18.56154363606249)
(8, 17.08476548343832)
(9, 25.552352091587977)
(10, 21.476414777789955)
(11, 11.081851872360211)
(12, 16.26755041975361)
(13, 4.764291973729396)
(14, 12.25619808402435)
(15, 4.701258029256599)
(16, 9.929177225896854)
(17, 11.012952181609311)
(18, 10.18613552868908)
(19, 7.217873176644817)
(20, 2.6270187325390713)
(21, 3.8690276130295937)
(22, -0.11211262979165992)
(23, -0.11269193813813104)
(24, 1.2454044456584628)
(25, 1.0029775691969633)
(26, -0.07237476254044173)
(27, 0.15727974287706076)
(28, 0.08003577008133775)
(29, -0.2205049975820622)
(30, 0.5770458214726301)
(31, 0.4529746601208951)
(32, 1.0111586605030705)
(33, 1.4029487097495856)
(34, 1.0335541563705846)
(35, 1.054328417580559)
(36, 1.0372387172071658)
(37, 0.8197523610634695)
(38, 0.6128213580051147)
(39, 0.43123884811676383)
(40, 0.44947595223082926)
(41, 0.37213465757297115)
(42, 0.34629162153752036)
(43, 0.3515605234216187)
(44, 0.3553633329398766)
(45, 0.35606504399352473)
(46, 0.3479434740628571)
(47, 0.3466727959092301)
(48, 0.337349364713518)
(49, 0.33792067673835846)
(50, 0.33792067673835846)
}

\renewcommand{\drawPixelTen}{%
(1, 20.54849472871166)
(2, 65.45500808342919)
(3, 50.31134315587076)
(4, -12.969267843333746)
(5, 24.096726523556477)
(6, 19.49671064580609)
(7, 4.974365422819462)
(8, 18.88829619466101)
(9, 11.591878722396256)
(10, 10.647337661013735)
(11, 22.103086753223025)
(12, 7.777619411227965)
(13, 8.620351804389909)
(14, 3.528954147239096)
(15, 9.552249409540316)
(16, 13.20920167735824)
(17, 12.424164955959991)
(18, 11.388863429373473)
(19, 11.969253834947345)
(20, 13.488188840498633)
(21, 7.889258260119334)
(22, 5.409548389379552)
(23, 6.269460662157293)
(24, 6.507215278395771)
(25, 6.095430943626557)
(26, 3.3441995830384794)
(27, 1.2728147689000657)
(28, 1.7009880404613371)
(29, 1.057963758877271)
(30, 0.11079578447016292)
(31, 0.7721956402908724)
(32, 1.0610085735713755)
(33, 0.8352706066205849)
(34, 0.5621965061388378)
(35, 0.1293632550668533)
(36, 0.19962699096668632)
(37, 0.23375698272147186)
(38, 0.2801468636527022)
(39, 0.3585916613075888)
(40, 0.3499635534902669)
(41, 0.32683745207208786)
(42, 0.31071444599568276)
(43, 0.26828198818078797)
(44, 0.24864231271440437)
(45, 0.24654975804190069)
(46, 0.2589644479538795)
(47, 0.25164877178462064)
(48, 0.24981912999123704)
(49, 0.2514189473232255)
(50, 0.2514189473232255)
}

==> data/drawPixel4.tex <==
\newcommand{\drawPixelOne}{%
(1, -0.7876386893794)
(2, -0.09373105246985995)
(3, -0.1034588546691015)
(4, 0.7033599046353282)
(5, 0.5935271382585608)
(6, -0.5045601961860766)
(7, 0.24806298950551353)
(8, 0.8625354018321671)
(9, 1.3654690987943474)
(10, 2.3748167869433754)
(11, 2.1199831691882713)
(12, 0.9906786852768195)
(13, 2.121687175929907)
(14, 2.0616069887429758)
(15, 2.24022087079602)
(16, 2.330717677220349)
(17, 1.8279028704415388)
(18, 0.776764393742524)
(19, -0.2947722349421408)
(20, -0.1361478978015151)
(21, -0.2742664848788518)
(22, 0.272898215765765)
(23, 0.9188533955971137)
(24, -0.6336143697675748)
(25, -0.08963245934364408)
(26, -0.1409988323554789)
(27, -1.1713952419840767)
(28, -0.659458671015011)
(29, -0.8368529477186617)
(30, 0.29235862283055375)
(31, 0.40233023550294195)
(32, 0.024664075876559416)
(33, 0.7390168018466656)
(34, 0.2209995218378898)
(35, -0.4116789082911131)
(36, 0.24974695103100436)
(37, -0.09481844299435435)
(38, 0.044582677419316485)
(39, -0.8430965889755955)
(40, -1.0466975702116696)
(41, -1.830950850305883)
(42, -1.2511086095816182)
(43, -0.9446127615256181)
(44, -1.2227548263671546)
(45, -0.7190899193933045)
(46, -0.7987663170130784)
(47, -0.7695137107014914)
(48, -0.43401845212157397)
(49, -0.38590446753555147)
(50, -0.3881051672234428)
}


\newcommand{\drawPixelTwo}{%
(1, 0.7032692184696532)
(2, 1.9064201580543871)
(3, 0.9390498753886369)
(4, 1.109172742219211)
(5, 0.23145749941846525)
(6, 0.7282426670616662)
(7, -0.6357947389376138)
(8, -0.7259413240850845)
(9, -0.7650217053348576)
(10, -0.5344909275501913)
(11, -0.7112186680124516)
(12, -0.8920580476352306)
(13, -0.7397176941996572)
(14, -1.4460183520114742)
(15, -0.6905697821053237)
(16, -0.9320225855451638)
(17, -1.7010945607494166)
(18, -1.5918797483991776)
(19, -1.0126357880466212)
(20, -0.9113953080928439)
(21, -1.74063505191511)
(22, -1.637838765144418)
(23, 0.24611305285041182)
(24, 0.1989945957299918)
(25, -0.2764554018756681)
(26, 0.45152924612830775)
(27, 0.26883056999964483)
(28, 1.8620857144843845)
(29, -0.21174961862606734)
(30, -0.8554008597407392)
(31, -0.5219901578516623)
(32, 0.36968470279142274)
(33, 0.8192785245846476)
(34, 0.27813197830777314)
(35, 0.46870670522284186)
(36, 0.10920026262597772)
(37, 0.20864667069642684)
(38, 0.4244781866992246)
(39, 0.35565517694730375)
(40, 0.6931896941137347)
(41, 0.8544502936843147)
(42, 0.7051145235146656)
(43, 0.0008980825894300271)
(44, 0.37551551617936946)
(45, 0.6973800856257657)
(46, 0.8417541612307708)
(47, 0.9046823988421495)
(48, 0.7730400294200046)
(49, 0.7334984384417377)
(50, 0.7253907322876056)
}


\newcommand{\drawPixelThree}{%
(1, 1.2307938511773404)
(2, 0.016756171859752957)
(3, 0.22485296114412967)
(4, 0.4319756634142318)
(5, 0.3710799876466322)
(6, 0.8718526746230418)
(7, 0.9429933761804365)
(8, -0.32350448594561965)
(9, 1.3343201797680826)
(10, 0.9095932665995297)
(11, 0.20780402468248374)
(12, 0.35123292756635244)
(13, 0.8924641298211747)
(14, 2.3265224016878983)
(15, 1.951634988810546)
(16, 2.0035042662694638)
(17, 0.36771645607520503)
(18, -0.8807159301256192)
(19, -0.15020926553065694)
(20, 0.48635473234176907)
(21, -1.307309012403855)
(22, -0.5970414421131334)
(23, -1.8325832912967892)
(24, -2.4801360727933353)
(25, -1.0490985030692093)
(26, -0.4078213276254965)
(27, -0.4163864123229731)
(28, -0.5706782623428324)
(29, -0.4048972808839259)
(30, -0.32934797140717015)
(31, -0.40623861903748715)
(32, -0.7090781398659681)
(33, -0.5909316120550624)
(34, -0.7018792848969593)
(35, -1.6680968211543648)
(36, -1.063656092153313)
(37, -0.8140243026455313)
(38, -0.9225251096240019)
(39, 0.07953727012738343)
(40, -0.5280294846691838)
(41, -0.5540442477076432)
(42, -0.5065052249311652)
(43, -0.326548730064637)
(44, -0.6242036234858707)
(45, -0.6871207142887392)
(46, -0.5036850130966758)
(47, -0.2764599750599551)
(48, -0.17419053924008837)
(49, -0.23307992118073317)
(50, -0.24203412986123166)
}


\newcommand{\drawPixelFour}{%
(1, 0.09463861022870025)
(2, -0.027528912378681537)
(3, -0.45413823148776744)
(4, -0.06241560935139571)
(5, 0.3297855641560095)
(6, -0.2213520145726101)
(7, -0.8979540980711394)
(8, 0.44361948206111523)
(9, 1.5182682271896497)
(10, 0.8811755867789942)
(11, 0.1347658287502361)
(12, 0.09403661418408489)
(13, 0.7124546934037269)
(14, 1.3677455706021848)
(15, 0.40330696625797235)
(16, 0.9442557746910054)
(17, 0.6463713924636916)
(18, 0.07194742545714249)
(19, 0.7341181972118314)
(20, -0.9264776107042533)
(21, 0.09008328195045243)
(22, 1.3749637023942607)
(23, 2.1406186763658908)
(24, 1.569739686645511)
(25, 1.382607581016451)
(26, 1.3465728191752948)
(27, 0.3957259882805574)
(28, -1.4073895813078987)
(29, -1.2159325835248262)
(30, -0.39821317551144514)
(31, -0.40412388200579763)
(32, -0.49743220323465764)
(33, -0.04774131537378119)
(34, -0.583237471924714)
(35, -0.08280981568113488)
(36, -0.45345613004814317)
(37, -0.7985982147328099)
(38, -0.7174592658542729)
(39, -0.5754619771406528)
(40, -0.2234491208231184)
(41, 0.012488107699961656)
(42, -0.0181066201494878)
(43, 0.33461901474457034)
(44, 0.49321282192533716)
(45, 0.28478888065090413)
(46, -0.09080506037380508)
(47, -0.0725392179289617)
(48, -0.11635557395024176)
(49, -0.04724122484238415)
(50, -0.054271183689209614)
}


\newcommand{\drawPixelFive}{%
(1, -0.03359248906362733)
(2, -0.8145866691284981)
(3, -0.45869148133408544)
(4, -0.7502014223982205)
(5, -0.5442837928951275)
(6, -1.034101816603664)
(7, -0.6042856936412896)
(8, -1.0401179662580686)
(9, -0.6029743826888304)
(10, 0.7706868453752138)
(11, 1.777206798661969)
(12, 2.032036703808533)
(13, 1.1140552393417589)
(14, 1.4046104198798315)
(15, 1.0394567169184195)
(16, 0.7647807152672897)
(17, -0.23588273107193447)
(18, 0.8343094792138369)
(19, 1.0129560487818294)
(20, -0.34951595084228765)
(21, -0.2293490610954866)
(22, -2.151958301378777)
(23, -1.2915854801275264)
(24, -1.1580862112112134)
(25, -1.0964703974895489)
(26, -0.5104980578054272)
(27, -0.3970337146489069)
(28, -0.6132312692971669)
(29, -0.9925124216849297)
(30, -0.5246454264112501)
(31, -0.14793079063332704)
(32, 0.10981943646812477)
(33, 1.0319903840650033)
(34, 0.301568119661431)
(35, -0.7537297403742333)
(36, 0.22459150024919589)
(37, -0.12750331666138454)
(38, 0.33084122569360913)
(39, -0.2834598844232472)
(40, 0.5022006734449452)
(41, 0.6821224929002124)
(42, 0.4264437444288789)
(43, 0.5090569952167407)
(44, 0.4800820429717805)
(45, 0.504528378959292)
(46, 0.6072531382911531)
(47, 0.46708676799553217)
(48, 0.4103135733073186)
(49, 0.37297420170829715)
(50, 0.37566226265442515)
}


\newcommand{\drawPixelSix}{%
(1, 0.8997626425836398)
(2, 0.6988966098174375)
(3, 0.3580099647558156)
(4, -0.22243608341795362)
(5, -0.043502533279718994)
(6, -0.5775478315037818)
(7, -0.387988450625507)
(8, 0.23348528841952787)
(9, -0.13580390409048407)
(10, -1.387795423232067)
(11, -0.2137395332263877)
(12, 0.9039447188858021)
(13, 1.209806290738479)
(14, 0.5781720408178723)
(15, 0.35591419956117093)
(16, -0.3038954247474406)
(17, -1.178355208361927)
(18, -0.8803222924131149)
(19, -1.529659667009428)
(20, -1.0150490784289063)
(21, 0.14196008749554317)
(22, 0.08455424481260959)
(23, 0.9192407210129833)
(24, 0.4916280006104547)
(25, 0.7130730977696009)
(26, 1.3805226888300273)
(27, 1.6256830056677056)
(28, -0.8059622722532929)
(29, -0.9987772765762357)
(30, -0.5449207666957222)
(31, -1.1719747185574865)
(32, -1.0261002622446904)
(33, -0.8994822870333626)
(34, -0.2034151759092865)
(35, 1.6332743614681375)
(36, 1.2070446308990048)
(37, 1.024671189647147)
(38, 0.3322872126116983)
(39, 0.573633665512474)
(40, 0.2840235747073982)
(41, 0.2230342750724634)
(42, 0.05309561592366621)
(43, -0.008359747841948928)
(44, 0.4144635336337537)
(45, 0.25035807348577266)
(46, 0.24618829736454945)
(47, 0.2856875083973901)
(48, 0.2600730279945526)
(49, 0.2578803515988604)
(50, 0.25596135370523015)
}


\newcommand{\drawPixelSeven}{%
(1, 0.3903883052571334)
(2, 1.1994512518340643)
(3, 0.7473069804715949)
(4, -0.3874508450094206)
(5, -1.0639731700731407)
(6, -0.5739991320095535)
(7, -1.3454993936059987)
(8, -1.1144021862229734)
(9, -1.6583483348520602)
(10, -2.0515843980090844)
(11, -1.736970263348557)
(12, -1.4793284894264762)
(13, -2.860707693359355)
(14, -0.7910768640480609)
(15, -0.9177145473962571)
(16, -0.27997677500438095)
(17, 0.17028531381077638)
(18, -0.5554066493335558)
(19, -1.397627650287873)
(20, -0.3434529001229847)
(21, 0.9914822604444543)
(22, 0.9332413935347627)
(23, 1.0397915395987527)
(24, 0.4086965200363206)
(25, -0.10097784017400027)
(26, 0.4104906687517458)
(27, 1.1414166848824319)
(28, 1.7680083391364316)
(29, 2.2133631883564098)
(30, 1.7379573552498995)
(31, 1.9559561789230415)
(32, 1.1337168131795219)
(33, 1.939293934523991)
(34, 1.6347951207313205)
(35, 0.4487340810506194)
(36, 1.8481569732417713)
(37, 1.2578181395821086)
(38, 0.5007393088242067)
(39, 0.4604774091987809)
(40, 0.41776327121886364)
(41, 0.277509656808546)
(42, 0.8999419882894488)
(43, 0.7337651565021535)
(44, 0.8703443278821801)
(45, 0.6549595285284981)
(46, 0.6725589502573166)
(47, 0.5865988439952474)
(48, 0.2979260967311293)
(49, 0.385079618677816)
(50, 0.3835359137239963)
}


\newcommand{\drawPixelEight}{%
(1, -1.0371553588742228)
(2, -0.5052196382169573)
(3, -1.2844950414312075)
(4, -1.6253377768062691)
(5, -1.126093675182298)
(6, -1.6690852579375957)
(7, -2.0406818310282016)
(8, -1.2881269260204529)
(9, -1.2812965403012349)
(10, 0.3470830461486993)
(11, 0.29624637420668737)
(12, -0.10056983104139319)
(13, -0.5943003272093594)
(14, -1.4231310549657754)
(15, -1.0609453920808682)
(16, -1.5544281855318545)
(17, -2.318940621985953)
(18, -1.6677625851535485)
(19, -0.5914654260243272)
(20, 0.07616003887075234)
(21, -0.06394791250232988)
(22, -0.5354840120683496)
(23, -0.6080701588600249)
(24, 0.06976131024523362)
(25, -0.08057737060611089)
(26, 0.03877306011754727)
(27, 0.5335968421620609)
(28, 0.05605074726669254)
(29, 0.38476910528933295)
(30, 0.6208931637050877)
(31, 0.019902910970345022)
(32, 1.387627035282811)
(33, 0.057118656642784676)
(34, -0.6010324885557725)
(35, -0.2043261850488611)
(36, 0.6775301008170861)
(37, 0.8861842928327179)
(38, 0.2629677015829629)
(39, 1.0638044093961991)
(40, 0.4954369512705613)
(41, 0.9525357436023004)
(42, 0.7540778415144502)
(43, 1.3093200468486943)
(44, 0.7889872615263972)
(45, 0.8028375764496134)
(46, 0.9403357012037683)
(47, 0.7772879658388245)
(48, 0.43481088268599194)
(49, 0.41824665081941)
(50, 0.42814821345367643)
}


\newcommand{\drawPixelNine}{%
(1, 0.14187627846726464)
(2, 0.3106932303789995)
(3, -0.723900216512481)
(4, -0.7291644377528015)
(5, -0.7803878341752113)
(6, 0.5931753808560044)
(7, 0.550670900586288)
(8, 0.41472602386579094)
(9, 0.2331141533102381)
(10, 0.715143887126995)
(11, 1.864394952283261)
(12, 1.994782460784268)
(13, 1.1050952082718204)
(14, 2.0206334193051947)
(15, 0.19606253534119458)
(16, -0.84129784304984)
(17, 0.038656650076179876)
(18, 0.283304432079605)
(19, 0.859408150646495)
(20, 0.5784752629371339)
(21, 0.9842692885104993)
(22, 0.7401691305034596)
(23, -0.11780452765449595)
(24, 1.0850086462052573)
(25, 0.8700125314019003)
(26, 0.765990603254599)
(27, -0.8395375030725584)
(28, -1.2045507186910114)
(29, -1.2960798624517986)
(30, -0.2972795368639923)
(31, -0.33831408580884914)
(32, 0.6112763138694062)
(33, -0.18871736272162673)
(34, 0.6175833759132484)
(35, 0.5131596402789499)
(36, 0.22663964859052838)
(37, 0.5121829131082983)
(38, 0.9297832806266546)
(39, 0.7150636192575951)
(40, 0.7314006443232992)
(41, 0.5204328443825981)
(42, 0.5419720272642181)
(43, 0.24228078794312027)
(44, 0.2577551955073627)
(45, 0.9161514008311209)
(46, 0.6486113369872961)
(47, 0.7114577439696066)
(48, 0.6829417574304872)
(49, 0.4920633113553427)
(50, 0.502350421084999)
}


\newcommand{\drawPixelTen}{%
(1, -1.8832212222624158)
(2, -1.0536978442384237)
(3, -1.2775988917984455)
(4, -1.405935528660242)
(5, -2.152319028718155)
(6, -0.6478994501495622)
(7, -0.6340344786495742)
(8, -0.18484501669975759)
(9, 1.051701492103573)
(10, 1.3310664698694468)
(11, 0.541038645162534)
(12, 0.2989149258277439)
(13, -0.6768270540219617)
(14, -0.49953728433130257)
(15, -1.1661494332526452)
(16, -1.2389807082852193)
(17, -0.9453990766262268)
(18, -0.5395893401673845)
(19, -0.3258110697834808)
(20, -0.3552932909003033)
(21, -0.8738213984586976)
(22, -0.04346829313112418)
(23, -0.790432118838558)
(24, -0.23025512010859922)
(25, 0.6285046396657246)
(26, 0.7087540574761269)
(27, 0.7925679774032757)
(28, -0.14788987518857483)
(29, 0.17350922353216736)
(30, -0.04846034885475166)
(31, 0.7534521252435187)
(32, 0.5896118909528428)
(33, 0.19607649950310768)
(34, -0.4830220977227694)
(35, -0.06089737652028063)
(36, -0.8074485759053538)
(37, -0.43261867993665704)
(38, -0.5647392537889215)
(39, -0.4809573678207112)
(40, -0.29592436596016997)
(41, -0.6169701069435058)
(42, 0.2066595848432004)
(43, -0.09657913657733586)
(44, -0.13209011780822638)
(45, -0.06513804081700808)
(46, 0.41868215430593037)
(47, 0.5949602412513278)
(48, 0.5384626738428002)
(49, 0.5070773769204207)
(50, 0.510275781603442)
}


==> data/drawPixel4_cifar.tex <==
\newcommand{\drawPixelOne}{%
(1, 0.5455710666656857)
(2, 0.047587600608478484)
(3, -0.5392375053975494)
(4, -0.7586126102829638)
(5, -0.713023454274746)
(6, 0.17746834274309128)
(7, -0.10210919630950861)
(8, -0.04973042986578648)
(9, 2.2719113291974744)
(10, 2.1815449687731765)
(11, 0.8538626915939082)
(12, 0.6619566574715843)
(13, 2.766138431007927)
(14, 2.7515633734822753)
(15, 2.2864674871142836)
(16, 0.8282804398825371)
(17, 1.221995410608304)
(18, 0.7899052762668046)
(19, 0.1667806710461067)
(20, -0.4534246144672085)
(21, -0.5880055885236312)
(22, 0.06502640858373923)
(23, -0.807850189090092)
(24, -0.5128406937763752)
(25, -1.04517263625602)
(26, -1.106768154282117)
(27, -1.673925750613325)
(28, -0.7440056277629796)
(29, -0.9916612651216431)
(30, -0.639364827191851)
(31, -0.7862672307307168)
(32, -0.8234336984584564)
(33, -0.7648224084586673)
(34, -0.7853340197886722)
(35, -0.6400620766705387)
(36, 0.181596886734555)
(37, -0.37767971263700784)
(38, -0.5226423225446577)
(39, -0.2763525792024757)
(40, -0.91529132925758)
(41, -0.2974587565323039)
(42, -0.009433075636600702)
(43, -0.4760625416105412)
(44, -0.3659609507339742)
(45, -0.1602191352332472)
(46, -0.1702771981684106)
(47, -0.17147194864388146)
(48, -0.01850842163730118)
(49, 0.07547274064483717)
(50, 0.07530159006872648)
}

\newcommand{\drawPixelTwo}{%
(1, -1.5015452229273056)
(2, -0.9396139235430092)
(3, 0.050500688969410915)
(4, 0.42571881674165357)
(5, -0.8683458811265036)
(6, 0.36463915721032886)
(7, 1.0319582903961857)
(8, 1.274540150850373)
(9, 0.9098992542769926)
(10, 0.6315496641207413)
(11, -0.20196308946672356)
(12, 0.3261415831920459)
(13, -0.287980884341053)
(14, -0.34356668135583734)
(15, -1.277057327236221)
(16, -1.287987903204881)
(17, -0.5127877241049931)
(18, -0.2216098460441277)
(19, 0.0438553565222636)
(20, 0.6666656168551611)
(21, -0.1456573823878117)
(22, 0.39183956816975196)
(23, 0.7204033289339595)
(24, 1.0810604255046083)
(25, 0.4866144199272814)
(26, 1.40066988549158)
(27, 1.1318524673578048)
(28, 0.5642052672660355)
(29, 1.1033501489805349)
(30, 0.7715191803399213)
(31, 1.0497436828032174)
(32, 0.6000849825810489)
(33, 1.3715152156148473)
(34, 1.590790947862126)
(35, 1.4993660761331968)
(36, 1.1657309073836983)
(37, 0.7709899377735375)
(38, 1.1949098747048048)
(39, 1.09113862884531)
(40, 1.1590374074945202)
(41, 1.5428209839262246)
(42, 0.9464879432062869)
(43, 0.6714357675466767)
(44, 0.55378866240973)
(45, 0.5866470351077717)
(46, 1.0185037308557963)
(47, 0.7235738648900362)
(48, 0.5135651491606854)
(49, 0.39466865168816256)
(50, 0.3976991255231494)
}

\newcommand{\drawPixelThree}{%
(1, -0.257898631522387)
(2, 0.023569255820194937)
(3, 0.04544431270862937)
(4, -0.10144158940110493)
(5, -0.7785714493985482)
(6, -1.4103543673859005)
(7, -3.39037797816054)
(8, -2.872151114160582)
(9, -0.9448632962824012)
(10, 0.42019431741937235)
(11, 0.8460715324165394)
(12, 0.15965073021531445)
(13, 1.2097450509917986)
(14, 0.5193515465818941)
(15, -0.9008394869813104)
(16, -1.3824534481209871)
(17, -0.8209570349518565)
(18, -0.0934748876033907)
(19, -0.7535401717458167)
(20, 0.11869949928892659)
(21, 0.6932033629029517)
(22, 0.17146902917227033)
(23, 0.292692906228209)
(24, 0.07734232267571997)
(25, 0.24360056474542646)
(26, 0.9296952580415044)
(27, 0.6135953249855737)
(28, -0.46340373239779475)
(29, -0.49642871526158266)
(30, -0.002345812294858757)
(31, -0.23269419129400298)
(32, 0.02104913879552163)
(33, -0.24712090038732423)
(34, -0.15253211344025785)
(35, -0.13878861884898763)
(36, 0.14444236291863252)
(37, -0.2894901974011967)
(38, -0.4562981703853661)
(39, -0.20962350872742447)
(40, -0.3187091211378783)
(41, 0.40536965093110905)
(42, -0.24154116371009896)
(43, -0.6912220513170229)
(44, -1.084469999175489)
(45, -0.9592428224499555)
(46, -0.8913455060134603)
(47, -0.5344444211805751)
(48, -0.5188065896753142)
(49, -0.43017225599273246)
(50, -0.4294112606637348)
}

\newcommand{\drawPixelFour}{%
(1, 0.8580893881079756)
(2, 1.4626682599582068)
(3, 1.9522555397082546)
(4, 1.9469156691095193)
(5, 2.1498785923524752)
(6, 1.6075092380643983)
(7, 1.9828821703111945)
(8, 1.8314607585010776)
(9, 0.003142350116185507)
(10, -0.23491852634331803)
(11, 1.08143169303857)
(12, 1.7160170488840993)
(13, 1.9049314194713907)
(14, 1.2836623405508327)
(15, 2.3950657083301636)
(16, 1.9252484781547248)
(17, 1.0259103413959292)
(18, 1.7155509498858383)
(19, 2.087043402200119)
(20, 2.356923172897426)
(21, 2.4041690504131337)
(22, 0.8856292047497109)
(23, 1.4604814323313318)
(24, 0.5130584531423078)
(25, 0.06552932918959144)
(26, -0.1982563720286855)
(27, 1.788594282245813)
(28, 1.2789285014855032)
(29, 0.28542376542750886)
(30, -0.1044490405321721)
(31, -0.0798047126178936)
(32, -1.4419649238153935)
(33, -0.29858833661587647)
(34, -0.13409451493682611)
(35, -0.2065821937169903)
(36, 0.05205483098477651)
(37, 0.06246337584320444)
(38, 0.4632307863348645)
(39, 1.050424554576635)
(40, 1.5029497630772986)
(41, 1.1852167309748376)
(42, 1.132871071838969)
(43, 1.3833800167401173)
(44, 1.1224829968143137)
(45, 1.1496273782186788)
(46, 1.1039958772880734)
(47, 1.006017624350557)
(48, 0.8860753882582244)
(49, 0.9367810952185154)
(50, 0.9197939369643401)
}

\newcommand{\drawPixelFive}{%
(1, 0.10166407389100876)
(2, 1.1326660015300754)
(3, 0.5067396318547034)
(4, 1.4564245066526549)
(5, 0.4690276810430686)
(6, -0.8916349235883332)
(7, -0.9976344089811515)
(8, -0.8754005809835611)
(9, -0.3787655977529478)
(10, 0.061781129170784)
(11, -0.8501525969070443)
(12, 1.0766692146532708)
(13, 1.8359358814687667)
(14, 2.2690538960765814)
(15, 1.7943545704048196)
(16, 0.5715997107188181)
(17, 0.3083153857137222)
(18, 1.4059641395136022)
(19, 2.095929180952025)
(20, 0.36614429231739176)
(21, 0.9318106513217225)
(22, -0.08931726241636778)
(23, -0.8607544274116696)
(24, -0.7442666761810686)
(25, -0.5640396492837972)
(26, 0.10899512657236739)
(27, 0.6700603372018288)
(28, -0.2242268244391883)
(29, 0.004813733103541339)
(30, -0.029451339604682193)
(31, -1.1262964766797903)
(32, -0.5541390066301549)
(33, -1.0877463298924006)
(34, -0.41730148801809597)
(35, -0.28083671034958335)
(36, -0.6331317608291475)
(37, 0.15798865343638796)
(38, 0.2742061359171117)
(39, -0.09156828389997335)
(40, -0.2377226410114239)
(41, 0.14542620650557148)
(42, -0.6825492887703312)
(43, 0.18234700099252946)
(44, 0.038774097625764836)
(45, 0.36339143677733565)
(46, 0.5714734748930763)
(47, 0.4154963231924704)
(48, 0.37896333471585025)
(49, 0.16932335622766126)
(50, 0.15355632779686945)
}

\newcommand{\drawPixelSix}{%
(1, -0.9479339708863314)
(2, 1.047368182525387)
(3, 0.5899650245018855)
(4, -0.01551003456914118)
(5, 0.2914288733410109)
(6, -0.6545554560518738)
(7, -0.5676398988457563)
(8, 0.4519405244920033)
(9, -0.024386286241766697)
(10, -0.8195562168742557)
(11, -0.7401245423756583)
(12, -0.34305638963675433)
(13, 1.0275956918418547)
(14, 0.7997513020537442)
(15, 1.1316524943730701)
(16, 0.7457707367966557)
(17, -0.4036912986018866)
(18, -1.0746071892632187)
(19, -0.9417633515121361)
(20, -0.4500957293522344)
(21, -0.7042286024588881)
(22, -0.13831526850096337)
(23, -1.2142451121318962)
(24, -1.2984509418117482)
(25, -1.825650829012965)
(26, -1.8878980900536468)
(27, 0.3737433907747536)
(28, 0.44205772846780456)
(29, 0.6532062287981061)
(30, 1.062589856554154)
(31, 0.9665410687321603)
(32, -0.2374497174712553)
(33, 0.036367745043893035)
(34, 0.16391920408028327)
(35, 0.6269194483191698)
(36, 1.1064189693425752)
(37, 1.361379235966931)
(38, 1.181110805086444)
(39, 0.19248463938026256)
(40, 1.1126928855963993)
(41, 0.2761108808660973)
(42, 1.1807517562035674)
(43, 1.5294416262373924)
(44, 1.3082788062709516)
(45, 0.8575956152524916)
(46, 1.0661910253428606)
(47, 0.9717857045982141)
(48, 0.8476743688334492)
(49, 0.9253419442333195)
(50, 0.9259651856966704)
}

\newcommand{\drawPixelSeven}{%
(1, 0.2520548963223668)
(2, 0.8004919938368091)
(3, -0.6348815081711484)
(4, 0.5679510362794078)
(5, 1.2217099546769612)
(6, 1.3303939794576574)
(7, -0.03839452989890099)
(8, 0.2978264882501128)
(9, 0.8411866353331865)
(10, 1.887851715434958)
(11, 2.400454772685135)
(12, 1.5227176652276238)
(13, 2.09955618800974)
(14, 1.5488931576653036)
(15, 1.5431238029294756)
(16, 1.1286925125790919)
(17, 1.2356043275017683)
(18, 1.3856514175689694)
(19, 1.4895896882752189)
(20, 1.544665721712617)
(21, 2.1558849557181192)
(22, 1.5721533292976833)
(23, 1.343166291850946)
(24, 1.656854964355569)
(25, 2.199831777599824)
(26, 1.989632448968283)
(27, 1.9330947051104137)
(28, 1.2092163484259992)
(29, 0.182241540547469)
(30, 1.3589780687329363)
(31, 1.1434084595781067)
(32, 0.6916855370846928)
(33, 0.16593305223591742)
(34, -0.26487432888164797)
(35, 0.8496637646881677)
(36, 0.4613759242294191)
(37, 1.4810400865043285)
(38, 1.6580826388679215)
(39, 1.8030519671624696)
(40, 1.1605163275846189)
(41, 1.0475895956021788)
(42, 1.1329722233696946)
(43, 1.4998107438979662)
(44, 1.4884965178483955)
(45, 1.2902464358617276)
(46, 1.340876921068993)
(47, 1.2466204868948796)
(48, 1.045370136796738)
(49, 0.8322922446496364)
(50, 0.8427693270992485)
}

\newcommand{\drawPixelEight}{%
(1, 1.0602008275765595)
(2, 0.618559042868281)
(3, -0.3203443855880798)
(4, -1.0348747165083594)
(5, -0.05973465152446679)
(6, 1.1397987857612286)
(7, 1.5256420728234052)
(8, 0.7450024550451958)
(9, 0.41330905156248116)
(10, 0.03192747511945584)
(11, 0.485627180876539)
(12, 0.48373251679418955)
(13, 0.6128655728435222)
(14, 1.4101339625693616)
(15, 1.1696716252990993)
(16, 0.720738255154929)
(17, 0.9138546664993955)
(18, 0.8638072025560399)
(19, 2.361445691287071)
(20, 1.369863877791075)
(21, 0.9624123902867315)
(22, 0.6829825922748433)
(23, -0.3359702122512898)
(24, 0.0029618717035625325)
(25, 0.08378610229484709)
(26, 0.7207248082705744)
(27, 0.733959421701601)
(28, 0.7042803886834339)
(29, 0.1387961650397521)
(30, 0.365558520329476)
(31, 1.3743857970377653)
(32, 0.7919480521669888)
(33, -0.5596375455937623)
(34, -0.8691967107991284)
(35, -0.010021116700358573)
(36, -0.03171830445604795)
(37, 0.16068939392763795)
(38, -0.20799957093406182)
(39, -0.037385003456780114)
(40, 0.32929932009702495)
(41, 0.42221457962757486)
(42, 0.32930469801300627)
(43, 0.2338631181058966)
(44, 0.40876379003730184)
(45, 0.26607206968891906)
(46, 0.1707737625790511)
(47, 0.09826523101624285)
(48, 0.032803274023899445)
(49, 0.09813582798669918)
(50, 0.09698491108081181)
}

\newcommand{\drawPixelNine}{%
(1, 0.20213200490708383)
(2, -0.6359241599391265)
(3, 0.5371783912925137)
(4, 0.6611001064397269)
(5, 0.09735432758913974)
(6, 0.3340499098977065)
(7, 0.1610201271243729)
(8, -0.06448572017217878)
(9, 0.5423316073090342)
(10, 1.1380646777453123)
(11, 1.2925619504302492)
(12, 1.4802803255540453)
(13, 1.9806017158408182)
(14, 1.5841150901361207)
(15, 2.2154319384618293)
(16, 0.9941128605965295)
(17, 0.8431827949550508)
(18, 0.3294461892241324)
(19, 0.7440189600361121)
(20, 0.263129102328902)
(21, -0.48118400775538167)
(22, -0.6575321969662565)
(23, -0.15961924914563086)
(24, -0.6750103037233415)
(25, 0.056576580696741846)
(26, 0.9902734648359053)
(27, 0.42656257679420795)
(28, 0.26472776208397564)
(29, -0.7466356373343839)
(30, -0.5819428713323281)
(31, 0.641488992661498)
(32, 0.0697600893080213)
(33, 1.5612640257682766)
(34, 1.3136600375138612)
(35, 0.3736297474454719)
(36, 0.22266278256657845)
(37, 1.423234928263619)
(38, 0.5604342477379164)
(39, 0.19741840012000034)
(40, -0.2720402520729139)
(41, 0.1936862893785363)
(42, 0.5542428959101227)
(43, 0.906848611480797)
(44, 0.8031918266618218)
(45, 0.7570375879131732)
(46, 0.952657017509235)
(47, 0.7912644866801118)
(48, 0.717706509384259)
(49, 0.7678329775452994)
(50, 0.7668676921664853)
}

\newcommand{\drawPixelTen}{%
(1, -0.5451944118727557)
(2, -1.179249813548714)
(3, -1.7324970819169747)
(4, -2.160124973271396)
(5, -1.5686621288178497)
(6, -0.6155140864116974)
(7, -0.09617703145060584)
(8, 0.3888415064331436)
(9, 1.2626958390423855)
(10, 1.1216307748185645)
(11, 0.8844113567999391)
(12, -0.3972870640097731)
(13, -1.3146976433360547)
(14, -0.3267208633928772)
(15, 0.03143452290075591)
(16, -0.6115204563193753)
(17, -0.3106003399661317)
(18, 0.3046110443316)
(19, 0.3805692429180936)
(20, 0.5587369155856542)
(21, 0.5526220219990701)
(22, 1.820163528086788)
(23, 2.395049696518488)
(24, 1.5468677307354755)
(25, 0.38361601883413493)
(26, 0.8858501763417543)
(27, 0.5185141035148049)
(28, 1.50032045475999)
(29, -0.0020547582296344957)
(30, 0.04250535663834473)
(31, 1.0041528491627676)
(32, 0.995433664002903)
(33, 0.7179952035732711)
(34, 0.6438732015194291)
(35, 0.8706388155635121)
(36, 0.5868583308185358)
(37, 0.39168775015767365)
(38, 0.2514749273837537)
(39, 0.6589557887519927)
(40, 0.6259439980327979)
(41, 0.680106790497319)
(42, 0.8400011533362114)
(43, 1.189380349679634)
(44, 0.9029410472744521)
(45, 0.6483638757829924)
(46, 1.0447888928689004)
(47, 1.0198711853944489)
(48, 0.957066336880484)
(49, 0.9225184774427003)
(50, 0.9210131447675509)
}

==> data/drawPixel5.tex <==
\newcommand{\drawPixelOne}{%
(1, -0.7878121833967535)
(2, -0.09391458684281688)
(3, -0.10364730995864013)
(4, 0.7031294032140258)
(5, 0.5934009861790633)
(6, -0.5045425347691418)
(7, 0.24817089545247958)
(8, 0.8628512905792529)
(9, 1.3666191022697334)
(10, 2.3765843797763115)
(11, 2.1224219743757304)
(12, 0.9929608632464758)
(13, 2.1260172779346815)
(14, 2.066973897144831)
(15, 2.247095384331428)
(16, 2.336801466121246)
(17, 1.831998466456933)
(18, 0.7781207052437926)
(19, -0.2951097288322929)
(20, -0.1341669701842666)
(21, -0.2727310540921395)
(22, 0.26834577609413823)
(23, 0.8970027308154686)
(24, -0.6258725052767429)
(25, -0.07402000143447773)
(26, -0.11064140135795934)
(27, -1.1142586583827265)
(28, -0.6839601954786135)
(29, -0.8178422991138703)
(30, 0.03208346507833626)
(31, 0.022767874937415944)
(32, -0.25811032146930823)
(33, 0.029036059275109938)
(34, -0.28529253421840534)
(35, -0.6231060435776552)
(36, -0.45017476417390023)
(37, -0.5483970613756178)
(38, -0.5163987219521446)
(39, -0.72632757091119)
(40, -0.7831574348178574)
(41, -0.8883997195754659)
(42, -0.8426478544591464)
(43, -0.8260474341866468)
(44, -0.8575867831549908)
(45, -0.8339932313702151)
(46, -0.8409232401120876)
(47, -0.8442165814385463)
(48, -0.8320852083056345)
(49, -0.8305787705059077)
(50, -0.8304861685500596)
}


\newcommand{\drawPixelTwo}{%
(1, 0.7027502080584637)
(2, 1.905604061653017)
(3, 0.9382017552791282)
(4, 1.1084361293298444)
(5, 0.23098225868067485)
(6, 0.7279245992502876)
(7, -0.6360410097919803)
(8, -0.7261885443631771)
(9, -0.7659909787460542)
(10, -0.5349535309341402)
(11, -0.7119236546827143)
(12, -0.8931235689865719)
(13, -0.740089003102497)
(14, -1.4483827976920014)
(15, -0.6958037783912704)
(16, -0.9402496519099812)
(17, -1.7116914985453235)
(18, -1.6029697645930674)
(19, -1.0210482712222821)
(20, -0.9166036585053429)
(21, -1.7389389147719752)
(22, -1.6281751657597134)
(23, 0.24813650817543462)
(24, 0.2087745407063151)
(25, -0.23764580027253807)
(26, 0.47357488268792225)
(27, 0.3196334936202802)
(28, 1.7088973205972293)
(29, -0.03427663091090491)
(30, -0.44874261161897444)
(31, -0.12458508921216033)
(32, 0.4527687873452209)
(33, 0.6532567631270179)
(34, 0.387189742114546)
(35, 0.47133361997123485)
(36, 0.3371467991817377)
(37, 0.3493984134337215)
(38, 0.3838169414691492)
(39, 0.35963750924692384)
(40, 0.410433989674678)
(41, 0.42374633833466446)
(42, 0.4053733365648501)
(43, 0.3427752615979809)
(44, 0.369631976674896)
(45, 0.3904268499230314)
(46, 0.4021354128613862)
(47, 0.41125732293911116)
(48, 0.41056845668077696)
(49, 0.41132886587197504)
(50, 0.40907289347012216)
}


\newcommand{\drawPixelThree}{%
(1, 1.2304809673773223)
(2, 0.01654169593052553)
(3, 0.22463078945046075)
(4, 0.4317331208264677)
(5, 0.3709254936852211)
(6, 0.8718167265788764)
(7, 0.9430971237939572)
(8, -0.32327241800273804)
(9, 1.3354729529726967)
(10, 0.9108652034186581)
(11, 0.2093335730808461)
(12, 0.35272414748145636)
(13, 0.8948944766777752)
(14, 2.3303464235291407)
(15, 1.9565660992234775)
(16, 2.00758970147273)
(17, 0.36800992624334444)
(18, -0.8837008375858377)
(19, -0.15199779342007252)
(20, 0.48641022852499377)
(21, -1.3051331060627442)
(22, -0.5988877527009441)
(23, -1.824299539582228)
(24, -2.4593597723236003)
(25, -1.0180485047723205)
(26, -0.397058907465894)
(27, -0.36759720735874246)
(28, -0.4627378282552052)
(29, -0.29870750924692974)
(30, -0.3460778852791758)
(31, -0.5134306212801443)
(32, -0.7776242336505845)
(33, -0.7478261644062477)
(34, -0.8342750359622453)
(35, -1.206644921504725)
(36, -0.9643032920390131)
(37, -0.8696895834203437)
(38, -0.888729905508348)
(39, -0.7204064336654193)
(40, -0.8463373062481195)
(41, -0.8762023396956394)
(42, -0.8837964129039331)
(43, -0.8756786474512391)
(44, -0.9031354442914348)
(45, -0.9057022209580687)
(46, -0.8960843994310472)
(47, -0.8838740700672378)
(48, -0.8743405475703322)
(49, -0.8721652374949321)
(50, -0.8746072166440312)
}


\newcommand{\drawPixelFour}{%
(1, 0.09423685412155151)
(2, -0.028117637824797814)
(3, -0.4547202516314687)
(4, -0.06283796295550567)
(5, 0.3295124765095619)
(6, -0.22154168937069796)
(7, -0.8982357559640249)
(8, 0.44328192744765044)
(9, 1.517260590232653)
(10, 0.8804342319538364)
(11, 0.1337284348884307)
(12, 0.09284240480267768)
(13, 0.7115961301988569)
(14, 1.3676197797642757)
(15, 0.4008484781530396)
(16, 0.9410266767321902)
(17, 0.6417022895974885)
(18, 0.06539506279390056)
(19, 0.7292100952466167)
(20, -0.9298701501565751)
(21, 0.09069622525151008)
(22, 1.372317355328016)
(23, 2.125867624164686)
(24, 1.5523327625666072)
(25, 1.359219697102163)
(26, 1.3109422029690472)
(27, 0.42659208789217484)
(28, -1.114450346980487)
(29, -0.8501317819323533)
(30, -0.1357574284614812)
(31, -0.07074482745578134)
(32, -0.06159390149302707)
(33, 0.2366951102287311)
(34, 0.04472450627771024)
(35, 0.24703148603468797)
(36, 0.12265562917044648)
(37, 0.05394832088584407)
(38, 0.09539442915001753)
(39, 0.12702969428430427)
(40, 0.20445675979457364)
(41, 0.24207535271717126)
(42, 0.243330958497582)
(43, 0.2736852577892743)
(44, 0.2878609283646976)
(45, 0.27580526739971734)
(46, 0.25463844424672766)
(47, 0.2508488257822779)
(48, 0.2431969729239938)
(49, 0.2442526882885207)
(50, 0.24260736808890096)
}


\newcommand{\drawPixelFive}{%
(1, -0.03408355382624435)
(2, -0.8152120285000167)
(3, -0.45939674356556603)
(4, -0.7507968278621706)
(5, -0.5446907331313844)
(6, -1.0343185072608543)
(7, -0.6044121668269398)
(8, -1.040127369855494)
(9, -0.6032764621450426)
(10, 0.7714108490492684)
(11, 1.7783971156893053)
(12, 2.0334742271833552)
(13, 1.1159048906391034)
(14, 1.4070979813554487)
(15, 1.0384945548901825)
(16, 0.7610959240130094)
(17, -0.24187904860681617)
(18, 0.8291780597905342)
(19, 1.0090360980372333)
(20, -0.352773644408517)
(21, -0.22758788983534115)
(22, -2.1426033934320654)
(23, -1.2857713330493874)
(24, -1.1281159244017342)
(25, -1.033392569118215)
(26, -0.43214868875569157)
(27, -0.2797328598398039)
(28, -0.4167983973626772)
(29, -0.6574433290880897)
(30, -0.21975663374667082)
(31, 0.10415823376994532)
(32, 0.3083998358930319)
(33, 0.7987137030789777)
(34, 0.44548007029188164)
(35, 0.0369070547517453)
(36, 0.3775460726836231)
(37, 0.27255056452504156)
(38, 0.36488278214313913)
(39, 0.26097095653316293)
(40, 0.38009702958821806)
(41, 0.40253214827583095)
(42, 0.37089696500080477)
(43, 0.38399248488366117)
(44, 0.3816851149098934)
(45, 0.38439590321391487)
(46, 0.3911685375024763)
(47, 0.38619901043416155)
(48, 0.38321786180913553)
(49, 0.3782073580953401)
(50, 0.3787056358127724)
}


\newcommand{\drawPixelSix}{%
(1, 0.8992901330059171)
(2, 0.698173396099492)
(3, 0.3571980463464374)
(4, -0.22319570882712916)
(5, -0.044068549929151074)
(6, -0.5779513779930803)
(7, -0.3884345197329139)
(8, 0.2327970591388984)
(9, -0.13746544356196727)
(10, -1.3893050537529614)
(11, -0.21537402196957198)
(12, 0.9024266403338358)
(13, 1.2081616504887962)
(14, 0.5742415560510767)
(15, 0.35023054512567436)
(16, -0.31175972977585803)
(17, -1.188406850805089)
(18, -0.890727057163976)
(19, -1.5396100011443685)
(20, -1.022592096139806)
(21, 0.13678098488908427)
(22, 0.08189354315236128)
(23, 0.9111323327275247)
(24, 0.48891053030653125)
(25, 0.7082256264070553)
(26, 1.338522248828313)
(27, 1.5385286595618533)
(28, -0.6045284943535815)
(29, -0.6797854153940635)
(30, -0.2433633218135122)
(31, -0.5835305023830708)
(32, -0.38063774529689653)
(33, -0.2011717050054811)
(34, 0.16764299241666689)
(35, 0.882925821746047)
(36, 0.7099521320606335)
(37, 0.624968978221896)
(38, 0.4223597138182082)
(39, 0.4557240567304207)
(40, 0.3944430686103986)
(41, 0.36582023971335836)
(42, 0.33826048246006285)
(43, 0.3271442417772769)
(44, 0.35967524433437853)
(45, 0.34640010983468345)
(46, 0.34246374983410094)
(47, 0.3416550470875801)
(48, 0.34074779703502706)
(49, 0.34401444352357946)
(50, 0.34307836677828685)
}


\newcommand{\drawPixelSeven}{%
(1, 0.38996125112327296)
(2, 1.1987562269961443)
(3, 0.7465418906632993)
(4, -0.38809195453469747)
(5, -1.0643892118820282)
(6, -0.574343019630757)
(7, -1.3459349015907218)
(8, -1.1151240576002033)
(9, -1.6601658151832888)
(10, -2.0533551667753773)
(11, -1.7390942926058757)
(12, -1.4815858079390367)
(13, -2.8647752923104752)
(14, -0.7953063549895031)
(15, -0.9227149936970724)
(16, -0.28479165398207906)
(17, 0.1648825290279497)
(18, -0.5633286190701595)
(19, -1.4059363155732636)
(20, -0.3498445196854263)
(21, 0.985076750140705)
(22, 0.9244023855128549)
(23, 1.0277429961727966)
(24, 0.40343248181323993)
(25, -0.08092103566034026)
(26, 0.42108002231998537)
(27, 1.0938179845135108)
(28, 1.6020250827654907)
(29, 1.8859123659952277)
(30, 1.4125814541678787)
(31, 1.4454085991821792)
(32, 0.8163048369865331)
(33, 1.1618098808943058)
(34, 0.9346599861465548)
(35, 0.4497411185489057)
(36, 0.8788908393705739)
(37, 0.6628665632195488)
(38, 0.4593663888788846)
(39, 0.44210834892961864)
(40, 0.41596503115004757)
(41, 0.3969534215181553)
(42, 0.47350626289285774)
(43, 0.462861870848227)
(44, 0.4744912380448095)
(45, 0.46485004311759454)
(46, 0.46760570963734915)
(47, 0.46586708794954806)
(48, 0.4535260983078224)
(49, 0.4570106864960089)
(50, 0.4555028063612709)
}


\newcommand{\drawPixelEight}{%
(1, -1.037588339822272)
(2, -0.5058870707585053)
(3, -1.2851791291504577)
(4, -1.625835612546)
(5, -1.1264220315839744)
(6, -1.6693021761515705)
(7, -2.040978428072962)
(8, -1.2884836037975331)
(9, -1.2824840900045742)
(10, 0.34647232822120794)
(11, 0.29569758297271426)
(12, -0.10140416038335995)
(13, -0.5951767331259329)
(14, -1.42419048052606)
(15, -1.0640562815623107)
(16, -1.560691186185364)
(17, -2.327864416849217)
(18, -1.6769133920830326)
(19, -0.5978596831678543)
(20, 0.07317010253592643)
(21, -0.061918577861545684)
(22, -0.5253416263634993)
(23, -0.5857969665957349)
(24, 0.09110869257541142)
(25, -0.042417132010535485)
(26, 0.08903906040222276)
(27, 0.5614545725594406)
(28, 0.15272220864277405)
(29, 0.4428513640476554)
(30, 0.6162076439232935)
(31, 0.217177432795431)
(32, 1.0516975470785694)
(33, 0.32012671134914883)
(34, 0.07921754231598394)
(35, 0.2882985592685565)
(36, 0.5861530357356234)
(37, 0.6306110130503463)
(38, 0.4766448442445528)
(39, 0.6220398843791066)
(40, 0.5404377715796005)
(41, 0.5897565584693513)
(42, 0.5664001129032806)
(43, 0.6173112928483605)
(44, 0.5843302207603149)
(45, 0.588256254025724)
(46, 0.6028122621216052)
(47, 0.6033876164982217)
(48, 0.5905693897390214)
(49, 0.5864467002303945)
(50, 0.5892035814931651)
}


\newcommand{\drawPixelNine}{%
(1, 0.14147861402465622)
(2, 0.3100976828384894)
(3, -0.7244770645118805)
(4, -0.7295750640157094)
(5, -0.780650342551549)
(6, 0.5929503960351254)
(7, 0.5504226867087297)
(8, 0.4144661844198654)
(9, 0.2321121911618545)
(10, 0.7146040799038853)
(11, 1.8643450561903407)
(12, 1.9949341248458283)
(13, 1.1051515568205963)
(14, 2.022104902315551)
(15, 0.19450945506832673)
(16, -0.8462533768753627)
(17, 0.0336797121151123)
(18, 0.27744942568851)
(19, 0.8549021872445431)
(20, 0.5760996388106914)
(21, 0.9849174208827578)
(22, 0.7434164593641832)
(23, -0.10221220900390746)
(24, 1.084183571666092)
(25, 0.8713296390563305)
(26, 0.7700985431954361)
(27, -0.6879959029163099)
(28, -0.9323729960714642)
(29, -0.9132743468187794)
(30, -0.06059898810661141)
(31, -0.03805309445332633)
(32, 0.5670134838723505)
(33, 0.13764296696193629)
(34, 0.540843420489229)
(35, 0.5192890178770004)
(36, 0.45320677782934576)
(37, 0.5679857485244916)
(38, 0.6660687715853242)
(39, 0.6324853100126792)
(40, 0.6286093924746212)
(41, 0.5911333947429097)
(42, 0.5979881128580601)
(43, 0.5772894500246751)
(44, 0.5729745211154523)
(45, 0.6227638362369127)
(46, 0.6174433407497787)
(47, 0.62659706388732)
(48, 0.633842146053096)
(49, 0.6324040448699888)
(50, 0.6333060704301019)
}


\newcommand{\drawPixelTen}{%
(1, -1.8835710187401644)
(2, -1.0542970813120494)
(3, -1.2782680950723082)
(4, -1.4066017180236123)
(5, -2.1527923581904593)
(6, -0.6482974797344652)
(7, -0.634441010985429)
(8, -0.1854343158605733)
(9, 1.0503240066502548)
(10, 1.3301331498611209)
(11, 0.5398242403321672)
(12, 0.2973928924343318)
(13, -0.67957279100029)
(14, -0.504204255206728)
(15, -1.173665175285662)
(16, -1.2484120094915883)
(17, -0.9552517331721544)
(18, -0.5495243746446417)
(19, -0.3343050643433413)
(20, -0.36265513011557254)
(21, -0.8772350068982623)
(22, -0.04431845813835543)
(23, -0.7774102839233938)
(24, -0.21494635939211143)
(25, 0.6299955005741558)
(26, 0.7108176673776591)
(27, 0.7859796931604234)
(28, -0.029442673308738315)
(29, 0.26855513407993936)
(30, 0.12117564464983699)
(31, 0.6957485270074258)
(32, 0.5595470279433197)
(33, 0.34359576825690935)
(34, 0.04238371771595112)
(35, 0.2402769404240674)
(36, 0.04243002289513434)
(37, 0.18277039262276543)
(38, 0.1973003037876429)
(39, 0.25125005121398736)
(40, 0.3066022923688356)
(41, 0.2786631337639303)
(42, 0.3685689133729917)
(43, 0.34460613038998306)
(44, 0.33572439744210325)
(45, 0.3326288894764496)
(46, 0.34969136998848377)
(47, 0.3558786580279756)
(48, 0.3513697144834573)
(49, 0.3485270683661163)
(50, 0.3486730096009108)
}

==> data/drawPixel5_cifar.tex <==
\renewcommand{\drawPixelOne}{%
(1, 0.5453795355077534)
(2, 0.04732623838168354)
(3, -0.5394306511550303)
(4, -0.7585995574593323)
(5, -0.7130281103941979)
(6, 0.17751779251307)
(7, -0.10197530966972886)
(8, -0.04968946444495101)
(9, 2.2721868164943837)
(10, 2.181817691205217)
(11, 0.8537975447336498)
(12, 0.662267554532253)
(13, 2.7679309368174683)
(14, 2.7550163998714408)
(15, 2.2896522204044523)
(16, 0.8291086273760097)
(17, 1.2240749335579988)
(18, 0.7917735415892879)
(19, 0.16746486104712272)
(20, -0.4534112910789791)
(21, -0.588527547564166)
(22, 0.06019208192177844)
(23, -0.8093702977471942)
(24, -0.5204134282351714)
(25, -1.026818135756138)
(26, -1.0505899447645972)
(27, -1.5486262886828215)
(28, -0.675502207007054)
(29, -0.8293465706569574)
(30, -0.5019791571636046)
(31, -0.5349707755810867)
(32, -0.46631755577103856)
(33, -0.3264741716598213)
(34, -0.2777196106046633)
(35, -0.14530672461664643)
(36, 0.15931907744293866)
(37, 0.03532095979279477)
(38, 0.03243791330319172)
(39, 0.09688591351141093)
(40, 0.02159289350150906)
(41, 0.10514813788537289)
(42, 0.1417820022735098)
(43, 0.1109027276924476)
(44, 0.12090070593054704)
(45, 0.13351571725348862)
(46, 0.1306876997190387)
(47, 0.12694641115771452)
(48, 0.13040501757905795)
(49, 0.1304282959471608)
(50, 0.13419669879315674)
}

\renewcommand{\drawPixelTwo}{%
(1, -1.5023441087420688)
(2, -0.9401725422593681)
(3, 0.04984038778958257)
(4, 0.42498839761514356)
(5, -0.8689440505823424)
(6, 0.36401575431234506)
(7, 1.0312861942062772)
(8, 1.2738958609191011)
(9, 0.9091600002356202)
(10, 0.6304952978538167)
(11, -0.2031760313320354)
(12, 0.32399414100865753)
(13, -0.29145943611682823)
(14, -0.3488259999975604)
(15, -1.2839959868977324)
(16, -1.296318473511396)
(17, -0.5214962610449614)
(18, -0.23037828141248115)
(19, 0.036793615033515886)
(20, 0.6623686032873156)
(21, -0.14761835783015415)
(22, 0.39675608077218333)
(23, 0.7264779002288078)
(24, 1.088539831635936)
(25, 0.524775033277512)
(26, 1.414339946028313)
(27, 1.1969928631502607)
(28, 0.7309173430176384)
(29, 1.1827037281930672)
(30, 0.929145458795457)
(31, 1.100779844592154)
(32, 0.7695942753996445)
(33, 1.1405759531051443)
(34, 1.1497677699231723)
(35, 1.0273658944353468)
(36, 0.8841167999562386)
(37, 0.7725050212008946)
(38, 0.8507686636394843)
(39, 0.8293403011634186)
(40, 0.8423230589568791)
(41, 0.8851792167999595)
(42, 0.8231178515139239)
(43, 0.8008799289014191)
(44, 0.7985575746653922)
(45, 0.8061629192022728)
(46, 0.8396560516064432)
(47, 0.8394265853932295)
(48, 0.8376593534305262)
(49, 0.838296414362785)
(50, 0.8377774866298227)
}

\renewcommand{\drawPixelThree}{%
(1, -0.2582043378883868)
(2, 0.023315091200039537)
(3, 0.04518753692205774)
(4, -0.10151322413339474)
(5, -0.7785959859862008)
(6, -1.4102372123224702)
(7, -3.389854847587198)
(8, -2.8719028872145778)
(9, -0.944626185381142)
(10, 0.4204163164675052)
(11, 0.8463377400875729)
(12, 0.15992511154559375)
(13, 1.2105054078974211)
(14, 0.5206208831483174)
(15, -0.901713842789019)
(16, -1.3847311193567862)
(17, -0.8217166176679133)
(18, -0.09303624134085657)
(19, -0.7534650140339771)
(20, 0.1195063010562426)
(21, 0.6903566279506248)
(22, 0.16774836669319362)
(23, 0.2820387695639564)
(24, 0.05860507400160365)
(25, 0.21487144194222033)
(26, 0.863265536115057)
(27, 0.5443031244006155)
(28, -0.4092770379991376)
(29, -0.4126796097100083)
(30, -0.016477848288265647)
(31, -0.15307563557939707)
(32, 0.030402741325523352)
(33, -0.08166513525907841)
(34, -0.01715710989874663)
(35, 0.009777732797068527)
(36, 0.10858761492209285)
(37, 0.0037162363944098498)
(38, -0.010945024118865623)
(39, 0.03415819119442925)
(40, 0.02637940675302355)
(41, 0.10523992504909835)
(42, 0.02390546837347246)
(43, -0.020977343420126963)
(44, -0.06379001788429335)
(45, -0.07544434904552039)
(46, -0.08658670430487804)
(47, -0.07779858816110884)
(48, -0.0807718044843881)
(49, -0.07898977130553453)
(50, -0.07531316701975022)
}

\renewcommand{\drawPixelFour}{%
(1, 0.8581513732272521)
(2, 1.4621727799817057)
(3, 1.9516276777154993)
(4, 1.9462432178317486)
(5, 2.149176564652467)
(6, 1.6068591529976173)
(7, 1.982303428214013)
(8, 1.830901288520802)
(9, 0.0025453099643756314)
(10, -0.2356124914785114)
(11, 1.080590755496329)
(12, 1.7144843385202868)
(13, 1.9029080644940732)
(14, 1.280012409947014)
(15, 2.3908185178275616)
(16, 1.9188735288385632)
(17, 1.0171820175452635)
(18, 1.7078427880855442)
(19, 2.080722252496908)
(20, 2.353126007733399)
(21, 2.4035339386916506)
(22, 0.8974775097215314)
(23, 1.4776514631068034)
(24, 0.5617426539183574)
(25, 0.1555847467032209)
(26, -0.056050523007325215)
(27, 1.8009376153206402)
(28, 1.3386441178668913)
(29, 0.5346055815768042)
(30, 0.2827264741420976)
(31, 0.36935576157937156)
(32, -0.33700405239368747)
(33, 0.40301771344361625)
(34, 0.5370290129640991)
(35, 0.5553729885553911)
(36, 0.6655412729012214)
(37, 0.706573848363444)
(38, 0.8148662502128446)
(39, 0.916152561592921)
(40, 0.965542176675884)
(41, 0.9179702441884114)
(42, 0.9082253939030935)
(43, 0.9173629426913175)
(44, 0.8962152547183964)
(45, 0.8964423027263237)
(46, 0.8957934428360352)
(47, 0.892725083977914)
(48, 0.8892596549107564)
(49, 0.8861197906180063)
(50, 0.8871789105208661)
}

\renewcommand{\drawPixelFive}{%
(1, 0.10155879992494612)
(2, 1.1324279212315025)
(3, 0.5064418467445893)
(4, 1.4561114904247967)
(5, 0.46872927900767447)
(6, -0.8919237512339133)
(7, -0.9977307339923901)
(8, -0.8753425756253237)
(9, -0.378654625440467)
(10, 0.0616860412827)
(11, -0.8503679442365436)
(12, 1.077278630326103)
(13, 1.83772879237593)
(14, 2.2720746917981645)
(15, 1.7972409004767176)
(16, 0.5724898032724198)
(17, 0.3079551282961293)
(18, 1.4065551410645696)
(19, 2.0971013419443136)
(20, 0.3651581833766297)
(21, 0.9289946057858567)
(22, -0.09328117794668049)
(23, -0.857445022184765)
(24, -0.724508611614627)
(25, -0.5344231385216702)
(26, 0.12697275695102478)
(27, 0.6533377378515203)
(28, -0.13122316487876912)
(29, 0.086465886478933)
(30, 0.084491410019251)
(31, -0.6182576404526847)
(32, -0.17739080984006156)
(33, -0.38731275715227986)
(34, 0.0030496774254782366)
(35, 0.09770142686131046)
(36, -0.008784054137950442)
(37, 0.18016794541760536)
(38, 0.18821909401582992)
(39, 0.1365995725440075)
(40, 0.14049379746343632)
(41, 0.2008276171244709)
(42, 0.11440635591232047)
(43, 0.19082533487436565)
(44, 0.18237750899006966)
(45, 0.20254072769779874)
(46, 0.2172585355634164)
(47, 0.21618335847056042)
(48, 0.2226060681680453)
(49, 0.22112588063775335)
(50, 0.21603329289630746)
}

\renewcommand{\drawPixelSix}{%
(1, -0.9484394336161824)
(2, 1.046826223445921)
(3, 0.5895493521918345)
(4, -0.015833284230559425)
(5, 0.29114201039329823)
(6, -0.6547766747707258)
(7, -0.5678927124683248)
(8, 0.4512703757591358)
(9, -0.0254649807585523)
(10, -0.8213041459358631)
(11, -0.7421102068108383)
(12, -0.34591211346916406)
(13, 1.0235066345653194)
(14, 0.793550564127289)
(15, 1.1241376608517537)
(16, 0.7368845890421059)
(17, -0.4153121756075254)
(18, -1.0872525999485825)
(19, -0.952410315187515)
(20, -0.45602278427235554)
(21, -0.7051742743782976)
(22, -0.13567905830519464)
(23, -1.1966894522520115)
(24, -1.2505118757102118)
(25, -1.7108277611997948)
(26, -1.67427225434376)
(27, 0.5005373165565581)
(28, 0.6143147023050457)
(29, 0.8293385675496935)
(30, 1.1543910869808198)
(31, 1.0820692544965616)
(32, 0.38469424050513956)
(33, 0.588378580986247)
(34, 0.6875931327062379)
(35, 0.888621437035911)
(36, 1.036962844783836)
(37, 1.076959984064258)
(38, 1.0176555825005462)
(39, 0.8469392779531008)
(40, 0.9702328836332633)
(41, 0.8624918144773941)
(42, 0.9499347668709898)
(43, 0.9699475613356896)
(44, 0.9470913311476682)
(45, 0.9246400667387166)
(46, 0.935924547123647)
(47, 0.9335498923186389)
(48, 0.9252552781840888)
(49, 0.9182919951835834)
(50, 0.9218811855516607)
}

\renewcommand{\drawPixelSeven}{%
(1, 0.25207635256479627)
(2, 0.8004387465380393)
(3, -0.6347083166961816)
(4, 0.5681493991880807)
(5, 1.221749542527912)
(6, 1.3302546858670066)
(7, -0.03853167905716258)
(8, 0.29712017791211554)
(9, 0.8401327120978912)
(10, 1.8864373912134034)
(11, 2.3989443711547644)
(12, 1.5203745598595562)
(13, 2.0959432723195683)
(14, 1.543384571908662)
(15, 1.536221337855058)
(16, 1.1203454660352807)
(17, 1.226699623111741)
(18, 1.3773976990768786)
(19, 1.4826621921552865)
(20, 1.5403641491627598)
(21, 2.153852624333857)
(22, 1.5780394778785274)
(23, 1.3597125375551127)
(24, 1.679193217024795)
(25, 2.203756704525476)
(26, 1.993072587871041)
(27, 1.9260583310703772)
(28, 1.2806377998730103)
(29, 0.4557616574784533)
(30, 1.3768449208960094)
(31, 1.2028871858539285)
(32, 0.9189665324701279)
(33, 0.6671047489332173)
(34, 0.5341528208028044)
(35, 0.9839261560216722)
(36, 0.8588280061425348)
(37, 1.113273705971015)
(38, 1.1181283326367313)
(39, 1.1215636302698426)
(40, 1.0128003669024117)
(41, 0.9946535429520938)
(42, 0.9996884405213226)
(43, 1.0266491380836338)
(44, 1.025572404681635)
(45, 1.0154901812882675)
(46, 1.0163452383482863)
(47, 1.0130335909525545)
(48, 1.0064821787227036)
(49, 1.0065590224201286)
(50, 1.000095532160556)
}

\renewcommand{\drawPixelEight}{%
(1, 1.060279316171447)
(2, 0.6185500676838117)
(3, -0.3201181886320799)
(4, -1.0345984213178852)
(5, -0.059665027740793054)
(6, 1.1397399724870836)
(7, 1.5256019437607866)
(8, 0.7448954307894718)
(9, 0.41311815043316574)
(10, 0.03135305014348436)
(11, 0.48484990277553863)
(12, 0.48225064979546833)
(13, 0.6116990608828579)
(14, 1.4097162080648618)
(15, 1.1682812632200692)
(16, 0.7184192860264996)
(17, 0.9100003198601726)
(18, 0.860015021412416)
(19, 2.359556206775639)
(20, 1.3676844302450109)
(21, 0.9643180237525466)
(22, 0.6896212333671018)
(23, -0.3146686636704255)
(24, 0.04832164874514143)
(25, 0.15869010350931573)
(26, 0.7852776787536871)
(27, 0.8126948510024057)
(28, 0.783395795980681)
(29, 0.3361721311760595)
(30, 0.5522360593970757)
(31, 1.2506276749145446)
(32, 0.8553144929882597)
(33, 0.1740938388461668)
(34, 0.10314219926706578)
(35, 0.4887090649498562)
(36, 0.509545219784637)
(37, 0.5837885673731966)
(38, 0.495197247852257)
(39, 0.49504251364505464)
(40, 0.5303278764730904)
(41, 0.5272810161754289)
(42, 0.521652678575269)
(43, 0.5085198608132303)
(44, 0.5164287476592161)
(45, 0.5066869435660738)
(46, 0.5000803109328877)
(47, 0.4930764610223152)
(48, 0.48689252204640215)
(49, 0.4893560552139231)
(50, 0.48960890070932644)
}

\renewcommand{\drawPixelNine}{%
(1, 0.2019136085412942)
(2, -0.6361742235104109)
(3, 0.5368688949943118)
(4, 0.6607879258368946)
(5, 0.09715253528303229)
(6, 0.3338431084313745)
(7, 0.16087899820116558)
(8, -0.06469909963389033)
(9, 0.5422271742441633)
(10, 1.1378574060022573)
(11, 1.2921214247815813)
(12, 1.4793790546912327)
(13, 1.9804192822811508)
(14, 1.5842271496154654)
(15, 2.2149854727242113)
(16, 0.9920027842794888)
(17, 0.8392687270048172)
(18, 0.32556856953110663)
(19, 0.7410062774105497)
(20, 0.26118242541206727)
(21, -0.47637340369379877)
(22, -0.6437142359323328)
(23, -0.13471401620836457)
(24, -0.6100890484187297)
(25, 0.13497293713198877)
(26, 1.0420562723343394)
(27, 0.5360323396981234)
(28, 0.4298275927367601)
(29, -0.323380464643004)
(30, -0.0987155249836944)
(31, 0.7848293847264235)
(32, 0.45014123642217585)
(33, 1.2361917805192233)
(34, 1.0413650181419343)
(35, 0.6616920343799813)
(36, 0.6276837655252949)
(37, 0.9344707325422666)
(38, 0.733498789720574)
(39, 0.6882651960946025)
(40, 0.6528878901271564)
(41, 0.7282597628304117)
(42, 0.7662177639182026)
(43, 0.785737165003388)
(44, 0.769360618072071)
(45, 0.7647666830125027)
(46, 0.7754848032587139)
(47, 0.7705759813417221)
(48, 0.7677132442268765)
(49, 0.7676167148429142)
(50, 0.769222053748931)
}

\renewcommand{\drawPixelTen}{%
(1, -0.5456824705759946)
(2, -1.1798050623358858)
(3, -1.7327885187362793)
(4, -2.1603350966739354)
(5, -1.5689697859368246)
(6, -0.6158306716956586)
(7, -0.09652912475477779)
(8, 0.3880771982024988)
(9, 1.2616952418270502)
(10, 1.1203696708271689)
(11, 0.8829668887959453)
(12, -0.3998943542742632)
(13, -1.3201072426452294)
(14, -0.3334428723212751)
(15, 0.023174924637886465)
(16, -0.6219710578723852)
(17, -0.3218666948003751)
(18, 0.29440562778054363)
(19, 0.3716298118054733)
(20, 0.5534695598007674)
(21, 0.551082852000223)
(22, 1.8164078375239232)
(23, 2.3774600225716815)
(24, 1.5375321064740715)
(25, 0.4167041131506467)
(26, 0.9282603887704309)
(27, 0.6281562437158721)
(28, 1.5215324036731874)
(29, 0.2995023604131939)
(30, 0.40529548346395117)
(31, 1.1080637238230349)
(32, 1.0856995842543895)
(33, 0.929773096513287)
(34, 0.8938023807176044)
(35, 0.9682080536353646)
(36, 0.8770137252462384)
(37, 0.8312928367923857)
(38, 0.8124990596789866)
(39, 0.8865862263118799)
(40, 0.8809087777283309)
(41, 0.8854512057677687)
(42, 0.8989452450467075)
(43, 0.9281115474260473)
(44, 0.9055415133980251)
(45, 0.885969757328474)
(46, 0.9018352705142212)
(47, 0.8999339811594598)
(48, 0.8974285002174138)
(49, 0.895310552990567)
(50, 0.8929448631511194)
}

==> data/drawPixel6.tex <==
\newcommand{\drawPixelOne}{%
(1, -56.33381608238145)
(2, -5.987971101590784)
(3, -5.88409578638154)
(4, 35.503296314699384)
(5, 26.57744645220141)
(6, -19.994735023029996)
(7, 8.692686568705714)
(8, 26.624323763812157)
(9, 37.06909729302212)
(10, 56.54610951931755)
(11, 44.18839575717212)
(12, 18.046055302169293)
(13, 33.63224155719192)
(14, 28.390356101462)
(15, 26.722667448934384)
(16, 24.007563556427243)
(17, 16.219789645029195)
(18, 5.933427430798397)
(19, -1.8954229287702673)
(20, -0.7527933073166402)
(21, -1.330566480640337)
(22, 1.036572262115013)
(23, 3.024670300896005)
(24, -1.908543575863207)
(25, -0.226866164571921)
(26, -0.2712588850198778)
(27, -2.0995787012400893)
(28, -1.189486762426164)
(29, -1.3049760754775126)
(30, -0.0685798526426154)
(31, -0.06351764050139769)
(32, -0.41386496760137537)
(33, -0.058038742200773596)
(34, -0.37780805450842564)
(35, -0.7115668610224206)
(36, -0.521701969363964)
(37, -0.6155127800536024)
(38, -0.5730218765776607)
(39, -0.7715159743942722)
(40, -0.8194535925591605)
(41, -0.9160776588804838)
(42, -0.86212153447864)
(43, -0.8407571749072157)
(44, -0.8672956731460875)
(45, -0.8396676898727728)
(46, -0.8423077216025652)
(47, -0.8418682379736678)
(48, -0.8285317953119621)
(49, -0.8264158440942451)
(50, -0.8262056708335876)
}


\newcommand{\drawPixelTwo}{%
(1, 50.249761889484375)
(2, 121.56603421324759)
(3, 53.29291701532428)
(4, 55.9584839505791)
(5, 10.342472013133209)
(6, 28.851292728574936)
(7, -22.263518613963637)
(8, -22.399234196719092)
(9, -20.764406811747296)
(10, -12.720309823197242)
(11, -14.814129447280559)
(12, -16.222154375057922)
(13, -11.705214582527105)
(14, -19.88778941336198)
(15, -8.251964713576852)
(16, -9.62101234840643)
(17, -15.103009296678525)
(18, -12.132338729481368)
(19, -6.601863207621733)
(20, -5.048029585638281)
(21, -8.199285238236959)
(22, -6.537418269447894)
(23, 0.9041380430612831)
(24, 0.6734601611218313)
(25, -0.5378312789650206)
(26, 1.0819221424975198)
(27, 0.6615141810434095)
(28, 2.8682853542045006)
(29, 0.028379171077110132)
(30, -0.5235968895151274)
(31, -0.0819808232234367)
(32, 0.6093872477128451)
(33, 0.8316254703161676)
(34, 0.5315735018339269)
(35, 0.600641066536002)
(36, 0.47128399243009905)
(37, 0.4986644214019638)
(38, 0.54228358251198)
(39, 0.5213902589184357)
(40, 0.5633626256407209)
(41, 0.5675916713331425)
(42, 0.5394175114221395)
(43, 0.4792539471621735)
(44, 0.5009143400147928)
(45, 0.5162273685530318)
(46, 0.5238422944006196)
(47, 0.5293845711925549)
(48, 0.5269726305900382)
(49, 0.5269217971510933)
(50, 0.5244174003601074)
}


\newcommand{\drawPixelThree}{%
(1, 87.99043227254853)
(2, 1.05887790673748)
(3, 12.76500048263859)
(4, 21.800681105145504)
(5, 16.613893742203647)
(6, 34.55750793217344)
(7, 33.01951151636897)
(8, -9.967774369383648)
(9, 36.22375254508165)
(10, 21.673127542610544)
(11, 4.358951414286652)
(12, 6.411809604980904)
(13, 14.158314173341214)
(14, 32.0140040216264)
(15, 23.27199011519827)
(16, 20.631543392378724)
(17, 3.272275552355683)
(18, -6.689696211688328)
(19, -0.9600588252762109)
(20, 2.7330681172045805)
(21, -6.1769644082369695)
(22, -2.433035828637788)
(23, -6.338325311028405)
(24, -7.330357950843061)
(25, -2.6158271686724937)
(26, -0.9525543755165268)
(27, -0.8119953163403331)
(28, -0.8374593562221143)
(29, -0.562977414094963)
(30, -0.610780002386098)
(31, -0.7693273808696145)
(32, -1.022512428604337)
(33, -0.9488198921382158)
(34, -1.0103634886325283)
(35, -1.3646936974013981)
(36, -1.1063731028491122)
(37, -1.012064777035824)
(38, -1.0268207337778414)
(39, -0.8569814304269228)
(40, -0.9665306205588922)
(41, -0.9800994377769391)
(42, -0.9818054539378821)
(43, -0.9753979062161835)
(44, -0.9989354027453903)
(45, -1.0023019688212773)
(46, -0.9930329171043861)
(47, -0.9814542547354113)
(48, -0.9725217809120279)
(49, -0.9706924675194729)
(50, -0.973031520843506)
}


\newcommand{\drawPixelFour}{%
(1, 6.734588299140873)
(2, -1.7998520830911415)
(3, -25.83870391695467)
(4, -3.176856673494472)
(5, 14.755091562726864)
(6, -8.781379613318713)
(7, -31.440781388393457)
(8, 13.679449801319183)
(9, 41.16795164517329)
(10, 20.956687514251026)
(11, 2.7919753861690078)
(12, 1.693858828426921)
(13, 11.263112204528305)
(14, 18.789411779403935)
(15, 4.783143520484453)
(16, 9.693807827996675)
(17, 5.711479362262763)
(18, 0.5432626506043667)
(19, 4.793928341183692)
(20, -5.122374574881553)
(21, 0.4823521336718856)
(22, 5.600454633409016)
(23, 7.377029522320039)
(24, 4.616230092350445)
(25, 3.4728662391316574)
(26, 2.8957753239211343)
(27, 0.874686655977462)
(28, -1.7411646088788073)
(29, -1.1510570453638085)
(30, -0.0882644674857262)
(31, 0.0015315511658026693)
(32, 0.022908981543456053)
(33, 0.35207540421783284)
(34, 0.14360274913871518)
(35, 0.38184024451438997)
(36, 0.27738156212627163)
(37, 0.22490716845276876)
(38, 0.2815886191350244)
(39, 0.33001691978141845)
(40, 0.4038025312137721)
(41, 0.4343960013302578)
(42, 0.4308053975651516)
(43, 0.45567341780654985)
(44, 0.4608740182888878)
(45, 0.4459545432044264)
(46, 0.42444736725336907)
(47, 0.42165206099461117)
(48, 0.4147652123859836)
(49, 0.4160279072092952)
(50, 0.41466125845909124)
}


\newcommand{\drawPixelFive}{%
(1, -2.4395647210755733)
(2, -52.01094384579315)
(3, -26.10205151731793)
(4, -37.91004483878797)
(5, -24.392461036107534)
(6, -40.99435512437242)
(7, -21.1554807223317)
(8, -32.08532642117369)
(9, -16.35601970117638)
(10, 18.356986983786125)
(11, 37.029536547749494)
(12, 36.95812406608164)
(13, 17.65709181297388)
(14, 19.33006353710227)
(15, 12.377562262506384)
(16, 7.85745763163346)
(17, -2.09748554705589)
(18, 6.354551076827)
(19, 6.620977723736895)
(20, -1.9069627274675356)
(21, -1.0137028388144695)
(22, -8.64624653814329)
(23, -4.433078485125661)
(24, -3.2945283302180197)
(25, -2.5663324229936015)
(26, -0.894337343314544)
(27, -0.4769358172653415)
(28, -0.6296323009303807)
(29, -0.8870125947344867)
(30, -0.20575608861555617)
(31, 0.21046275389731522)
(32, 0.42400969659329696)
(33, 0.9310704437108742)
(34, 0.5326850114121741)
(35, 0.13563248743970718)
(36, 0.48495004684803145)
(37, 0.38942725080868984)
(38, 0.488296499686437)
(39, 0.3861351757171347)
(40, 0.4995272957649226)
(41, 0.5196900668906962)
(42, 0.4867076149933207)
(43, 0.4951475547897191)
(44, 0.49132232413178867)
(45, 0.490428935248235)
(46, 0.4941852699745411)
(47, 0.48763303465413926)
(48, 0.48431682009851856)
(49, 0.47932293006344645)
(50, 0.47954279184341425)
}


\newcommand{\drawPixelSix}{%
(1, 64.3031396677126)
(2, 44.534844053171845)
(3, 20.28384579222756)
(4, -11.278003889988014)
(5, -1.9793723842442819)
(6, -22.91281254102114)
(7, -13.597052057211606)
(8, 7.187331889381938)
(9, -3.71263189879002)
(10, -33.04577780470041)
(11, -4.4749648369762625)
(12, 16.40821285195772)
(13, 19.12384606670387)
(14, 7.906828166072738)
(15, 4.193715444343188)
(16, -3.163834142683588)
(17, -10.47191928541259)
(18, -6.716612471826471)
(19, -9.971823297399672)
(20, -5.637598100777739)
(21, 0.6936283956689506)
(22, 0.38123989443323714)
(23, 3.1858179501607764)
(24, 1.5018908773047317)
(25, 1.8454891522985029)
(26, 2.9597495556331106)
(27, 2.9587796661605843)
(28, -0.8868829581228173)
(29, -0.8874841845878316)
(30, -0.21615050380260892)
(31, -0.5939264538878553)
(32, -0.3078732374524503)
(33, -0.09171427811171146)
(34, 0.3160086714563475)
(35, 1.0226036401931813)
(36, 0.8182411888535778)
(37, 0.7171347758017771)
(38, 0.5411595714621236)
(39, 0.5754154707277747)
(40, 0.5291504210817737)
(41, 0.5184965984502331)
(42, 0.5033854003522801)
(43, 0.4993904032521884)
(44, 0.529726276701004)
(45, 0.5182500642617666)
(46, 0.5149722622194716)
(47, 0.5148439161032448)
(48, 0.5133501343595862)
(49, 0.5156013573333624)
(50, 0.5139058232307434)
}


\newcommand{\drawPixelSeven}{%
(1, 27.881429957496508)
(2, 76.46951157490881)
(3, 42.40164206327559)
(4, -19.60229245803997)
(5, -47.668418324373775)
(6, -22.769748432485866)
(7, -47.11654534658635)
(8, -34.397819393798784)
(9, -45.017746142618755)
(10, -48.84682495125273)
(11, -36.20012109545236)
(12, -26.918148952433874)
(13, -45.31596955116355)
(14, -10.914886847910005)
(15, -10.960693090462257)
(16, -2.904243638063748)
(17, 1.488145411631833)
(18, -4.235922282565637)
(19, -9.107487326718747)
(20, -1.9009120464405296)
(21, 4.718471438651503)
(22, 3.7862362366560443)
(23, 3.5858048770786835)
(24, 1.2454768660177267)
(25, -0.13377376783486616)
(26, 0.9837106649752574)
(27, 2.131308083614289)
(28, 2.733312692266195)
(29, 2.8706832245187797)
(30, 2.000622120086905)
(31, 1.9067663665234884)
(32, 1.1123279110910924)
(33, 1.4421743339580457)
(34, 1.1595175623027498)
(35, 0.6182467959822617)
(36, 1.0124478165418735)
(37, 0.7807651407366243)
(38, 0.5834663247208063)
(39, 0.5678914318020389)
(40, 0.5579040846961749)
(41, 0.5422264225124989)
(42, 0.6047586337780305)
(43, 0.5863779199967136)
(44, 0.5919154200090827)
(45, 0.5758013347377834)
(46, 0.5736893852271423)
(47, 0.5681653995447087)
(48, 0.5552022337749901)
(49, 0.5582313034663384)
(50, 0.5568881630897522)
}


\newcommand{\drawPixelEight}{%
(1, -74.20066834384603)
(2, -32.280565946178754)
(3, -73.0174977792336)
(4, -82.09147679197235)
(5, -50.44443925767319)
(6, -66.1657093869309)
(7, -71.44712194713689)
(8, -39.74845074722655)
(9, -34.77715137885859)
(10, 8.24946719546487)
(11, 6.162282066311613)
(12, -1.8362091616183764)
(13, -9.41188229123108)
(14, -19.565579590514407)
(15, -12.644050822416983)
(16, -16.005251085055164)
(17, -20.562685880700457)
(18, -12.699180988581382)
(19, -3.848743346520619)
(20, 0.4577378781237058)
(21, -0.2336128528378083)
(22, -2.0641977832574083)
(23, -1.955497236497254)
(24, 0.3259238171547225)
(25, -0.05037585658001659)
(26, 0.25322340190846526)
(27, 1.112526573061967)
(28, 0.3258973460602218)
(29, 0.7264841942114916)
(30, 0.9016457041266431)
(31, 0.339069846337811)
(32, 1.2628503807752165)
(33, 0.4056791961729937)
(34, 0.13553118071750697)
(35, 0.35413457753557026)
(36, 0.6536475611902246)
(37, 0.6916870011080719)
(38, 0.5431474253451523)
(39, 0.67476949921917)
(40, 0.5790197971543668)
(41, 0.6171263883793205)
(42, 0.5867401917799346)
(43, 0.6282308283362599)
(44, 0.593569561104928)
(45, 0.5944898099778247)
(46, 0.6075490786930559)
(47, 0.6065236393408285)
(48, 0.5936798181612657)
(49, 0.5898154667946757)
(50, 0.5927229523658752)
}


\newcommand{\drawPixelNine}{%
(1, 10.11287662277065)
(2, 19.77670720977325)
(3, -41.16396951910877)
(4, -36.84020395376676)
(5, -34.96042820818486)
(6, 23.500708611474927)
(7, 19.271800435724867)
(8, 12.790453673496009)
(9, 6.307943573160202)
(10, 17.009833352449803)
(11, 38.821391543003166)
(12, 36.258990803960515)
(13, 17.48949172179433)
(14, 27.778442469726233)
(15, 2.3292309472999717)
(16, -8.664490167007635)
(17, 0.33161006152308464)
(18, 2.1552571091574375)
(19, 5.614166012648939)
(20, 3.2601173771315257)
(21, 4.738129825456019)
(22, 3.068345438020485)
(23, -0.2876506859495726)
(24, 3.242050540700809)
(25, 2.2458713547729277)
(26, 1.7264011520473892)
(27, -1.2127592846809792)
(28, -1.4541494370902333)
(29, -1.2472757849667844)
(30, 0.0038782265942213234)
(31, 0.043280634555391106)
(32, 0.7421903567793735)
(33, 0.260541766258495)
(34, 0.6673408878282042)
(35, 0.6121448488299377)
(36, 0.5241241624389109)
(37, 0.6135340021092944)
(38, 0.6930904739518496)
(39, 0.6411867645083098)
(40, 0.6252630215770921)
(41, 0.5790354129660557)
(42, 0.5733147516100113)
(43, 0.5462194006498152)
(44, 0.5399071660660207)
(45, 0.581927611441407)
(46, 0.5739114798403093)
(47, 0.5806118003073516)
(48, 0.5863699943351314)
(49, 0.5844031087187664)
(50, 0.5850223302841187)
}


\newcommand{\drawPixelTen}{%
(1, -134.69490859121277)
(2, -67.26665766665819)
(3, -72.62498753820648)
(4, -71.02637517157068)
(5, -96.41047279411387)
(6, -25.70261142422187)
(7, -22.21045272225109)
(8, -5.717286141455264)
(9, 28.50408550216331)
(10, 31.658094436893624)
(11, 11.24850079192539)
(12, 5.4137335288249435)
(13, -10.741375021479861)
(14, -6.910197197157307)
(15, -13.934630510828205)
(16, -12.787506510915774)
(17, -8.41192186970055)
(18, -4.12644659733262)
(19, -2.1257992389578924)
(20, -1.9635307202373413)
(21, -4.119531699481058)
(22, -0.13389698570940706)
(23, -2.6353283619195853)
(24, -0.578226123593305)
(25, 1.6367961018579855)
(26, 1.5974063175742181)
(27, 1.546473830809993)
(28, 0.03665038641393786)
(29, 0.48504981536757674)
(30, 0.2668420740777247)
(31, 0.9513613587796832)
(32, 0.7602208172618242)
(33, 0.5068115928156379)
(34, 0.20207177864756865)
(35, 0.4190525247461887)
(36, 0.22849106295190824)
(37, 0.37135840921930097)
(38, 0.3791958415415533)
(39, 0.4218305495772015)
(40, 0.4743990868129461)
(41, 0.45770025014855914)
(42, 0.5440911260481004)
(43, 0.5225597930733331)
(44, 0.5194540217814038)
(45, 0.5197596984080882)
(46, 0.5371743591900207)
(47, 0.5421036486579648)
(48, 0.5378838462879432)
(49, 0.5355725347790314)
(50, 0.5360975861549377)
}

==> data/drawPixel6_cifar.tex <==
\renewcommand{\drawPixelOne}{%
(1, 38.99025638685403)
(2, 3.0077705949702533)
(3, -30.65296219645004)
(4, -38.303150114960644)
(5, -31.932443800853058)
(6, 7.037851062030207)
(7, -3.562599052287096)
(8, -1.5240242846682746)
(9, 61.63512160768617)
(10, 51.91411628395153)
(11, 17.78012922244433)
(12, 12.037422695347114)
(13, 43.79124003156964)
(14, 37.84220053803121)
(15, 27.236221635402064)
(16, 8.522509095726779)
(17, 10.831627459641119)
(18, 6.012513306013165)
(19, 1.0864213168098256)
(20, -2.5335879679728266)
(21, -2.812615215811702)
(22, 0.21736479294475664)
(23, -2.8204784963772314)
(24, -1.570864876122549)
(25, -2.618177359022587)
(26, -2.295463931249862)
(27, -2.935096367823213)
(28, -1.1512091427057842)
(29, -1.249324531753238)
(30, -0.7026778075665235)
(31, -0.6907484160818432)
(32, -0.5668095143056449)
(33, -0.38385793764266085)
(34, -0.31508663067659726)
(35, -0.1666799676165911)
(36, 0.15249463403404523)
(37, 0.028936453593296635)
(38, 0.028017523292943755)
(39, 0.0940786827491337)
(40, 0.019152597808107366)
(41, 0.1020522401759246)
(42, 0.13938094909035179)
(43, 0.10888938944405055)
(44, 0.11897560920629813)
(45, 0.13185653499759417)
(46, 0.12855761554033818)
(47, 0.12435983771571874)
(48, 0.12756950581398738)
(49, 0.1273003859177966)
(50, 0.1302463263273239)
}

\renewcommand{\drawPixelTwo}{%
(1, -107.43096764501767)
(2, -59.97929574253647)
(3, 2.8240863534371234)
(4, 21.443636328181007)
(5, -38.92573579545478)
(6, 14.413584602735378)
(7, 36.088418241488625)
(8, 39.29140291844661)
(9, 24.662022745906405)
(10, 15.007983175044982)
(11, -4.223502982600687)
(12, 5.899705497174583)
(13, -4.595095823994916)
(14, -4.774436425020652)
(15, -15.253437308974943)
(16, -13.29407346496512)
(17, -4.586123239680372)
(18, -1.7159848936310582)
(19, 0.27173422685239523)
(20, 3.7222992923758635)
(21, -0.6639412279329472)
(22, 1.6543519875375026)
(23, 2.568533557970005)
(24, 3.272901042184677)
(25, 1.3985723565766044)
(26, 3.135219859190512)
(27, 2.3023863187677174)
(28, 1.266168113331506)
(29, 1.7921009808312824)
(30, 1.3139622782266709)
(31, 1.4285203500390415)
(32, 0.9627401564333837)
(33, 1.3330624899945192)
(34, 1.300034945113296)
(35, 1.1422383555738578)
(36, 0.9763526563313526)
(37, 0.849603123101046)
(38, 0.9187430654225817)
(39, 0.895067807890156)
(40, 0.9072579571464303)
(41, 0.9473000486474374)
(42, 0.884766437243299)
(43, 0.8639771004232087)
(44, 0.862978562051734)
(45, 0.8698932013429213)
(46, 0.8967055497760364)
(47, 0.8911727286066794)
(48, 0.886815351747344)
(49, 0.8855161349447329)
(50, 0.8828494548797607)
}

\renewcommand{\drawPixelThree}{%
(1, -18.464872559837)
(2, 1.4867669488064865)
(3, 2.56586459098068)
(4, -5.121414251841912)
(5, -34.86325328450586)
(6, -55.89129731674363)
(7, -118.64957862356671)
(8, -88.58201131978089)
(9, -25.61192309494536)
(10, 10.013247774786167)
(11, 17.62908028468558)
(12, 2.913401765254669)
(13, 19.15765844850529)
(14, 7.154362125088841)
(15, -10.721556500747484)
(16, -14.219009722372261)
(17, -7.2711250055695995)
(18, -0.7121209131487567)
(19, -4.915601306553434)
(20, 0.649592237305836)
(21, 3.2584696406352798)
(22, 0.6661475216450375)
(23, 0.9547344281978383)
(24, 0.14308348080004346)
(25, 0.5104673770623863)
(26, 1.8388293149887012)
(27, 1.001417469585447)
(28, -0.6921321392293106)
(29, -0.6325019940479644)
(30, -0.056271176958620446)
(31, -0.21577946263625158)
(32, 0.009943644632361415)
(33, -0.11226109246334043)
(34, -0.038024579094073654)
(35, -0.006327931655552843)
(36, 0.09856719392220958)
(37, -0.008337780147209296)
(38, -0.023646133588194493)
(39, 0.021157264624704058)
(40, 0.014237333784022439)
(41, 0.09141328428459974)
(42, 0.007287734712560945)
(43, -0.03878355589338825)
(44, -0.08189078505086313)
(45, -0.09297177236626995)
(46, -0.10351368239060378)
(47, -0.09489605356245348)
(48, -0.0976906534613982)
(49, -0.09582522119384006)
(50, -0.092554472386837)
}

\renewcommand{\drawPixelFour}{%
(1, 61.35880018453129)
(2, 93.25992694798114)
(3, 110.84823444681308)
(4, 98.24219563945124)
(5, 96.21896244311108)
(6, 63.67035285068024)
(7, 69.38347129819283)
(8, 56.484666056437476)
(9, 0.07322140082461336)
(10, -5.597903928397812)
(11, 22.507083480948758)
(12, 31.16788360151654)
(13, 30.1208157221717)
(14, 17.603468716985613)
(15, 28.468319523374976)
(16, 19.75063018622046)
(17, 9.044782300445398)
(18, 13.027478143254665)
(19, 13.599498114864911)
(20, 13.148088061594944)
(21, 11.46896795590984)
(22, 3.691209796248815)
(23, 5.155082349015299)
(24, 1.7160058702819903)
(25, 0.4609081387195362)
(26, -0.04494434110361434)
(27, 3.4223169044620922)
(28, 2.246727672155618)
(29, 0.8316180380423158)
(30, 0.4287929400800049)
(31, 0.504672336504537)
(32, -0.34210918571325444)
(33, 0.4804804859970109)
(34, 0.6163255715031677)
(35, 0.6313531979374138)
(36, 0.7403933738884082)
(37, 0.7743452308939693)
(38, 0.8790811414052796)
(39, 0.9784528933983222)
(40, 1.0260022938712021)
(41, 0.9766822120761817)
(42, 0.9659180399791163)
(43, 0.9746107691022767)
(44, 0.9519252180083315)
(45, 0.9513878062089873)
(46, 0.9500793518879441)
(47, 0.9456669052892099)
(48, 0.9414545449563223)
(49, 0.9386100916356156)
(50, 0.9398468732833863)
}

\renewcommand{\drawPixelFive}{%
(1, 7.250285293435402)
(2, 72.23350921949029)
(3, 28.75968439640691)
(4, 73.5086712546138)
(5, 20.981123375544335)
(6, -35.36495871759214)
(7, -34.933534408385654)
(8, -27.00553752443262)
(9, -10.267458971067548)
(10, 1.4728749640806935)
(11, -17.702404149685734)
(12, 19.575084316216817)
(13, 29.07353561219473)
(14, 31.20752604478852)
(15, 21.37543933065021)
(16, 5.882302095640657)
(17, 2.731128771664565)
(18, 10.698399426448056)
(19, 13.662875957562106)
(20, 2.0420379152545043)
(21, 4.411230437542658)
(22, -0.38293926584473303)
(23, -2.9665437369871404)
(24, -2.136849895086202)
(25, -1.3638684050906695)
(26, 0.26380983355564064)
(27, 1.2300599312198188)
(28, -0.22074925326096106)
(29, 0.11670879537828367)
(30, 0.10210803641555333)
(31, -0.7505366863079811)
(32, -0.20343927261320677)
(33, -0.4268116737499879)
(34, 0.011193109774249504)
(35, 0.11592419044546025)
(36, 0.007331138325955833)
(37, 0.1969041687751294)
(38, 0.20315785882383247)
(39, 0.15165003058023227)
(40, 0.15734804034410302)
(41, 0.21703748321776953)
(42, 0.12766664568390493)
(43, 0.20403528767556647)
(44, 0.19398643101529367)
(45, 0.21359716091920275)
(46, 0.2273618704196368)
(47, 0.22539437188460185)
(48, 0.23126006776161562)
(49, 0.22974321963134312)
(50, 0.22535714507102966)
}

\renewcommand{\drawPixelSix}{%
(1, -67.82283217040245)
(2, 66.77935436093497)
(3, 33.48713144258133)
(4, -0.8059052899505207)
(5, 13.03068232613359)
(6, -25.957913021049094)
(7, -19.880217832556202)
(8, 13.928895572012928)
(9, -0.6787207380991193)
(10, -19.52770534365885)
(11, -15.437991001033042)
(12, -6.270586051002959)
(13, 16.213532909078122)
(14, 10.93059098557113)
(15, 13.408648436276906)
(16, 7.612026851810067)
(17, -3.627334730868335)
(18, -8.209776021620169)
(19, -6.145793496845557)
(20, -2.4768369025950903)
(21, -3.2872729573561066)
(22, -0.5122774151443448)
(23, -4.106977130839576)
(24, -3.6625150894074787)
(25, -4.2998383746842475)
(26, -3.6011312938803655)
(27, 0.9430978885033209)
(28, 1.020059348884827)
(29, 1.2359126662228366)
(30, 1.5641198597584525)
(31, 1.3623696505267664)
(32, 0.4854672214214053)
(33, 0.6893866119031813)
(34, 0.7801246609290661)
(35, 0.9776223661213639)
(36, 1.1146038825424627)
(37, 1.1462344750273508)
(38, 1.0787842831538563)
(39, 0.9045234087809721)
(40, 1.030851580111331)
(41, 0.9319186099336189)
(42, 1.0155845467460107)
(43, 1.0333212476680667)
(44, 1.0117496593627862)
(45, 0.9882323070142337)
(46, 0.9979099534396768)
(47, 0.9938150461510051)
(48, 0.9869005944947894)
(49, 0.9816455913138146)
(50, 0.986658275127411)
}

\renewcommand{\drawPixelSeven}{%
(1, 18.02518174944638)
(2, 51.062527207593874)
(3, -36.05825590500052)
(4, 28.686500456206314)
(5, 54.70794091986613)
(6, 52.720688917537316)
(7, -1.3474951049621522)
(8, 9.171273615531703)
(9, 22.79431112287247)
(10, 44.88957612192418)
(11, 49.94860188212488)
(12, 27.63693977232173)
(13, 33.17618295692102)
(14, 21.22823224622877)
(15, 18.306353856466714)
(16, 11.547168629492944)
(17, 10.895892090915918)
(18, 10.51411921983813)
(19, 9.703508041270027)
(20, 8.627961095769187)
(21, 10.292789953771749)
(22, 6.449788223274989)
(23, 4.755767008510373)
(24, 4.994139664938069)
(25, 5.604632387147587)
(26, 4.372472561506124)
(27, 3.6627583473491256)
(28, 2.152262578459041)
(29, 0.7130231824717143)
(30, 1.868511818588337)
(31, 1.5169261477801148)
(32, 1.1047433122054229)
(33, 0.7802182432060463)
(34, 0.6135099597295028)
(35, 1.0732333153058495)
(36, 0.9345907296953729)
(37, 1.179801063951834)
(38, 1.1713963759390937)
(39, 1.1566160849779654)
(40, 1.0400525728912586)
(41, 1.016052184982336)
(42, 1.016421311739959)
(43, 1.0379310071690386)
(44, 1.0330538643032157)
(45, 1.0205705147913815)
(46, 1.0207625605682822)
(47, 1.0171547389554139)
(48, 1.0101133171875112)
(49, 1.0099181464528426)
(50, 1.004776954650879)
}

\renewcommand{\drawPixelEight}{%
(1, 75.81170934294082)
(2, 39.45398489861958)
(3, -18.18540260099754)
(4, -52.231741818866)
(5, -2.6740850526539397)
(6, 45.171095185986616)
(7, 53.406631359588744)
(8, 22.98482166021185)
(9, 11.213254357186138)
(10, 0.75582504799356)
(11, 10.103286215392878)
(12, 8.773770121123043)
(13, 9.684934473361027)
(14, 19.37116178348655)
(15, 13.908851621344102)
(16, 7.394100702532276)
(17, 8.072291660431258)
(18, 6.559017391188247)
(19, 15.394025913709235)
(20, 7.6540499773427495)
(21, 4.637270060386687)
(22, 2.8639964313411785)
(23, -0.992233551410681)
(24, 0.2426935105301563)
(25, 0.4983267006991917)
(26, 1.7951377482403106)
(27, 1.6191584230897123)
(28, 1.3764178496011472)
(29, 0.5643549156692965)
(30, 0.8213881577660335)
(31, 1.6142039070621665)
(32, 1.0655565249138081)
(33, 0.27159997695976806)
(34, 0.18665084856904035)
(35, 0.5887491639207741)
(36, 0.6095795553273017)
(37, 0.6849560977779346)
(38, 0.6000136067417611)
(39, 0.6016075990148876)
(40, 0.6379704682476381)
(41, 0.6364599989373841)
(42, 0.6327061851474801)
(43, 0.6212396936413987)
(44, 0.6297299994874076)
(45, 0.6208798574430349)
(46, 0.6127541895782185)
(47, 0.6048174307032651)
(48, 0.5977210155793977)
(49, 0.5996729753228282)
(50, 0.5988879799842834)
}

\renewcommand{\drawPixelNine}{%
(1, 14.434613077610086)
(2, -40.59246323901931)
(3, 30.49072112778855)
(4, 33.35401061581117)
(5, 4.3469384462155425)
(6, 13.227859483394756)
(7, 5.632349245705543)
(8, -1.9896780181962503)
(9, 14.714812000194353)
(10, 27.07699389570365)
(11, 26.905898612092344)
(12, 26.891008964158516)
(13, 31.336437143545492)
(14, 21.764151592740717)
(15, 26.359901301890268)
(16, 10.20736740243819)
(17, 7.45217554679582)
(18, 2.4973588466362076)
(19, 4.852025223714422)
(20, 1.4871024529897157)
(21, -2.209848260758888)
(22, -2.5485741183473776)
(23, -0.39131079372782285)
(24, -1.7001695654045856)
(25, 0.43889890468738024)
(26, 2.355607250097452)
(27, 1.0993277747001318)
(28, 0.7895539887286177)
(29, -0.40823455635310046)
(30, -0.05980492881048838)
(31, 1.0364114365434265)
(32, 0.5912238340745851)
(33, 1.4278639354501759)
(34, 1.1831413847883354)
(35, 0.7613182003141985)
(36, 0.7130362564247472)
(37, 1.0161724246192871)
(38, 0.8078060063645783)
(39, 0.7584817032859315)
(40, 0.7214107942032859)
(41, 0.7970312868785381)
(42, 0.8353348039004372)
(43, 0.8545068671347856)
(44, 0.8364460810090596)
(45, 0.8303500714738316)
(46, 0.8412617240940018)
(47, 0.8390120842931684)
(48, 0.8374880351407389)
(49, 0.8377102002015386)
(50, 0.8394249677658082)
}

\renewcommand{\drawPixelTen}{%
(1, -39.02633193276053)
(2, -75.28024728104597)
(3, -98.44948131738133)
(4, -109.08361364716578)
(5, -70.27103769569406)
(6, -24.41846891447702)
(7, -3.382238366968081)
(8, 11.974910845687301)
(9, 34.227199658806086)
(10, 26.66486799025354)
(11, 18.392189189162433)
(12, -7.252922051654232)
(13, -20.859039621448296)
(14, -4.5497595316973065)
(15, 0.3111099075819566)
(16, -6.348444862426204)
(17, -2.80268497487265)
(18, 2.2873120098360973)
(19, 2.476365979350253)
(20, 3.1404660405996356)
(21, 2.690968424458613)
(22, 7.415738876900179)
(23, 8.252668331329042)
(24, 4.563614736221739)
(25, 1.122403622352223)
(26, 2.0688864838285403)
(27, 1.2281531245704849)
(28, 2.53747864727565)
(29, 0.48697068148930633)
(30, 0.5851102872205867)
(31, 1.3978152125678152)
(32, 1.302757730500292)
(33, 1.0800198024385632)
(34, 1.0175301143157074)
(35, 1.0802884953414866)
(36, 0.9702100211715747)
(37, 0.9182457512332655)
(38, 0.8997616556672512)
(39, 0.9749205986323926)
(40, 0.9688889631752763)
(41, 0.9751487237828934)
(42, 0.9875360923099915)
(43, 1.0108967537864069)
(44, 0.989749139972525)
(45, 0.9745191768349196)
(46, 0.9914804213155399)
(47, 0.9908465280865331)
(48, 0.9882673099672322)
(49, 0.9868435125354865)
(50, 0.9857709407806398)
}

==> trajectories/plot-trajectories3.tex <==
\input{data/drawPixel3.tex}
\node[label={[label distance=0.5cm,text depth=-1ex]right:{\bf\Large disc=edm, schedule=linear, scaling=none}}] at (1.5,8.5) {};
\begin{axis}[
 ymin=-120,
        ymax=152,
  grid={minor}, legend pos={north east}, legend cell align={left}, legend style={font=\normalsize, /tikz/every even column/.append style={column sep=1.6mm}},
  xmin=0,
        xmax=55,
		axis y line*=left,
		axis x line*=bottom,
		xtick={0, 10, 20, 30, 40, 50, 55}, xticklabels={$0$, $10$, $20$, $30$, $40$, $50$},
        yticklabels={},
        %xlabel={steps},
        % ylabel={Pixel state},
        label style={font=\huge},
        tick label style={font=\huge} 
]

\addplot[C0] coordinates {\drawPixelOne}; 
\addplot[C1] coordinates {\drawPixelTwo};
\addplot[C2] coordinates {\drawPixelThree};
\addplot[C3] coordinates {\drawPixelFour};
\addplot[C4] coordinates {\drawPixelFive};
\addplot[C5] coordinates {\drawPixelSix};
\addplot[C6] coordinates {\drawPixelSeven};
\addplot[C7] coordinates {\drawPixelEight};
\addplot[C8] coordinates {\drawPixelNine};
\addplot[C9] coordinates {\drawPixelTen};

%\legend{
%  {ADM},
%  {EDM},
%  {EDM-SEEDS (Ours)}
%}
\end{axis}

==> trajectories/plot-trajectories6.tex <==
\input{data/drawPixel6.tex}
% \node[label={[label distance=0.5cm,text depth=-1ex]right:{\bf\Large disc=edm, schedule=vp, scaling=vp}}] at (2,6) {};

\begin{axis}[
% width=\hh, height=\vv,
  xmin={0}, xmax={50}, xmode={linear}, xtick={0, 10, 20, 30, 40, 50}, xticklabels={$0$, $10$, $20$, $30$, $40$, $50$},
  %
  ymin={-130}, ymax={120}, ymode={linear}, ytick={1.2, 1.4, 1.6, 1.8, 2.0, 2.2, 2.4, 2.6, 2.8}, yticklabels={},
  grid={minor}, legend pos={north east}, legend cell align={left}, legend style={font=\normalsize, /tikz/every even column/.append style={column sep=1.6mm}},
  xmin=0,
        xmax=55,
		axis y line*=left,
		axis x line*=bottom,
		xtick={0, 10, 20, 30, 40, 50, 55}, xticklabels={$0$, $10$, $20$, $30$, $40$, $50$, $\text{steps}$},
        yticklabels={},
        %xlabel={steps},
        ylabel={Pixel state},
]

\addplot[C0] coordinates {\drawPixelOne}; 
\addplot[C1] coordinates {\drawPixelTwo};
\addplot[C2] coordinates {\drawPixelThree};
\addplot[C3] coordinates {\drawPixelFour};
\addplot[C4] coordinates {\drawPixelFive};
\addplot[C5] coordinates {\drawPixelSix};
\addplot[C6] coordinates {\drawPixelSeven};
\addplot[C7] coordinates {\drawPixelEight};
\addplot[C8] coordinates {\drawPixelNine};
\addplot[C9] coordinates {\drawPixelTen};

%\legend{
%  {ADM},
%  {EDM},
%  {EDM-SEEDS (Ours)}
%}
\end{axis}
